Certifying MIP-based Presolve Reductions for 0-1 Integer Linear Programs

It is well known that reformulating the original problem can be crucial for the performance of mixed-integer programming (MIP) solvers. To ensure correctness, all transformations must preserve the fea sibility status and optimal value of the problem, but there is currently no established methodology to express and verify the equivalence of two mixed-integer programs. In this work, we take a first step in this direction by showing how the correctness of MIP presolve reductions on 0-1 integer linear programs can be certified by using (and suitably extending) the VeriPB tool for pseudo-Boolean proof logging. Our experimental evaluation on both decision and optimization instances demonstrates the computational viability of the approach and leads to suggestions for future revisions of the proof format that will help to reduce the verbosity of the certificates and to accelerate the certification and verification process further.

==> TMP_snippets.tex <==

%%%
%%% TEXT SNIPPETS TO THROW AWAY OR USE ELSEWHERE
%%%




********** OMIT OR MOVE TO PRELIMINARIES **********

pseudo-Boolean formulas are in effect just another syntactic way of writing \mbox{$0$--$1$}  integer linear programs in the form
\begin{align*}
\min
&& \sum_{j\in N} c_j & x_j\\
\text{s.t.}
&& \sum_{j\in N} a_{ij} & x_j \geq b_i && \text{for } i\in\{1,\ldots,m\} \eqcomma\\
&&& x_j \in \{0, 1\} && \text{for } j \in N = \{1,\ldots,n\} \eqcomma
%\label{eq::pseudoboolean}
\end{align*}
with all $c_{j}, a_{ij}, b_i\in\mathbb{Z}$.
%
In the interest of readability, we will drop the row index~$i$ in constraints whenever this does not create ambiguity.
%
When convenient, we refer to a pair of constraints $E_{\geq} \synteq \sum_{j\in N} a_{j} x_j \geq b$ and $E_{\leq}  \synteq \sum_{j\in N} -a_{j} x_j \geq -b$ as an \emph{equality} $E \synteq E_{\geq}  \land E_{\leq} $.
% 
As a result, MIP solvers can be applied to solve pseudo-Boolean decision and
optimization problems directly \cite{BertholdHeinzPfetsch2008}, and are quite competitive for decision problems and most often superior for optimization problems \cite{DGN21LearnToRelax,DGDNS21Cutting}.


==> sections/experiments.tex <==
\section{Computational Study}
\label{sec::experiments}

In this section we quantify the cost of \emph{certifying} presolve reductions in a state-of-the-art implementation for MIP-based presolve (Sec.~\ref{subsec:impact-of-proof-logging-on-papilo}) and the cost of \emph{verifying} the resulting certificates (Sec.~\ref{subsec::verifying-presolving}).
In Sec.~\ref{subsec::analysis-on-propagation} we analyze the impact of certifying constraint propagation by RUP or by an explicit cutting planes proof.

\subsection{Experimental Setup}

For generating the presolve certificates we use the solver-independent presolve library \papilo~\cite{papilo},
which provides a large set of MIP and LP techniques from the literature, described in Sec.~\ref{sec::certifying}.
%For an even more detailed summary of MIP presolving refer to \cite{presolving_achterberg}.
%  offers multi-precision support AG: not used
Additionally, it accelerates the search for presolving reductions by parallelization.
To avoid expensive synchronization on the matrix, \papilo uses a transaction-based design.
However, logging the certificate is performed sequentially while evaluating the found transactions.

We base our experiments on models from the Pseudo-Boolean competition 2016~\cite{PB16} including
1398~linear small integer decision and 532~linear small integer optimization instances of the competitions
PB10, PB11, PB12, PB15, and PB16 and 295~decision and 145~optimization instances from MIPLIB~2017~\cite{GleixnerHendelGamrathEtal2021} in the OPB translation from \cite{MIPLIB01}.
(We exclude only the large-scale instance 
%%% Harmonizing that all instance names are using \solver style -AO
\solver{ivu06-big}
with a runtime of over 2 hours in \papilo.)
We use \papilo~2.2.0~\cite{papilo_b2f8073}
running on 16 threads and \veripb~2.0~\cite{veri_pb_a33ddbd7}.
This yields a total of 677~optimization and 1693~decision instances. 
%
The experiments are carried out on identical machines
with Intel Xeon Gold 5122 @ 3.60GHz 96 GB and are assigned 50,000 MB of memory. 
Three hours are set as a strict time limit for presolve plus certification and verification.
Reported times (always in seconds) do not include time for reading the instance file. 
For all aggregations, we use the shifted geometric mean with a shift of 1~second.

\subsection{Overhead of Proof Logging}
\label{subsec:impact-of-proof-logging-on-papilo}

In the first experiment, we analyze the overhead of proof logging in \papilo.
The average results are summarized in \Cref{tab::papilo::overhead},
separately over decision (dec) and optimization (opt) instances for \pb and \miplib.  
%Each row represents a different test set.
%The ``instances'' column contains all instances of the test set.
%The ``default'' column contains the runtime of \papilo without  default settings, 
%the ``verification'' column  contains the runtime while printing additionally the certificate. 
Column ``relative'' indicates the average slow-down incurred by printing the certificate.

\begin{table}[ht]
	\centering
	\small
	\begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}lrrr}
		\toprule
		Test set & size &  default (in seconds) & w/proof log (in seconds) & relative \\
		\midrule
		\pb-dec & 1398 & 0.050 & 0.076 & 1.52\\[-0.5ex]
		% default:  https://rubberband.zib.de/result/AYwgmpDMz5ZsptQZOoY5
		% RUP:		https://rubberband.zib.de/result/AYwu4u25z5ZsptQZOsKe
		% ADD:		https://rubberband.zib.de/result/AYwrtDe9z5ZsptQZOrta
		
		\miplib-dec&  295 & 0.500 & 0.633 & 1.27 \\[-0.5ex] 
		% default:  https://rubberband.zib.de/file/AYwgmPzez5ZsptQZOoR4
		% RUP:		https://rubberband.zib.de/result/AYwu4kbLz5ZsptQZOsFz
		% ADD:		https://rubberband.zib.de/result/AYwrsu4Lz5ZsptQZOreB
		
		\pb-opt &  532 & 0.442 & 0.807 & 1.83 \\[-0.5ex]
		% default:  https://rubberband.zib.de/result/AYwgO8Hvz5ZsptQZOn1X
		% RUP:		https://rubberband.zib.de/result/AYwu451nz5ZsptQZOsgY
		% ADD:		https://rubberband.zib.de/result/AYwrs4DMz5ZsptQZOrlC
		
		\miplib-opt&  144 & 0.414 & 1.956 & 4.72 \\[-0.5ex] 
		% supportcase11,ivu06-big
		% default:  https://rubberband.zib.de/result/AYwgmY3Nz5ZsptQZOoWj
		% RUP:		https://rubberband.zib.de/result/AYwu4gwaz5ZsptQZOsDd
		% ADD: 		https://rubberband.zib.de/result/AYwrsxvVz5ZsptQZOris
		\bottomrule
	\end{tabular*}
	\caption{Runtime comparison of \papilo with and without proof logging.}
	\label{tab::papilo::overhead}
\end{table}

The relative overhead of proof logging on decision instances is 52\% (for \pb) and 26.6\% (for \miplib), while the absolute difference is within a tenth of a second.
On optimization instances the overhead is significantly larger:  82.6\% (for \pb) and 472.5\% (for \miplib). 
This difference is explained by the fact that the objective function update rule requires \papilo to print the entire objective in the certificate when updating the objective. 
Hence, after every variable fixing the entire objective is printed even if only one coefficient and the offset have changed.
Especially for instances with dense and large objective functions this can lead to large certificate sizes and a large overhead.

One striking example is the instance \solver{normalized-datt256} of \pb, where bound strengthening finds $135\,206$ variable fixings.
Updating the objective function with $262\,144$ non-zeros for each of these variables leads to a huge certificate of about 138~GB.
As a result, the presolve time increases from 0.975~seconds without to 6625~seconds with proof logging.
%PB16-used/PB11/normaled-PB11/OPT-SMALL-INT/heinz/normalized-datt256
If the objective function was removed and the instance was treated as a decision problem, presolve plus proof logging would only take 3.369~seconds.
%Besides Probing which finds additional 68 variable fixes the presolver return the exactly same reductions.
%Even worse, 
One optimization instance (\solver{supportcase11} of \miplib) fails due to memory issues and is excluded in \Cref{tab::papilo::overhead}.

The above results demonstrate convincingly that the explicit objective function update rule described in Sec.~\ref{subsubsec:obju} should be complemented by an implicit version for which only the changes to the objective function need to be printed.
%
From the above results we may extrapolate that this would reduce the size of the certificate drastically and yield a proof logging performance that is very likely on par with the performance on the decision instances.
%Such an interface could be similar to the polish notation used for the constraints.
%~
For 99\% decision instances, we can further observe that the \emph{overhead per applied reduction} is below $0.186 \cdot 10^{-3}$~seconds over both test sets.
%
This means that the proof logging overhead is not only small on average, but that it is small also per applied reduction and on the vast majority of the instances.
%
These results show that the overhead scales well with the number of applied reductions and that proof logging remains feasible even for instances with a large number of transactions.
%
Here, under applied reductions we subsume all applied transactions and each variable fixing or row deletion in the first model clean-up phase.
%
During model clean-up, \papilo fixes variables and removes redundant constraints from the problem in a quick sequential sweep.
%
While \papilo technically does not count these reductions as full transactions found during the parallel presolve phase, their certification can incur the same overhead.


%% In \Cref{fig:secondspertransactions} we plot the costs per (applied) reductions as defined above on the y-axis and the number of transactions found on the x-axis.
%% Due to the parallel design, the presolvers in \papilo{} encapsulate each reduction they find in a transaction.
%% A transaction has additional data to check if the reduction can still be applied on a modified problem or needs to be discarded otherwise.
%% \papilo{} has also a model-clean up phase where fixed variables and constraints that are always true are removed from the problem.
%% Though this model-clean-up is quite trivial it can remove large chunks of the matrix and hence causes an overhead for the certifying.
%% Therefore, we count each variable fixing and each row deletion in the first model-clean-up call as transaction.
%Opening the file and starting to write takes time and is the dominating time factor for certifying instances with small certificates.
%Therefore, instances with less than 20 transactions have significantly higher costs per transaction than instances with more transactions.
%These are the instances in the upper left of the \Cref{fig:secondspertransactions}.
%For optimization, instances can be significantly larger depending on the non-zero entries of the objective function as discussed above.
%Meanwhile, on the decision instances, the 99\% quantile is $1.66 \cdot 10^{-4}$ respectively $2.53 \cdot 10^{-4}$.
%Using these values as upper-bounds for certifying means that the overhead is reasonable even for instances with many transactions.

\subsection{Verification Performance on Presolve Certificates}
\label{subsec::verifying-presolving}

In this experiment, we analyze the time to verify the certificates generated by \papilo.
The results over all instances for which \papilo{} took less than 30 minutes for presolving with proof logging are summarized in \Cref{tab::papilo_vs_veripb}.
The ``verified'' column lists the amount of instances verified within the time limit of 3~hours.
%The ``default'' and ``verification'' columns contain the runtime of \papilo with default and verification settings.
%The column ``\veripb{}'' lists the time that was necessary to verify the certificates.
Timeouts of \veripb are counted by twice the time limit, i.e., treated as PAR2.
Similar to \Cref{tab::papilo::overhead}, the ``relative'' columns report the relative overhead of \veripb{} runtime compared to \papilo.

\begin{table}[ht]
	\centering
	\small
	\begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrr}
		\toprule
		&           &           & \multicolumn{2}{c}{\papilo time (in s)} & \multicolumn{1}{c}{\veripb} & \multicolumn{2}{c}{relative time w.r.t.} \\
		\cmidrule{4-5}
		\cmidrule{7-8}
		Test set & size &  verified & w/proof log & default & \multicolumn{1}{c}{time (in s)} &  w/proof log & default  \\
		\midrule
		\pb-dec & 1398 & 1398 & 0.076 &0.050  & 1.28 & 16.81 & 25.54\\[-0.5ex] 
		\miplib-dec & 293 & 261 & 0.55 & 0.42 & 17.36 & 31.78& 41.37\\[-0.5ex] 
		\pb-opt & 531 & 520 & 0.78 & 0.44 & 16.17 & 20.74 & 36.75 \\[-0.5ex] 
		\miplib-opt & 140 & 133 & 1.38 & 0.27 & 10.40 & 7.53& 38.32 \\[-0.5ex] 
		\bottomrule
	\end{tabular*}
	\caption{
		Time (in seconds) to verify the certificates on instances with at most~30 minutes to presolve with proof logging. 
		Timeouts in \veripb{} are treated with PAR2.
		}
	\label{tab::papilo_vs_veripb}
\end{table}

%\AHil{
%	In \veripb{} it is not possible to set an time limit so I decided in the experiments to set the timelimit of \papilo{} and \veripb{} to 3 hours. 
%	\papilo{} is usually pretty fast so there should be plenty of time for \veripb{}. 
%	To ensure that I excluded instances where \papilo{} takes more than 30 minutes. 
%	In this case, \veripb{} still has 2.5 hours to verify which should be a fair amount. 
%	The timelimit of \veripb{} is then adjusted to 10800- presolving\_time.
%}
%\AO{I think this is fine. Alternatively, we could say that the timeout for presolving is 30 minutes and the timeout for VeriPB to 2.5 hours. So then we could look at the presolving time and exclude all instances that took more than 30 minutes from further consideration. For the remaining instances we can look at where the solving time is larger than 2.5 hours and say that these instances are timeout.}

First note that all certificates are successfully verified by \veripb{} (partially on the 50~instances where \veripb{} times out).
%
%However, verification generates a significant overhead. 
On average, for decision instances it takes between 16.81 and 31.78 times the time to verify the certificates than to produce them. 
The performance figures on optimization instances on slightly optimistic, since due to the bottlenecks on objective functions with many non-zeros exhibited in Sec.~\ref{subsec:impact-of-proof-logging-on-papilo}, six~instances are not included for which no certificates could be produced within 30 minutes.
Nevertheless, some decision instances produce a larger than average overhead.
For 25\% of the \pb-dec instances it takes more than 61.5x, and for 25\% of the \miplib-dec instances it takes more than 467x time to verify than to presolve the instance, see also Fig.~\ref{fig::experiment::PaPILOVeriPB}. 
%This is larger than what has been reported in the literature for verifying the certificates of a full solving process~\cite{BBNOV23CertifiedCoreGuided,GN21CertifyingParity}.
%% \AG{@AO/AH: Add citations for this.}
%% \AO{
%% 	The first two numbers are for proof logging overhead. The verification of proof from core-guided MaxSAT solvers \cite{BBNOV23CertifiedCoreGuided} is 3 times slower than solving in the median.
%% 	For SAT symmetry breaking, the paper does not report on mean/median slowdowns. They only give a 75\% percentile of 3.2 times slower checking than solving.
%% 	In \cite{GN21CertifyingParity}, I read that the solving time was 0.01 seconds without proof logging, 0.03 seconds with proof logging and unsatisfiability was verified in 1.29 seconds (factor 43).
%% 	In Constraint Programming~\cite{GMN22AuditableCP}, the slowdowns are also quite big. They did not do an extensive experimental evaluation and only report results on some instances. They have the following factors as slowdown for the instances they discuss: 1667.78, 7924, 57.4, 17.58, 48.46, 65, 10.4
%% 	AH: \cite{GMNO22CertifiedCNFencodingPB} is about 49 times slower.
%% }

To understand this result note that presolving amounts more to a transformation than to a (partial) solution of the problem.
%
Each reduction has to be certified and verified while a purely solution-targeted algorithm may be able to skip certifying of a larger part of the findings that eventually do not contribute to the final proof of optimality.
%
Hence, the performance of \veripb on presolve certificates should rather be compared to the overhead for verifying CNF translations~\cite{GMNO22CertifiedCNFencodingPB},
for which a similar performance overhead is reported as in Fig.~\ref{fig::experiment::PaPILOVeriPB}.

\begin{figure}[ht]
	\centering
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
			\begin{axis}[
				scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
				ylabel=\veripb (time in seconds),
				xlabel=\papilo (time in seconds),
				xmode=log,
				ymode=log,
				grid=both,
				grid style={line width=.1pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				minor tick num=5,
				xtick={-0.01,0.01,0.1,1,10,100,1000},
				ytick={-0.01,0.01,0.1,1,10,100,1000,10000},
			]
				\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x });
				\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x + 10});
				\addplot[scatter,only marks, scatter src=explicit symbolic]
				table[meta=label] {
					x y label
					1000 1000 peer
					-0.01 -0.01 peer
					0.058 2.02 green
					0.02 1.0 green
					0.07 2.7600000000000002 green
					0.112 4.2 green
					0.023 1.11 green
					1.024 32.56999999999999 green
					1.108 35.169999999999995 green
					0.446 17.689999999999998 green
					0.941 27.98 green
					0.508 19.25 green
					0.982 33.209999999999994 green
					1.402 42.89 green
					1.07 32.12 green
					0.479 18.23 green
					1.031 32.949999999999996 green
					0.469 19.66 green
					1.02 32.269999999999996 green
					1.104 34.339999999999996 green
					1.289 40.089999999999996 green
					0.468 17.86 green
					1.16 36.19 green
					0.501 19.06 green
					1.203 37.37 green
					1.08 34.8 green
					0.465 17.939999999999998 green
					1.039 31.63 green
					1.176 36.97 green
					0.524 19.6 green
					0.516 12.89 green
					1.12 33.51 green
					1.442 44.64 green
					1.447 44.379999999999995 green
					0.309 9.11 green
					1.397 44.26 green
					0.367 10.709999999999999 green
					1.338 42.23 green
					0.392 13.01 green
					0.272 7.48 green
					0.852 21.97 green
					1.089 42.209999999999994 green
					0.674 26.61 green
					1.49 45.33 green
					0.645 15.280000000000001 green
					1.675 52.18 green
					0.603 23.85 green
					1.236 39.019999999999996 green
					1.378 210.77 green
					1.372 150.78 green
					1.445 210.3 green
					1.798 207.85 green
					2.002 288.67 green
					1.141 137.12 green
					1.743 323.05 green
					1.467 191.64999999999998 green
					3.119 294.14000000000004 green
					3.341 200.76000000000002 green
					1.102 302.51 green
					1.65 341.38 green
					1.082 149.09 green
					1.485 179.56 green
					1.702 300.03000000000003 green
					0.934 146.24 green
					1.466 275.27000000000004 green
					2.736 273.46 green
					3.586 280.03000000000003 green
					1.676 319.07 green
					2.139 293.93 green
					1.239 130.37 green
					1.056 248.16 green
					0.948 272.12 green
					1.346 174.12 green
					1.476 211.54000000000002 green
					1.861 202.27 green
					2.255 294.22999999999996 green
					0.996 267.0 green
					1.282 282.06 green
					2.147 232.55 green
					1.261 212.92 green
					0.957 220.92000000000002 green
					1.702 254.49 green
					2.347 217.75 green
					1.347 298.47 green
					1.419 157.02 green
					1.896 213.84 green
					1.043 246.2 green
					2.003 156.13 green
					2.987 269.0 green
					1.653 248.66 green
					2.797 245.4 green
					1.289 193.14000000000001 green
					2.308 263.06 green
					3.1 199.9 green
					1.422 209.85 green
					1.442 307.64 green
					2.019 255.01999999999998 green
					0.955 178.31 green
					1.408 275.09 green
					3.25 213.19000000000003 green
					1.555 183.82999999999998 green
					1.163 292.73 green
					1.222 154.23 green
					0.242 14.450000000000001 green
					0.408 14.379999999999999 green
					0.375 10.510000000000002 green
					0.346 10.34 green
					0.462 9.870000000000001 green
					0.575 17.52 green
					0.456 12.48 green
					0.506 18.8 green
					0.355 17.78 green
					0.842 19.25 green
					0.3 9.92 green
					0.512 15.459999999999999 green
					0.346 14.389999999999999 green
					0.42 11.360000000000001 green
					0.202 11.85 green
					0.353 8.23 green
					0.458 11.63 green
					0.464 17.36 green
					0.371 13.88 green
					0.347 15.459999999999999 green
					0.258 11.34 green
					0.367 13.74 green
					0.36 17.52 green
					0.314 18.55 green
					0.284 10.14 green
					0.745 21.52 green
					0.322 14.049999999999999 green
					0.368 22.96 green
					0.357 10.870000000000001 green
					0.784 141.67000000000002 green
					1.416 142.96 green
					1.363 125.78 green
					1.259 190.61999999999998 green
					1.695 109.08 green
					1.086 133.11 green
					1.073 130.41 green
					1.211 130.67000000000002 green
					1.611 123.44 green
					0.91 124.06 green
					1.672 162.19 green
					0.865 147.1 green
					1.644 157.74 green
					1.403 160.81 green
					1.569 121.92 green
					1.016 122.91000000000001 green
					1.008 171.0 green
					1.945 122.92 green
					1.507 80.24 green
					0.691 112.78999999999999 green
					1.017 73.63000000000001 green
					1.073 84.76 green
					1.86 121.66 green
					1.804 124.47999999999999 green
					2.586 151.42000000000002 green
					0.829 98.88 green
					1.909 131.78 green
					1.318 117.23 green
					1.901 133.2 green
					0.971 125.45 green
					1.151 123.28 green
					0.696 112.45 green
					0.755 44.93 green
					0.578 51.77 green
					0.788 30.35 green
					0.768 38.62 green
					0.806 46.11 green
					0.689 61.19 green
					0.749 36.14 green
					0.897 56.82 green
					0.649 60.290000000000006 green
					0.825 39.88 green
					0.878 68.22999999999999 green
					1.525 47.41 green
					0.758 46.75 green
					0.916 61.41 green
					1.082 34.71 green
					0.805 70.64 green
					0.663 54.85 green
					0.69 44.410000000000004 green
					0.887 91.22 green
					0.593 48.21 green
					0.686 55.7 green
					1.356 53.12 green
					1.228 57.96 green
					0.121 2.61 green
					8.28 1522.1 green
					0.046 2.54 green
					1.797 1105.18 green
					0.589 4.1899999999999995 green
					0.046 6.52 green
					0.161 129.15 green
					0.117 2.33 green
					2.122 50.73 green
					2.501 17.9 green
					0.064 14.030000000000001 green
					1.17 61.59 green
					0.036 3.35 green
					0.338 1.37 green
					0.39 72.36000000000001 green
					0.038 1.1 green
					0.041 4.05 green
					2.787 2298.02 green
					23.582 730.9200000000001 green
					0.373 214.34 green
					0.164 1.2400000000000002 green
					11.829 288.56 green
					12.797 9338.81 green
					5.463 6.449999999999996 green
					0.041 1.63 green
					0.045 1.6600000000000001 green
					0.043 1.65 green
					0.042 1.7200000000000002 green
					0.04 1.6199999999999999 green
					0.044 1.5999999999999999 green
					0.066 1.16 green
					0.043 1.6400000000000001 green
					0.04 1.65 green
					0.051 1.73 green
					0.056 1.2 green
					0.043 1.65 green
					0.041 1.6400000000000001 green
					0.043 1.65 green
					0.049 1.65 green
					0.052 1.14 green
					0.047 1.65 green
					0.059 1.3399999999999999 green
					0.059 1.3199999999999998 green
					0.061 2.79 green
					0.171 19.49 green
					0.157 15.65 green
					0.117 7.64 green
					1.551 236.67999999999998 green
					2.429 542.5699999999999 green
					0.87 149.12 green
					2.883 492.05 green
					2.445 543.42 green
					2.569 560.5699999999999 green
					3.108 570.5699999999999 green
					1.48 221.04000000000002 green
					2.783 552.78 green
					2.46 542.45 green
					2.814 593.6999999999999 green
					2.856 563.4200000000001 green
					1.466 210.60000000000002 green
					2.902 571.46 green
					2.627 566.6800000000001 green
					1.634 396.22 green
					2.025 397.86 green
					1.531 233.3 green
					2.182 456.32 green
					3.248 594.88 green
					28.712 4814.55 green
					11.544 7445.39 green
					0.384 641.04 green
					36.375 3728.98 green
					0.366 352.07 green
					29.009 4815.26 green
					0.415 144.20999999999998 green
					0.365 277.45 green
					0.351 176.67999999999998 green
					0.316 81.14 green
					0.357 283.24 green
					35.499 3749.5699999999997 green
					12.209 1428.4199999999998 green
					0.369 278.07 green
					35.987 3706.46 green
					0.365 279.92 green
					0.296 276.69 green
					0.422 631.04 green
					0.423 636.8299999999999 green
					35.261 3741.86 green
					14.692 959.79 green
					0.353 173.67 green
					0.308 81.54 green
					0.313 79.92 green
					43.199 2565.06 green
					36.104 3729.95 green
					44.41 2556.75 green
					11.952 7381.62 green
					28.889 4818.21 green
					0.35 369.28 green
					14.974 9254.61 green
					2.893 9248.31 green
					15.048 9167.84 green
					15.529 9222.88 green
					15.695 1133.1799999999998 green
					14.689 5619.71 green
					14.824 9204.179999999998 green
					14.342 9205.839999999998 green
					15.131 9212.01 green
					15.0 9221.660000000002 green
					15.13 9228.630000000001 green
					0.152 28.43 blue
					0.189 35.449999999999996 blue
					0.17 31.11 blue
					0.183 37.269999999999996 blue
					0.187 34.44 blue
					0.511 62.17 blue
					0.181 34.739999999999995 blue
					0.115 20.299999999999997 blue
					0.176 31.03 blue
					0.12 20.060000000000002 blue
					0.181 22.919999999999998 blue
					0.177 34.339999999999996 blue
					0.192 33.74 blue
					0.188 34.35 blue
					0.177 33.68 blue
					0.227 46.04 blue
					0.175 27.38 blue
					0.069 10.22 blue
					0.246 43.23 blue
					0.215 44.95 blue
					0.054 7.17 blue
					0.076 10.54 blue
					0.1 17.01 blue
					0.075 11.43 blue
					0.193 37.269999999999996 blue
					0.209 34.14 blue
					0.158 29.46 blue
					0.076 12.15 blue
					0.117 19.63 blue
					0.086 14.26 blue
					0.17 25.38 blue
					0.179 40.559999999999995 blue
					0.168 32.83 blue
					0.087 14.2 blue
					0.295 72.71 blue
					0.291 71.32 blue
					0.341 95.94 blue
					0.746 233.73000000000002 blue
					0.457 135.68 blue
					0.605 158.58 blue
					0.554 181.06 blue
					3.106 285.77 blue
					0.265 63.53 blue
					0.689 153.44 blue
					0.916 197.41 blue
					0.461 137.82999999999998 blue
					0.694 111.82 blue
					0.607 187.5 blue
					0.486 158.74 blue
					0.637 196.33999999999997 blue
					2.251 179.86999999999998 blue
					0.373 97.25 blue
					0.78 137.95 blue
					1.205 153.42 blue
					0.708 194.0 blue
					0.901 243.61 blue
					0.672 178.83 blue
					0.494 146.74 blue
					0.703 187.24 blue
					0.594 165.60999999999999 blue
					0.535 182.82000000000002 blue
					1.207 276.65 blue
					0.376 104.39 blue
					0.392 113.06 blue
					0.233 80.66 blue
					0.516 131.1 blue
					1.36 176.95999999999998 blue
					0.584 113.27999999999999 blue
					0.525 168.43 blue
					0.201 41.23 blue
					1.053 231.14000000000001 blue
					0.358 102.38 blue
					0.29 74.92 blue
					0.407 117.49 blue
					1.103 202.51 blue
					0.355 104.55000000000001 blue
					0.701 214.65 blue
					0.171 32.71 blue
					0.264 56.370000000000005 blue
					0.17 35.300000000000004 blue
					0.406 105.46000000000001 blue
					0.372 96.25999999999999 blue
					1.066 103.01 blue
					0.126 22.46 blue
					0.267 57.54 blue
					0.19 38.96 blue
					0.201 58.269999999999996 blue
					0.271 63.03 blue
					0.248 52.86 blue
					0.143 26.099999999999998 blue
					0.222 77.71 blue
					0.179 38.96 blue
					0.278 63.49 blue
					0.376 102.45 blue
					0.224 44.67 blue
					0.307 73.5 blue
					0.212 72.44000000000001 blue
					0.158 31.400000000000002 blue
					0.25 55.9 blue
					0.194 42.63 blue
					0.107 18.46 blue
					0.179 34.77 blue
					0.355 89.2 blue
					0.287 66.62 blue
					0.36 91.25 blue
					0.13 33.8 blue
					0.416 113.24 blue
					0.047 7.23 blue
					0.053 6.82 blue
					0.04 7.2700000000000005 blue
					0.026 2.28 blue
					0.071 9.790000000000001 blue
					0.064 9.270000000000001 blue
					0.146 15.97 blue
					0.101 15.62 blue
					0.063 6.44 blue
					0.025 3.7 blue
					0.15 12.520000000000001 blue
					0.132 18.68 blue
					0.07 10.860000000000001 blue
					0.069 9.71 blue
					0.094 10.16 blue
					0.135 15.479999999999999 blue
					0.078 11.49 blue
					0.085 12.8 blue
					0.062 10.860000000000001 blue
					0.115 13.629999999999999 blue
					0.1 10.239999999999998 blue
					0.044 5.86 blue
					0.024 1.8 blue
					0.097 13.77 blue
					0.066 12.55 blue
					0.085 9.15 blue
					0.068 8.530000000000001 blue
					0.106 12.54 blue
					0.071 9.930000000000001 blue
					0.092 15.24 blue
					0.196 1.4700000000000002 blue
					0.192 1.4900000000000002 blue
					0.92 4.27 blue
					0.238 6.23 blue
					5.848 50.11 blue
					0.175 1.3000000000000003 blue
					1.774 199.87 blue
					6.535 53.03 blue
					0.234 8.96 blue
					1.157 14.530000000000001 blue
					74.857 700.27 blue
					1.043 25.61 blue
					106.694 1247.08 blue
					0.235 1.8499999999999999 blue
					0.194 4.529999999999999 blue
					0.335 5.39 blue
					0.157 1.15 blue
					1.638 210.83 blue
					0.821 6.550000000000001 blue
					1.646 209.52 blue
					1.089 8.56 blue
					1.638 210.17000000000002 blue
					1.239 97.72 blue
					11.395 97.36999999999999 blue
					4.917 41.150000000000006 blue
					1.568 121.82000000000001 blue
					0.181 1.3000000000000003 blue
					0.151 1.16 blue
					0.96 7.609999999999999 blue
					0.999 7.41 blue
					5.184 595.72 blue
					0.198 1.48 blue
					0.962 16.05 blue
					0.961 7.859999999999999 blue
					0.862 6.5600000000000005 blue
					0.971 7.799999999999999 blue
					1.094 8.52 blue
					0.179 1.33 blue
					0.201 1.48 blue
					0.261 6.38 blue
					0.21 5.42 blue
					4.497 37.370000000000005 blue
					20.617 164.42 blue
					0.852 13.290000000000001 blue
					0.174 1.31 blue
					0.061 4.94 blue
					0.113 10.41 blue
					0.173 20.82 blue
					0.18 24.89 blue
					0.041 4.96 blue
					0.039 3.93 blue
					0.046 3.53 blue
					0.042 4.82 blue
					0.042 4.71 blue
					0.045 4.7 blue
					0.041 4.5 blue
					0.044 3.93 blue
					0.044 4.46 blue
					0.04 3.64 blue
					0.04 3.77 blue
					0.041 4.03 blue
					0.042 4.45 blue
					0.038 3.48 blue
					0.044 3.48 blue
					0.04 3.96 blue
					0.041 3.5100000000000002 blue
					0.043 5.0 blue
					0.039 3.98 blue
					0.039 3.8 blue
					0.042 4.46 blue
					0.043 4.890000000000001 blue
					0.037 3.46 blue
					0.041 4.2700000000000005 blue
					0.043 4.38 blue
					0.038 3.8000000000000003 blue
					0.041 3.82 blue
					0.039 3.47 blue
					0.041 4.25 blue
					0.041 4.37 blue
					0.048 4.12 blue
					0.048 3.52 blue
					0.042 4.75 blue
					0.063 4.34 blue
					0.044 4.3500000000000005 blue
					0.038 3.61 blue
					0.046 3.81 blue
					0.051 3.9699999999999998 blue
					0.044 3.68 blue
					0.046 3.87 blue
					0.042 4.840000000000001 blue
					0.047 3.1100000000000003 blue
					0.033 2.91 blue
					0.037 2.5 blue
					0.03 3.08 blue
					0.036 2.72 blue
					0.044 4.74 blue
					0.037 2.92 blue
					0.038 3.33 blue
					0.04 3.6300000000000003 blue
					0.028 2.5 blue
					0.043 4.87 blue
					0.036 2.91 blue
					0.031 3.03 blue
					0.041 4.25 blue
					0.036 3.45 blue
					0.042 4.42 blue
					0.036 3.1 blue
					0.041 4.71 blue
					0.033 2.8200000000000003 blue
					0.036 3.1900000000000004 blue
					0.045 4.04 blue
					0.033 3.0900000000000003 blue
					0.049 3.81 blue
					0.041 3.0700000000000003 blue
					0.049 4.16 blue
					0.03 3.17 blue
					0.045 2.79 blue
					0.047 4.08 blue
					0.035 3.11 blue
					0.039 4.01 blue
					0.042 2.7600000000000002 blue
					0.04 4.0600000000000005 blue
					0.035 2.6 blue
					0.034 2.55 blue
					0.04 4.03 blue
					0.038 2.5700000000000003 blue
					0.043 4.24 blue
					0.033 3.1 blue
					0.033 3.17 blue
					0.048 4.050000000000001 blue
					0.028 2.91 blue
					0.046 4.7700000000000005 blue
					0.029 2.97 blue
					0.032 2.4899999999999998 blue
					0.041 4.07 blue
					0.037 2.54 blue
					0.042 4.46 blue
					0.028 2.7800000000000002 blue
					0.048 3.1700000000000004 blue
					0.049 4.2 blue
					0.037 2.6900000000000004 blue
					0.056 4.140000000000001 blue
					0.033 3.41 blue
					0.042 3.24 blue
					0.037 3.72 blue
					0.037 3.0 blue
					0.038 3.4400000000000004 blue
					0.028 2.47 blue
					0.044 3.93 blue
					0.032 3.35 blue
					0.042 4.2 blue
					0.029 2.6500000000000004 blue
					0.034 3.31 blue
					0.046 4.87 blue
					0.031 2.55 blue
					0.049 4.94 blue
					0.034 3.29 blue
					0.036 3.2600000000000002 blue
					0.045 4.96 blue
					0.039 3.1100000000000003 blue
					0.039 3.9000000000000004 blue
					0.045 2.97 blue
					0.031 3.1500000000000004 blue
					0.044 4.86 blue
					0.042 3.0100000000000002 blue
					0.04 3.61 blue
					0.033 3.11 blue
					0.04 3.78 blue
					0.042 2.81 blue
					0.038 3.1500000000000004 blue
					0.046 4.58 blue
					0.034 2.73 blue
					0.043 3.72 blue
					0.044 2.75 blue
					0.044 4.01 blue
					0.041 3.39 blue
					0.039 2.6500000000000004 blue
					0.04 3.92 blue
					0.039 2.7 blue
					0.044 4.08 blue
					0.032 2.7800000000000002 blue
					0.044 3.3200000000000003 blue
					0.038 3.56 blue
					0.034 3.35 blue
					0.04 3.86 blue
					0.038 2.7 blue
					0.041 4.2 blue
					0.032 2.53 blue
					0.047 4.84 blue
					0.03 2.75 blue
					0.038 2.83 blue
					0.04 4.09 blue
					0.037 3.38 blue
					0.047 3.83 blue
					0.03 2.74 blue
					0.041 3.0300000000000002 blue
					0.043 4.54 blue
					0.036 2.99 blue
					0.051 4.21 blue
					0.039 3.0900000000000003 blue
					0.046 4.890000000000001 blue
					0.036 2.85 blue
					0.035 2.9000000000000004 blue
					0.042 4.140000000000001 blue
					0.041 2.8800000000000003 blue
					0.035 2.72 blue
					0.044 4.87 blue
					0.035 3.0 blue
					0.039 3.7 blue
					0.034 2.9 blue
					0.041 3.93 blue
					0.044 3.08 blue
					0.033 2.77 blue
					0.04 3.5 blue
					0.031 3.12 blue
					0.042 3.66 blue
					0.042 3.41 blue
					0.04 4.07 blue
					0.038 3.0900000000000003 blue
					0.037 3.58 blue
					0.042 4.390000000000001 blue
					0.042 3.54 blue
					0.042 3.9899999999999998 blue
					0.04 4.16 blue
					0.038 3.3200000000000003 blue
					0.031 2.6900000000000004 blue
					0.043 4.11 blue
					0.034 3.1 blue
					0.047 4.0200000000000005 blue
					0.068 1.15 blue
					0.071 1.1400000000000001 blue
					0.076 1.1400000000000001 blue
					0.461 108.85000000000001 blue
					0.038 1.32 blue
					0.079 1.12 blue
					0.902 178.9 blue
					0.064 1.0299999999999998 blue
					0.879 165.73999999999998 blue
					0.061 1.02 blue
					0.077 1.1600000000000001 blue
					0.022 3.22 blue
					0.072 1.06 blue
					0.075 1.1600000000000001 blue
					0.064 1.02 blue
					0.071 1.0 blue
					0.017 1.44 blue
					0.044 7.32 blue
					0.075 48.42 blue
					0.029 1.02 blue
					0.024 1.89 blue
					0.029 2.32 blue
					0.043 22.7 blue
					0.114 17.0 blue
					0.067 42.760000000000005 blue
					0.023 1.24 blue
					0.032 2.05 blue
					0.042 3.22 blue
					0.064 8.09 blue
					0.053 1.92 blue
					0.051 1.95 blue
					0.055 1.96 blue
					0.055 1.89 blue
					0.059 2.1100000000000003 blue
					0.065 1.96 blue
					0.062 2.01 blue
					0.059 1.93 blue
					0.061 2.07 blue
					0.055 1.94 blue
					0.057 1.98 blue
					0.06 1.96 blue
					0.054 2.0 blue
					0.068 1.9799999999999998 blue
					0.054 1.94 blue
					0.065 2.0 blue
					0.063 1.77 blue
					0.072 1.83 blue
					0.061 1.83 blue
					0.071 1.8399999999999999 blue
					0.063 1.75 blue
					0.064 1.88 blue
					0.063 1.73 blue
					0.071 1.83 blue
					0.061 1.76 blue
					0.063 1.78 blue
					0.076 1.95 blue
					0.062 1.83 blue
					0.074 2.03 blue
					0.064 1.77 blue
					0.058 1.76 blue
					0.059 1.75 blue
					0.062 1.76 blue
					0.073 1.8699999999999999 blue
					0.07 1.8499999999999999 blue
					0.06 1.77 blue
					0.07 1.93 blue
					0.076 1.8399999999999999 blue
					0.06 1.8599999999999999 blue
					0.067 1.77 blue
					0.05 1.88 blue
					0.085 1.95 blue
					0.063 1.8599999999999999 blue
					0.068 1.96 blue
					0.067 1.96 blue
					0.072 1.9699999999999998 blue
					0.128 5.04 blue
					0.164 6.06 blue
					0.203 6.65 blue
					0.13 5.05 blue
					0.137 5.23 blue
					0.16 5.85 blue
					0.18 5.79 blue
					0.176 6.12 blue
					0.148 5.510000000000001 blue
					0.149 5.7 blue
					0.129 5.1000000000000005 blue
					0.168 5.989999999999999 blue
					0.181 6.1899999999999995 blue
					0.131 5.37 blue
					0.192 6.23 blue
					0.179 5.82 blue
					0.131 5.21 blue
					0.137 5.49 blue
					0.152 5.69 blue
					0.145 5.54 blue
					0.183 6.21 blue
					0.199 6.49 blue
					0.196 6.1000000000000005 blue
					0.146 3.16 blue
					0.168 5.47 blue
					0.16 5.96 blue
					0.17 3.0900000000000003 blue
					0.181 6.28 blue
					0.179 6.1000000000000005 blue
					0.127 5.04 blue
				};
			\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\begin{minipage}[t]{.05\linewidth}
		\ 
	\end{minipage}
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
			\begin{axis}[
				scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
				ylabel=\veripb (time in seconds),
				xlabel=\papilo (time in seconds),
				xmode=log,
				ymode=log,
				grid=both,
				grid style={line width=.1pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				minor tick num=5,
				xtick={0.01,0.1,1,10,100,1000},
				ytick={0.01,0.1,1,10,100,1000,10000},
			]
				\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x});
				\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x + 10});
				\addplot[scatter,only marks, scatter src=explicit symbolic]%
				table[meta=label] {
					x y label
					1000 1000 peer
					0.102 1.19 green
					3.848 165.72 green
					27.457 646.6500000000001 green
					0.182 12.59 green
					0.115 1.05 green
					0.123 6.8 green
					0.139 11.43 green
					0.842 256.86 green
					38.94 7884.12 green
					11.558 419.35 green
					0.664 1.0700000000000003 green
					0.089 45.68 green
					8.87 479.37 green
					0.234 8.51 green
					0.702 54.300000000000004 green
					5.387 316.85999999999996 green
					0.497 69.61 green
					1.274 3.34 green
					2.018 1.6799999999999997 green
					1.025 9.86 green
					0.054 1.1 green
					311.138 7942.97 green
					0.059 17.09 green
					0.611 15.020000000000001 green
					2.16 20.25 green
					2.329 470.56 green
					88.496 9503.519999999999 green
					0.241 43.98 green
					0.09 2.96 green
					23.603 479.96 green
					0.057 1.38 green
					0.054 7.7299999999999995 green
					0.143 1.33 green
					0.029 3.6100000000000003 green
					0.028 1.13 green
					0.4 47.0 green
					0.161 26.88 green
					13.733 758.45 green
					1.51 969.4 green
					0.031 1.0999999999999999 green
					295.229 6644.179999999999 green
					0.591 14.3 green
					0.272 1.06 green
					0.218 5.01 green
					0.057 4.93 green
					0.924 97.39 green
					2.17 960.87 green
					0.116 2.9699999999999998 green
					0.046 159.42 green
					56.545 5013.660000000001 green
					2.515 240.53 green
					1.339 14.08 green
					4.246 196.54999999999998 green
					0.03 2.14 green
					6.343 142.73 green
					0.707 76.77 green
					0.035 1.3 green
					0.575 2.7800000000000002 green
					0.02 1.2 green
					19.694 747.0500000000001 green
					18.963 454.07 green
					1.394 2.26 green
					1.196 5.729999999999999 green
					0.223 2.38 green
					1.044 196.88 green
					0.358 61.07 green
					0.087 13.799999999999999 green
					14.235 1466.05 green
					67.257 1499.74 green
					0.065 2.5700000000000003 green
					0.727 429.64000000000004 blue
					0.253 492.65999999999997 blue
					0.226 2.39 blue
					0.295 453.4 blue
					0.033 101.67999999999999 blue
					3.288 4722.26 blue
					0.32 34.519999999999996 blue
					0.035 9.26 blue
					0.052 7.640000000000001 blue
					0.205 1740.51 blue
					2.507 789.37 blue
					0.102 1.46 blue
					0.033 2.16 blue
					0.037 1.94 blue
					1.259 194.56 blue
					0.059 1.48 blue
					2.54 240.45999999999998 blue
					0.59 3.2300000000000004 blue
					0.029 13.549999999999999 blue
					0.105 7.1499999999999995 blue
					0.677 51.75 blue
					0.128 2.92 blue
					0.09 1.21 blue
					0.217 2.41 blue
					8.411 8839.38 blue
					0.079 8.02 blue
					0.589 3.2300000000000004 blue
					0.02 1.25 blue
					0.133 8.66 blue
					0.065 7.74 blue
					0.044 159.69 blue
					0.676 51.769999999999996 blue
					2.503 242.9 blue
					0.124 1.29 blue
					0.68 9191.4 blue
					1.223 195.06 blue
					0.218 4.95 blue
					1.408 2.66 blue
					0.65 1.25 blue
					0.333 227.86 blue
					2.122 20.69 blue
					0.098 1.46 blue
					0.031 1.51 blue
					0.104 180.04 blue
					0.065 5.31 blue
					0.301 34.57 blue
					0.251 1533.37 blue
					0.702 79.07000000000001 blue
					0.136 5.13 blue
					1.151 5.3500000000000005 blue
					0.288 451.75 blue
					1.492 2724.86 blue
					0.041 1.6400000000000001 blue
					0.232 492.82 blue
					0.572 2.8200000000000003 blue
					1.143 433.0 blue
					1.041 10.100000000000001 blue
					3.292 4719.4800000000005 blue
					0.715 429.37 blue
					0.054 25.959999999999997 blue
					0.255 22.14 blue
					0.023 16.669999999999998 blue
					0.033 2.39 blue
					0.054 101.11999999999999 blue
					0.036 1.08 blue
					0.126 1.31 blue
					0.02 1.4 blue
					0.144 1043.3 blue
					1.47 2700.6 blue
					0.032 13.09 blue
					0.109 7.03 blue
					0.101 3.2600000000000002 blue
					0.086 59.309999999999995 blue
					0.207 5.010000000000001 blue
					0.011 1.07 blue
					1.126 439.37 blue
					0.093 59.209999999999994 blue
					0.028 16.06 blue
					0.034 1.07 blue
					0.093 1.21 blue
					0.033 13.05 blue
					8.402 8841.449999999999 blue
					1.887 1.67 blue
					0.104 179.29 blue
					0.018 1.19 blue
					30.348 954.29 blue
					0.625 79.46 blue
					0.82 215.37 blue
					0.046 26.24 blue
					0.105 778.59 blue
					0.034 1.94 blue
					0.132 2.9400000000000004 blue
					0.023 1.52 blue
					0.687 9190.679999999998 blue
					0.129 10.879999999999999 blue
					0.647 1.2599999999999998 blue
					0.167 1.06 blue
					0.44 1928.73 blue
					0.845 686.22 blue
					1.331 2.6799999999999997 blue
					0.015 10.04 blue
					0.372 1922.74 blue
					0.171 12.55 blue
					0.017 1.41 blue
					2.119 20.83 blue
					0.199 401.85999999999996 blue
					0.021 16.14 blue
					0.825 220.87 blue
					0.02 16.720000000000002 blue
					0.172 192.10999999999999 blue
					0.051 4.89 blue
					0.011 1.07 blue
					0.123 11.219999999999999 blue
					0.176 5.5 blue
					0.168 12.280000000000001 blue
					0.053 7.67 blue
					9.402 8953.82 blue
					0.197 404.46999999999997 blue
					0.181 1.06 blue
					0.836 682.47 blue
					0.329 78.22 blue
					0.997 9.79 blue
					0.054 111.6 blue
					0.03 1.14 blue
					0.805 145.70999999999998 blue
					0.046 6.61 blue
					0.105 778.61 blue
					0.036 13.45 blue
					0.053 111.88 blue
					0.704 75.95 blue
					0.936 95.37 blue
					0.013 9.84 blue
					0.123 11.4 blue
					1.912 1.6699999999999995 blue
					0.172 191.7 blue
					0.571 73.81 blue
					0.271 2985.85 blue
					0.03 2.01 blue
					9.373 3835.96 blue
					0.037 5.6 blue
					5.302 318.26 blue
				};
			\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\caption{
		Running times of \veripb vs. \papilo (with proof log) on test sets \pb (left) and \miplib (right), including all instances with more than 1~seconds in \veripb{} and less than 30~minutes in \papilo, and excluding timeouts.
		Green $+$ signs mark optimization and blue $\times$ signs mark decision instances.
%		The $y$-axis gives the time for presolving and
%		the $x$-axis gives the time for verifying. 
	}
	\label{fig::experiment::PaPILOVeriPB}
\end{figure}

\subsection{Performance Analysis on Constraint Propagation}
\label{subsec::analysis-on-propagation}

Finally, we analyze how \veripb's performance
% reductions of 
depends on whether we use RUP
or 
% deriving the propagation 
% directly is used (POL).
explicit
cutting planes rules (POL) to certify bound strengthening reductions from constraint propagation.\AG{clarify what we used above}
The results are summarized in \Cref{tab:rup_vs_add}.
%Each row represents a different test set.
%The ``instances'' column contains all instances of the test set.
The ``verified'' column contains the number of instances which \veripb could verify within the time limit; the ``time'' column reports the time for verification.
%The results of \Cref{tab:rup_vs_add} are visualized in \Cref{fig:add_vs_rup}. 

\begin{table}[ht]
	\centering
	\small
	\begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}lrrrrr}
		\toprule
		& &  \multicolumn{2}{c}{POL} & \multicolumn{2}{c}{RUP} &  \\[-0.5ex] 
		\cmidrule{3-4}
		\cmidrule{5-6}
		& size &  verified & time (in s) & verified & time (in s) & relative \\[-0.5ex] 
		\midrule
		\pb-dec & 284 & 284 & 4.23 & 284 & 4.54 & 1.073\\[-0.5ex] 
		\miplib-dec & 44 & 36 & 273.49 & 36 & 288.23& 1.053\\[-0.5ex] 
		\pb-opt & 155 & 143 & 29.67 & 143 & 30.97 & 1.043\\[-0.5ex] 
		\miplib-opt & 18 & 14 & 281.58 & 13 & 295.05& 1.048\\[-0.5ex] 

		\bottomrule
	\end{tabular*}
	\caption{Comparison of the runtime (in seconds) of \veripb with POL and RUP for instances with at least 10 propagations.}
	\label{tab:rup_vs_add}
\end{table}

Deriving the propagation directly is 5.3\% faster on \pb-dec, 7.3\% on \miplib-dec,  and 4.8\% faster on the \miplib-opt and 4.3\% on the \pb-opt.
A maximal slowdown of 4\% can be observed on 99\% of the decision instances when using RUP. 
While it is expected that verification is faster when the cutting planes proof is given explicitly, it is surprising that the performance difference of the methods is not more pronounced.
%
This is partly due to the cost of the watched-literal scheme~\cite{MMZZM01Engineering,SS06Pueblo} used by \veripb{} for unit propagation.
%
The overhead of maintaining the watches is present regardless of whether (reverse) unit propagation is used or not.
%
Furthermore, unit propagation is also used for automatically verifying redundance-based strengthening. 
%
Together, this limits the potential for runtime savings by providing the explicit cutting planes proof.

Furthermore, providing an explicit cutting planes proof for propagation requires printing the constraint into the certificate.
Hence, the certificate size becomes dependent on the number of non-zeros in the constraints leading to propagations.
By contrast, the overhead of RUP is constant and much smaller.
%% Especially for constraints with many non-zeros, deriving the constraint can lead to memory issues in \papilo and huge certificates. 
%% An example is the instance \solver{normalized-datt256} with zero objective function, for which verification time increases from 3.369 seconds (with RUP) to 865.321 seconds (with POL).

All in all, these results suggest to prefer RUP when deriving constraint propagation since it barely impacts the performance of \veripb{} and keeps the size of the certificate smaller.
%
The computational cost of RUP could be further reduced by extending it to accept an ordered list of constraints that shall be propagated first, similar as in~\cite{LRAT}. 
Such an extension could also be used for other presolving techniques, in particular probing and simple probing.

%Two optimization instances of \pb{} resulted in aborts when using the ``POL'' settings. 
%Please refer to \cref{subsec::analysis-on-propagation}.


==> sections/experiments_diff.tex <==
\section*{Experiments with diff}

excluded instances 

\miplib-opt: ivu59, ivu06-big, a2864-99blp, supportcase11

\miplib-dec: a2864-99blp.0.s/u, supportcase11.0.s/u

\pb-dec: normalized-184, 

\pb-opt: normalized-pb-simp-nonunif 

We use \papilo~2.2.0~\cite{papilo_3b082d4}
running on 16 threads and \veripb~2.0~\cite{veri_pb_dd7aa5a1}.

\begin{table}[ht]
	\centering
	\small
	\begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}lrrr}
		\toprule
		Test set & size &  default (in seconds) & w/proof log (in seconds) & relative \\
		\midrule
		\pb-dec & 1397 & 0.06 & 0.06 &  1.00\\[-0.5ex]
		\miplib-dec & 284 & 0.41 & 0.42 &  1.02\\[-0.5ex]
		\pb-opt & 530 & 0.64 & 0.66 &  1.03\\[-0.5ex]
		\miplib-opt & 141 & 0.32 & 0.33 &  1.03\\[-0.5ex]
		\bottomrule
	\end{tabular*}
	\caption{Runtime comparison of \papilo with and without proof logging.}
	\label{tab::papilo::overhead_obju_diff}
\end{table}

For 99\% decision instances, we can further observe that the \emph{overhead per applied reduction} is below $0.0$~seconds over all test sets.


\begin{table}[ht]
	\centering
	\small
	\begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrr}
		\toprule
		&           &           & \multicolumn{2}{c}{\papilo time (in s)} & \multicolumn{1}{c}{\veripb} & \multicolumn{2}{c}{relative time w.r.t.} \\
		\cmidrule{4-5}
		\cmidrule{7-8}
		Test set & size &  verified & w/proof log & default & \multicolumn{1}{c}{time (in s)} &  w/proof log & default  \\
		\midrule
		\pb-dec & 1397 & 1397 & 0.06 & 0.06 & 0.88 & 14.67 & 14.67\\[-0.5ex]
		\miplib-dec & 284 & 262 & 0.42 & 0.41 & 8.46 & 20.14 & 20.63\\[-0.5ex]
		\pb-opt & 530 & 519 & 0.66 & 0.64 & 10.30 & 15.61 & 16.09\\[-0.5ex]
		\miplib-opt & 141 & 138 & 0.33 & 0.32 & 4.95 & 15.00 & 15.47\\[-0.5ex]
		\bottomrule
	\end{tabular*}
	\caption{
		Time (in seconds) to verify the certificates on instances with at most~30 minutes to presolve with proof logging. 
		Timeouts in \veripb{} are treated with PAR2.
	}
	\label{tab::papilo_vs_veripb_obju_diff}
\end{table}


For 25\% over all test sets it takes more than 171x  time to verify than to presolve the instance, see also Fig.~\ref{fig::experiment::PaPILOVeriPB}. 

\begin{figure}[ht]
	\centering
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
		\begin{axis}[
		scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
		ylabel=\veripb (time in seconds),
		xlabel=\papilo (time in seconds),
		xmode=log,
		ymode=log,
		grid=both,
		grid style={line width=.1pt, draw=gray!10},
		major grid style={line width=.2pt,draw=gray!50},
		minor tick num=5,
		xtick={-0.01,0.01,0.1,1,10,100,1000},
		ytick={-0.01,0.01,0.1,1,10,100,1000,10000},
		]
		\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x });
		\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x + 10});
		\addplot[scatter,only marks, scatter src=explicit symbolic]
		table[meta=label] {
			x y label
			1000 1000 peer
			-0.01 -0.01 peer
		3.798 96.03 green
		2.867 161.12 green
		2.414 146.46 green
		3.924 186.22 green
		1.709 188.82999999999998 green
		2.165 207.76999999999998 green
		5.941 133.74 green
		3.539 124.39 green
		2.576 119.23 green
		1.364 94.25 green
		2.092 119.78 green
		2.35 110.08 green
		0.825 158.07999999999998 green
		1.014 143.22 green
		2.098 124.86000000000001 green
		2.283 219.14999999999998 green
		2.192 136.81 green
		1.751 188.59 green
		1.671 106.8 green
		4.193 166.22 green
		0.879 133.7 green
		4.05 179.98 green
		6.445 178.19 green
		7.607 157.57 green
		0.912 168.62 green
		1.982 126.78999999999999 green
		2.459 100.95 green
		2.501 112.58 green
		3.334 133.74 green
		0.943 109.07000000000001 green
		3.539 135.28 green
		5.216 153.17000000000002 green
		2.684 117.33999999999999 green
		3.619 157.24 green
		4.549 138.55 green
		2.917 165.89 green
		1.497 167.38 green
		5.187 169.34 green
		1.925 151.36 green
		2.091 104.17999999999999 green
		2.444 182.03 green
		1.782 167.82 green
		6.105 170.35999999999999 green
		3.262 178.58 green
		1.505 120.88 green
		1.594 123.57 green
		2.32 189.91 green
		1.008 151.23 green
		2.445 119.26 green
		0.994 188.18 green
		1.121 175.36 green
		4.42 185.89999999999998 green
		7.15 152.85 green
		2.556 204.51000000000002 green
		7.726 178.32000000000002 green
		3.653 37.93 green
		1.025 34.65 green
		0.942 37.559999999999995 green
		1.587 25.709999999999997 green
		1.214 41.82 green
		1.316 29.52 green
		1.571 25.94 green
		0.994 36.85 green
		1.502 23.939999999999998 green
		0.943 37.41 green
		1.76 41.18 green
		1.453 28.26 green
		2.888 34.12 green
		2.447 37.0 green
		1.152 27.61 green
		0.801 30.62 green
		1.442 42.98 green
		2.398 22.19 green
		1.011 33.24 green
		1.345 57.37 green
		1.577 25.44 green
		1.725 37.48 green
		1.435 29.9 green
		2.843 78.36999999999999 green
		2.343 101.25 green
		3.279 52.51 green
		0.682 68.25 green
		2.577 89.07 green
		2.48 76.21000000000001 green
		2.047 82.0 green
		5.863 96.66 green
		2.763 96.31 green
		1.138 76.97999999999999 green
		2.553 98.92999999999999 green
		3.998 77.61 green
		1.024 91.56 green
		1.936 78.01 green
		3.86 81.03999999999999 green
		2.835 97.23 green
		0.665 67.56 green
		0.824 86.77 green
		2.013 121.46000000000001 green
		1.353 107.64 green
		1.938 55.279999999999994 green
		3.638 78.92999999999999 green
		1.499 73.98 green
		3.918 76.21000000000001 green
		3.773 83.96 green
		1.616 81.33 green
		1.237 74.85 green
		3.034 77.41 green
		1.99 59.589999999999996 green
		1.251 78.85 green
		1.516 80.19 green
		3.571 71.0 green
		0.638 9.03 green
		0.966 9.709999999999999 green
		0.559 10.42 green
		0.287 8.76 green
		0.471 10.809999999999999 green
		0.566 6.0 green
		0.836 6.630000000000001 green
		0.673 8.959999999999999 green
		1.109 9.6 green
		1.114 10.2 green
		0.693 8.479999999999999 green
		0.458 8.17 green
		0.422 6.640000000000001 green
		0.227 9.219999999999999 green
		2.011 11.82 green
		1.102 6.21 green
		0.555 8.19 green
		0.649 12.53 green
		0.599 10.629999999999999 green
		1.868 11.76 green
		0.837 8.719999999999999 green
		0.724 6.7 green
		1.012 10.25 green
		1.098 11.66 green
		1.028 6.94 green
		0.754 5.0 green
		0.735 6.46 green
		0.771 8.52 green
		0.744 8.24 green
		0.007 1.24 green
		0.007 1.26 green
		0.005 1.0 green
		0.067 6.92 green
		0.058 6.6499999999999995 green
		0.055 7.23 green
		0.064 7.819999999999999 green
		0.056 6.64 green
		0.058 7.7299999999999995 green
		0.064 5.16 green
		0.067 7.569999999999999 green
		0.054 7.66 green
		0.058 5.930000000000001 green
		0.07 6.79 green
		0.081 7.06 green
		0.063 6.75 green
		0.061 6.46 green
		0.013 1.42 green
		0.063 7.2 green
		0.063 6.9399999999999995 green
		0.051 6.1 green
		0.059 7.3 green
		0.055 6.21 green
		0.056 7.09 green
		0.052 7.12 green
		0.062 7.3999999999999995 green
		0.055 6.279999999999999 green
		0.06 7.31 green
		0.067 8.940000000000001 green
		0.067 9.870000000000001 green
		0.07 8.530000000000001 green
		0.053 4.510000000000001 green
		0.018 1.82 green
		0.057 8.100000000000001 green
		0.058 8.33 green
		0.017 1.95 green
		0.024 2.48 green
		0.07 8.42 green
		0.038 10.940000000000001 green
		0.06 8.99 green
		0.014 1.4 green
		0.062 8.350000000000001 green
		0.061 8.47 green
		0.017 2.54 green
		0.211 61.25 green
		0.832 638.84 green
		0.033 4.04 green
		49.232 421.58 green
		0.749 26.01 green
		10.665 13.219999999999999 green
		0.068 102.11 green
		1.058 1.7200000000000002 green
		0.01 1.83 green
		0.064 311.11 green
		0.008 2.9000000000000004 green
		0.018 1.55 green
		0.178 2519.28 green
		0.013 5.08 green
		0.009 1.54 green
		3.355 105.99000000000001 green
		0.254 21.23 green
		2.355 1.3800000000000008 green
		32.01 4605.26 green
		30.612 4658.59 green
		32.981 543.4100000000001 green
		25.358 9715.19 green
		30.69 4581.91 green
		26.286 9755.460000000001 green
		29.759 4663.110000000001 green
		24.339 9726.05 green
		26.496 9668.22 green
		29.875 4618.59 green
		30.033 4597.33 green
		1.756 9667.83 green
		25.997 9705.29 green
		29.926 4653.5199999999995 green
		1.936 4710.24 green
		25.187 9701.35 green
		31.403 4615.2 green
		25.185 9715.85 green
		30.901 4610.400000000001 green
		0.243 928.01 green
		0.252 448.49 green
		0.151 316.92 green
		0.151 314.71 green
		0.173 131.7 green
		0.175 124.66 green
		0.181 27.380000000000003 green
		0.255 450.98 green
		0.137 129.9 green
		0.205 1445.27 green
		0.223 929.81 green
		0.242 920.89 green
		0.151 316.33 green
		0.141 317.77 green
		0.229 922.41 green
		0.171 128.5 green
		0.171 125.33 green
		0.257 446.7 green
		0.204 1441.7 green
		0.18 74.34 green
		0.203 935.9699999999999 green
		0.163 2902.8799999999997 green
		0.182 75.11 green
		0.179 27.37 green
		0.139 322.59 green
		0.624 2887.3399999999997 green
		0.21 1443.99 green
		0.18 27.39 green
		0.174 131.94 green
		0.244 925.0999999999999 green
		0.701 248.27 green
		0.416 222.92999999999998 green
		0.691 254.24 green
		0.412 214.42 green
		1.28 276.47 green
		1.833 263.34999999999997 green
		0.493 108.72999999999999 green
		1.382 219.58 green
		0.468 243.64 green
		0.404 191.67000000000002 green
		1.302 255.67 green
		0.392 96.89 green
		0.42 224.53 green
		0.469 106.39 green
		0.696 257.89000000000004 green
		0.409 218.79 green
		0.805 240.7 green
		1.036 256.21999999999997 green
		0.369 99.41 green
		0.482 101.38 green
		0.091 2.87 green
		0.136 5.949999999999999 green
		0.043 1.05 green
		0.147 7.37 green
		0.055 16.84 blue
		0.034 20.64 blue
		0.055 15.21 blue
		0.019 9.46 blue
		0.022 11.24 blue
		0.034 21.169999999999998 blue
		0.036 17.68 blue
		0.036 20.27 blue
		0.014 5.5200000000000005 blue
		0.022 10.950000000000001 blue
		0.016 7.1899999999999995 blue
		0.042 26.9 blue
		0.015 5.930000000000001 blue
		0.088 25.87 blue
		0.034 19.93 blue
		0.016 7.5200000000000005 blue
		0.424 37.23 blue
		0.015 6.24 blue
		0.038 21.799999999999997 blue
		0.035 22.07 blue
		0.04 21.869999999999997 blue
		0.036 21.61 blue
		0.037 24.47 blue
		0.085 13.72 blue
		0.037 19.05 blue
		0.043 30.209999999999997 blue
		0.029 17.38 blue
		0.011 3.86 blue
		0.087 19.91 blue
		0.031 17.43 blue
		0.032 19.12 blue
		0.015 6.59 blue
		0.038 20.619999999999997 blue
		0.022 11.360000000000001 blue
		0.05 36.59 blue
		0.038 24.18 blue
		0.088 70.38 blue
		0.068 37.190000000000005 blue
		0.074 61.349999999999994 blue
		0.077 68.98 blue
		0.029 16.12 blue
		0.036 22.45 blue
		0.036 23.02 blue
		0.075 64.7 blue
		0.032 19.17 blue
		0.023 10.930000000000001 blue
		0.035 20.32 blue
		0.101 70.46000000000001 blue
		0.075 59.169999999999995 blue
		0.082 58.72 blue
		0.032 18.35 blue
		0.066 41.99 blue
		0.076 31.71 blue
		0.025 13.32 blue
		0.045 29.009999999999998 blue
		0.049 33.169999999999995 blue
		0.073 61.599999999999994 blue
		1.65 82.35000000000001 blue
		0.054 32.79 blue
		0.066 37.45 blue
		0.084 53.589999999999996 blue
		0.057 50.15 blue
		0.073 40.540000000000006 blue
		0.043 27.61 blue
		2.094 105.0 blue
		0.836 127.13 blue
		0.09 69.25 blue
		0.041 27.06 blue
		0.246 113.14 blue
		4.235 105.53 blue
		0.248 124.32000000000001 blue
		0.058 46.13 blue
		0.437 121.14999999999999 blue
		0.102 100.38 blue
		0.151 110.06 blue
		0.061 48.43 blue
		0.121 109.47999999999999 blue
		1.292 167.09 blue
		0.085 65.25 blue
		0.348 129.56 blue
		0.082 69.83000000000001 blue
		0.132 89.77 blue
		0.257 106.18 blue
		0.138 99.08 blue
		0.056 42.33 blue
		0.466 114.82000000000001 blue
		0.74 87.32000000000001 blue
		0.486 101.98 blue
		0.077 64.49000000000001 blue
		1.103 134.4 blue
		0.092 88.26 blue
		0.237 105.91 blue
		0.691 146.03 blue
		0.094 74.98 blue
		0.264 87.21 blue
		0.111 66.55000000000001 blue
		0.75 72.98 blue
		0.237 82.71 blue
		1.669 96.58 blue
		0.806 93.65 blue
		0.124 99.25 blue
		6.033 175.36 blue
		0.081 66.77000000000001 blue
		0.418 139.12 blue
		1.596 160.69000000000003 blue
		0.065 47.470000000000006 blue
		0.406 119.03 blue
		0.016 5.63 blue
		0.03 5.01 blue
		0.013 4.79 blue
		0.004 1.11 blue
		0.056 7.680000000000001 blue
		0.013 4.76 blue
		0.016 4.44 blue
		0.017 6.46 blue
		0.018 7.15 blue
		0.092 8.93 blue
		0.067 8.280000000000001 blue
		0.021 6.140000000000001 blue
		0.018 7.38 blue
		0.019 7.44 blue
		0.005 1.46 blue
		0.048 6.69 blue
		0.039 6.41 blue
		0.032 4.17 blue
		0.019 8.44 blue
		0.012 4.07 blue
		0.026 4.4 blue
		0.017 6.86 blue
		0.036 6.57 blue
		0.014 4.78 blue
		0.035 9.66 blue
		0.014 4.78 blue
		0.007 2.35 blue
		0.008 2.8400000000000003 blue
		0.012 5.180000000000001 blue
		0.014 4.8500000000000005 blue
		1.841 292.87 blue
		1.651 2.79 blue
		2.039 6.130000000000001 blue
		2.178 3.67 blue
		0.309 2.83 blue
		0.226 2.37 blue
		11.604 24.059999999999995 blue
		20.692 45.33 blue
		0.198 2.49 blue
		1.633 5.9399999999999995 blue
		1.869 3.2 blue
		2.17 3.58 blue
		1.867 3.19 blue
		547.066 827.75 blue
		1.916 3.1900000000000004 blue
		10.491 22.140000000000004 blue
		3.217 59.82 blue
		0.258 5.79 blue
		1.8 12.02 blue
		0.457 101.34 blue
		0.594 96.32000000000001 blue
		0.456 100.9 blue
		8.903 18.67 blue
		0.235 2.87 blue
		1.625 2.84 blue
		2.166 47.92 blue
		7.993 16.26 blue
		0.449 101.27000000000001 blue
		1.877 3.13 blue
		1.873 3.1399999999999997 blue
		1.574 7.300000000000001 blue
		0.194 2.0999999999999996 blue
		382.464 539.67 blue
		0.24 2.83 blue
		0.142 2.25 blue
		0.215 2.73 blue
		0.186 2.58 blue
		0.137 2.25 blue
		0.161 2.41 blue
		0.209 2.6 blue
		0.242 2.88 blue
		0.184 2.58 blue
		0.171 2.48 blue
		0.136 2.25 blue
		0.218 2.74 blue
		0.142 2.33 blue
		0.128 2.18 blue
		0.24 2.7399999999999998 blue
		0.154 2.41 blue
		0.191 2.5900000000000003 blue
		0.156 2.37 blue
		0.167 2.45 blue
		0.204 2.7 blue
		0.237 2.6900000000000004 blue
		0.139 2.23 blue
		0.151 2.39 blue
		0.212 2.72 blue
		0.132 2.28 blue
		0.196 2.5900000000000003 blue
		0.15 2.3 blue
		0.192 2.5100000000000002 blue
		0.206 2.7 blue
		0.19 2.4000000000000004 blue
		0.156 10.66 blue
		0.046 1.73 blue
		0.152 8.83 blue
		0.093 4.27 blue
		0.206 65.59 blue
		0.11 75.11 blue
		0.219 66.17999999999999 blue
		0.004 1.42 blue
		0.012 1.82 blue
		0.013 2.0500000000000003 blue
		0.012 1.92 blue
		0.012 2.0500000000000003 blue
		0.011 1.67 blue
		0.012 1.86 blue
		0.012 2.19 blue
		0.012 2.1300000000000003 blue
		0.011 1.84 blue
		0.011 1.58 blue
		0.012 2.22 blue
		0.012 1.65 blue
		0.011 2.18 blue
		0.012 2.1500000000000004 blue
		0.011 2.0500000000000003 blue
		0.012 1.66 blue
		0.011 1.79 blue
		0.012 1.86 blue
		0.011 1.8 blue
		0.011 1.81 blue
		0.011 2.14 blue
		0.011 1.9999999999999998 blue
		0.011 1.57 blue
		0.012 2.0 blue
		0.011 1.72 blue
		0.011 1.6199999999999999 blue
		0.012 1.8699999999999999 blue
		0.013 2.22 blue
		0.011 1.91 blue
		0.011 1.89 blue
		0.012 1.75 blue
		0.011 1.58 blue
		0.012 1.84 blue
		0.012 1.93 blue
		0.012 1.99 blue
		0.012 1.71 blue
		0.011 1.82 blue
		0.012 1.73 blue
		0.013 2.22 blue
		0.011 1.82 blue
		0.011 1.64 blue
		0.011 1.67 blue
		0.011 1.74 blue
		0.011 2.12 blue
		0.011 1.9 blue
		0.01 1.57 blue
		0.011 1.71 blue
		0.011 1.97 blue
		0.012 1.81 blue
		0.012 1.98 blue
		0.012 1.58 blue
		0.012 2.2300000000000004 blue
		0.012 2.0300000000000002 blue
		0.011 1.6199999999999999 blue
		0.012 1.84 blue
		0.011 1.59 blue
		0.011 1.64 blue
		0.012 1.76 blue
		0.012 2.2 blue
		0.012 2.22 blue
		0.011 1.9 blue
		0.011 1.9999999999999998 blue
		0.011 1.72 blue
		0.011 1.8699999999999999 blue
		0.011 1.98 blue
		0.01 1.71 blue
		0.012 1.92 blue
		0.011 1.91 blue
		0.012 1.84 blue
		0.013 1.71 blue
		0.012 2.2 blue
		0.011 1.81 blue
		0.012 2.0300000000000002 blue
		0.011 1.85 blue
		0.012 1.73 blue
		0.011 1.77 blue
		0.013 2.18 blue
		0.012 1.9999999999999998 blue
		0.011 2.06 blue
		0.01 1.67 blue
		0.011 1.6199999999999999 blue
		0.011 2.1900000000000004 blue
		0.011 1.9 blue
		0.012 2.04 blue
		0.011 1.88 blue
		0.011 1.89 blue
		0.012 2.15 blue
		0.011 1.73 blue
		0.011 1.93 blue
		0.012 1.65 blue
		0.011 1.94 blue
		0.012 2.16 blue
		0.012 1.93 blue
		0.011 1.61 blue
		0.011 1.6199999999999999 blue
		0.01 1.72 blue
		0.012 1.95 blue
		0.011 1.61 blue
		0.011 1.73 blue
		0.013 1.9899999999999998 blue
		0.012 1.98 blue
		0.011 1.63 blue
		0.012 1.67 blue
		0.01 1.69 blue
		0.012 2.03 blue
		0.012 1.6199999999999999 blue
		0.012 2.22 blue
		0.012 1.6 blue
		0.012 1.74 blue
		0.011 2.0100000000000002 blue
		0.011 1.9999999999999998 blue
		0.012 2.0300000000000002 blue
		0.012 1.71 blue
		0.011 1.81 blue
		0.011 1.8 blue
		0.011 1.88 blue
		0.011 2.0300000000000002 blue
		0.011 1.6 blue
		0.011 2.04 blue
		0.013 1.8599999999999999 blue
		0.012 1.9 blue
		0.012 1.9 blue
		0.011 1.72 blue
		0.013 1.57 blue
		0.012 1.85 blue
		0.011 1.6 blue
		0.012 2.1 blue
		0.012 1.85 blue
		0.012 2.06 blue
		0.011 1.88 blue
		0.012 2.02 blue
		0.012 2.24 blue
		0.011 1.6199999999999999 blue
		0.011 1.67 blue
		0.012 1.65 blue
		0.011 2.02 blue
		0.012 1.61 blue
		0.011 2.12 blue
		0.011 1.88 blue
		0.013 1.84 blue
		0.011 2.04 blue
		0.011 1.67 blue
		0.012 1.77 blue
		0.012 2.06 blue
		0.012 2.05 blue
		0.011 1.89 blue
		0.012 1.94 blue
		0.011 1.74 blue
		0.011 2.1700000000000004 blue
		0.013 2.2100000000000004 blue
		0.011 1.64 blue
		0.011 1.93 blue
		0.011 1.8 blue
		0.012 2.16 blue
		0.011 1.72 blue
		0.01 1.75 blue
		0.012 1.92 blue
		0.012 1.82 blue
		0.013 1.65 blue
		0.011 1.82 blue
		0.011 1.83 blue
		0.012 2.16 blue
		0.011 2.12 blue
		0.011 1.83 blue
		0.011 2.02 blue
		0.011 1.63 blue
		0.011 1.6199999999999999 blue
		0.011 1.6 blue
		0.012 2.17 blue
		0.012 1.76 blue
		0.011 1.9 blue
		0.011 1.57 blue
		0.012 2.22 blue
		0.012 2.16 blue
		0.012 1.92 blue
		0.011 2.0100000000000002 blue
		0.012 2.1900000000000004 blue
		0.011 1.83 blue
		0.013 1.75 blue
		0.011 1.68 blue
		0.044 12.760000000000002 blue
		0.017 5.37 blue
		0.009 1.3699999999999999 blue
		0.011 1.52 blue
		0.011 1.7 blue
		0.044 12.629999999999999 blue
		0.021 5.91 blue
		0.021 6.220000000000001 blue
		0.039 11.58 blue
		};
		\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\begin{minipage}[t]{.05\linewidth}
		\ 
	\end{minipage}
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
		\begin{axis}[
		scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
		ylabel=\veripb (time in seconds),
		xlabel=\papilo (time in seconds),
		xmode=log,
		ymode=log,
		grid=both,
		grid style={line width=.1pt, draw=gray!10},
		major grid style={line width=.2pt,draw=gray!50},
		minor tick num=5,
		xtick={0.01,0.1,1,10,100,1000},
		ytick={0.01,0.1,1,10,100,1000,10000},
		]
		\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x});
		\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x + 10});
		\addplot[scatter,only marks, scatter src=explicit symbolic]%
		table[meta=label] {
			x y label
			1000 1000 peer
			0.146 34.11 green
			0.046 10.56 green
			0.091 47.99 green
			3.98 2.15 green
			7.495 8372.310000000001 green
			0.616 2094.58 green
			1.147 3.86 green
			5.324 1942.23 green
			0.027 27.380000000000003 green
			0.203 116.2 green
			10.054 153.29 green
			0.018 6.4399999999999995 green
			1.192 47.099999999999994 green
			0.137 22.29 green
			0.037 14.83 green
			0.113 5.48 green
			2.705 8.49 green
			1.218 1966.6000000000001 green
			1.816 193.01 green
			0.027 51.93 green
			0.138 81.47 green
			0.036 7.06 green
			0.072 1.28 green
			0.554 37.199999999999996 green
			0.052 13.32 green
			0.018 2.27 green
			0.279 6.51 green
			0.623 140.26999999999998 green
			0.066 3.45 green
			1.696 3.3000000000000003 green
			11.227 2104.3300000000004 green
			0.256 117.19 green
			1.028 726.36 green
			0.009 3.3800000000000003 green
			9.253 2358.98 green
			0.38 42.29 green
			0.034 1.9899999999999998 green
			0.229 36.07 green
			0.507 1.06 green
			0.705 22.540000000000003 green
			0.444 29.84 green
			1.167 4087.21 green
			0.255 194.31 green
			0.432 133.09 green
			4.257 1.35 green
			0.067 4.89 green
			0.389 408.48999999999995 green
			4.288 3533.3500000000004 green
			0.271 578.04 green
			1.113 106.58 green
			0.365 14.17 green
			0.062 1.28 green
			0.004 3.99 green
			0.017 37.48 green
			0.153 2.0 green
			0.007 23.2 blue
			0.048 46.46 blue
			0.349 253.9 blue
			0.068 4.84 blue
			1.519 1.3 blue
			0.126 71.61 blue
			0.021 2.5 blue
			0.302 99.78999999999999 blue
			0.003 2.18 blue
			1.485 2104.29 blue
			0.309 2548.8199999999997 blue
			0.168 2.0100000000000002 blue
			2.851 2945.7000000000003 blue
			0.009 3.56 blue
			0.017 37.699999999999996 blue
			0.022 2.85 blue
			0.309 10.88 blue
			0.004 3.52 blue
			0.028 1.3599999999999999 blue
			0.229 35.81 blue
			2.845 2970.08 blue
			0.584 119.0 blue
			0.095 52.01 blue
			1.492 2097.74 blue
			0.096 52.48 blue
			0.049 46.66 blue
			2.498 8.48 blue
			0.134 33.62 blue
			5.02 4385.97 blue
			0.018 6.91 blue
			0.042 28.34 blue
			0.023 3.66 blue
			10.217 150.37 blue
			0.511 162.20000000000002 blue
			0.163 112.34 blue
			0.676 124.38 blue
			0.709 22.11 blue
			0.286 532.91 blue
			0.006 3.8200000000000003 blue
			0.299 10.92 blue
			0.046 181.37 blue
			0.038 15.79 blue
			0.006 3.8200000000000003 blue
			1.108 105.86 blue
			0.059 3.4000000000000004 blue
			0.509 160.9 blue
			0.059 3.91 blue
			1.086 105.59 blue
			0.315 2552.48 blue
			0.06 3.39 blue
			4.02 2.19 blue
			0.009 3.6 blue
			0.382 42.25 blue
			5.325 8491.69 blue
			0.143 112.64 blue
			0.134 71.98 blue
			0.149 2.0 blue
			0.095 2.15 blue
			0.051 1.27 blue
			1.541 1.31 blue
			66.524 606.9300000000001 blue
			0.038 15.809999999999999 blue
			1.095 3.87 blue
			0.801 44.21 blue
			1.11 3.86 blue
			5.378 8462.77 blue
			0.029 1.98 blue
			0.043 4.9799999999999995 blue
			0.01 1.22 blue
			0.678 124.2 blue
			0.115 5.3500000000000005 blue
			0.352 255.34 blue
			0.007 23.36 blue
			0.288 530.83 blue
			0.589 119.86 blue
			0.028 1.9899999999999998 blue
			0.199 125.76 blue
			0.042 28.23 blue
			0.231 36.07 blue
			0.897 886.9599999999999 blue
			0.152 1.9900000000000002 blue
			0.092 10.13 blue
			0.163 78.86 blue
			0.021 2.86 blue
			0.895 877.3499999999999 blue
			0.296 97.86999999999999 blue
			0.017 1.49 blue
			0.125 71.16 blue
			0.003 2.18 blue
			0.709 22.15 blue
			0.029 8179.29 blue
			7.315 4356.2300000000005 blue
			2.499 8.41 blue
			0.067 4.84 blue
			0.014 3.5300000000000002 blue
			7.29 4351.83 blue
			0.114 5.33 blue
			0.011 1.09 blue
			0.198 125.94 blue
			4.989 4367.419999999999 blue
			0.018 2.2600000000000002 blue
			0.018 6.87 blue
			0.017 2.08 blue
			0.845 39.19 blue
			0.542 1.06 blue
			0.004 3.4800000000000004 blue
			0.047 181.42 blue
			0.03 8214.94 blue
			
		};
		\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\caption{
		Running times of \veripb vs. \papilo on test sets \pb (left) and \miplib (right), including all instances with more than 1~seconds in \veripb{} and less than 30~minutes in \papilo, and excluding timeouts.
		Green $+$ signs mark optimization and blue $\times$ signs mark decision instances.
	}
	\label{fig::experiment::PaPILOVeriPB_obju_diff}
\end{figure}


\begin{table}[ht]
	\centering
	\small
	\begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}lrrrrr}
		\toprule
		& &  \multicolumn{2}{c}{RUP} & \multicolumn{2}{c}{POL} &  \\[-0.5ex] 
		\cmidrule{3-4}
		\cmidrule{5-6}
		& size &  verified & time (in s) & verified & time (in s) & relative \\[-0.5ex] 
		\midrule
		\pb-dec & 284 & 284 & 2.21 & 284 & 2.14 &  0.97\\[-0.5ex]
		\miplib-dec & 35 & 31 & 153.23 & 31 & 148.88 &  0.97\\[-0.5ex]
		\pb-opt & 153 & 142 & 28.43 & 142 & 28.22 &  0.99\\[-0.5ex]
		\miplib-opt & 16 & 14 & 147.11 & 14 & 127.83 &  0.87\\[-0.5ex]
		\bottomrule
	\end{tabular*}
	\caption{Comparison of the runtime (in seconds) of \veripb with POL and RUP for instances with at least 10 propagations.}
	\label{tab:rup_vs_add_obju_add}
\end{table}


==> sections/unused_graphics.tex <==
\section{Unused Figures and Tables}\label{sec:unused-figures-and-tables}


\begin{figure}[ht]
	\centering
	\begin{tikzpicture}[scale=0.6, transform shape]
	\begin{axis}[
	scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
	ylabel=\veripb with RUP,	
	xlabel=\veripb with POL,
	xmode=log,
	ymode=log,
	grid=both,
	grid style={line width=.1pt, draw=gray!10},
	major grid style={line width=.2pt,draw=gray!50},
	minor tick num=5,
	xtick={0.01,0.1,1,10,100,1000,10000, 100000, 1000000, 10000000},
	ytick={0.01,0.1,1,10,100,1000,10000, 100000, 1000000, 10000000},
	]
	\addplot[scatter,only marks, scatter src=explicit symbolic]
	table[meta=label] {
		x y label
		34.28 18.27 green
		40.14 40.19 green
		32.54 17.91 green
		36.45 36.28 green
		35.34 19.11 green
		38.55 37.46 green
		34.75 34.89 green
		36.56 37.07 green
		44.74 44.74 green
		24.52 44.36 green
		22.22 10.76 green
		42.24 42.3 green
		48.73 26.66 green
		45.85 45.43 green
		28.6 52.29 green
		43.41 23.91 green
		2.64 2.63 green
		1354.84 1527.51 green
		248.4 129.21 green
		13.34 14.05 green
		0.31 0.31 green
		71.69 72.43 green
		1.07 1.12 green
		3.93 4.08 green
		2300.34 2298.5 green
		209.22 214.61 green
		0.23 0.23 green
		0.08 0.08 green
		0.13 0.13 green
		0.27 0.21 green
		0.15 0.14 green
		0.13 0.14 green
		0.07 0.05 green
		0.12 0.12 green
		0.14 0.14 green
		0.16 0.1 green
		0.08 0.07 green
		0.13 0.13 green
		0.13 0.11 green
		0.09 0.1 green
		0.16 0.16 green
		0.14 0.13 green
		0.09 0.09 green
		0.13 0.08 green
		0.17 0.17 green
		0.13 0.08 green
		0.08 0.07 green
		0.07 0.08 green
		0.26 0.26 green
		0.08 0.08 green
		0.29 0.21 green
		0.12 0.12 green
		0.13 0.13 green
		0.1 0.1 green
		0.16 0.17 green
		0.13 0.13 green
		0.29 0.29 green
		0.17 0.17 green
		0.1 0.1 green
		0.15 0.11 green
		0.07 0.07 green
		0.23 0.24 green
		0.13 0.09 green
		0.09 0.09 green
		0.13 0.12 green
		0.07 0.07 green
		0.1 0.1 green
		0.13 0.13 green
		0.13 0.1 green
		0.31 0.29 green
		0.11 0.11 green
		0.1 0.1 green
		0.12 0.08 green
		0.11 0.1 green
		0.24 0.24 green
		0.23 0.24 green
		0.08 0.08 green
		0.13 0.13 green
		0.11 0.07 green
		0.14 0.14 green
		0.12 0.12 green
		0.28 0.2 green
		1.16 1.46 green
		1.02 0.78 green
		1.16 1.45 green
		0.56 0.43 green
		0.31 0.23 green
		0.51 0.49 green
		0.32 0.37 green
		0.32 0.37 green
		3.41 2.92 green
		22.99 19.9 green
		18.6 16.02 green
		9.0 7.89 green
		4837.91 4814.8 green
		7442.4 7445.62 green
		364.93 641.26 green
		3723.57 3729.23 green
		634.75 352.17 green
		4813.52 4815.52 green
		278.46 144.32 green
		280.7 277.67 green
		176.12 176.89 green
		81.61 81.35 green
		277.65 283.45 green
		3740.56 3749.83 green
		3711.83 1428.55 green
		280.56 278.28 green
		3706.53 3706.71 green
		276.63 280.13 green
		280.49 276.9 green
		633.73 631.25 green
		360.34 637.05 green
		1450.31 3742.11 green
		2556.14 959.92 green
		174.46 173.88 green
		81.68 81.75 green
		81.55 80.13 green
		2560.18 2565.32 green
		3708.86 3730.2 green
		2559.79 2557.03 green
		7367.03 7381.86 green
		4832.74 4818.47 green
		635.22 369.38 green
		18888.55 18885.32 green
		18820.97 18881.86 green
		9227.12 9257.0 green
		18820.84 18869.0 green
		9228.85 9250.73 green
		18843.08 18769.03 green
		9217.42 9170.24 green
		18819.48 11832.59 green
		9194.5 9225.25 green
		18877.98 18916.64 green
		1096.12 1135.57 green
		9163.78 5620.93 green
		9236.06 9206.55 green
		9218.84 9208.21 green
		9170.76 9214.4 green
		11341.46 18852.15 green
		9239.01 9224.04 green
		18823.59 18873.35 green
		9222.8 9231.01 green
		35.86 37.36 blue
		32.63 31.12 blue
		33.79 34.43 blue
		43.14 45.06 blue
		40.86 40.66 blue
		33.39 32.93 blue
		93.69 96.14 blue
		164.25 158.87 blue
		171.06 181.34 blue
		99.27 97.47 blue
		146.82 147.0 blue
		104.35 104.61 blue
		96.92 96.44 blue
		56.82 57.69 blue
		76.6 58.36 blue
		10.0 7.25 blue
		9.27 6.84 blue
		15.27 15.67 blue
		9.88 9.75 blue
		11.42 11.53 blue
		12.89 12.84 blue
		15.27 15.28 blue
		0.37 0.36 blue
		4.65 5.07 blue
		11.11 10.66 blue
		21.64 21.19 blue
		25.78 25.3 blue
		4.77 5.02 blue
		3.76 3.99 blue
		3.5 3.59 blue
		4.83 4.88 blue
		4.54 4.76 blue
		4.58 4.75 blue
		4.39 4.56 blue
		3.88 3.98 blue
		4.35 4.52 blue
		3.71 3.7 blue
		3.74 3.83 blue
		3.97 4.09 blue
		4.34 4.51 blue
		3.46 3.53 blue
		3.48 3.53 blue
		3.9 4.01 blue
		3.52 3.56 blue
		4.72 5.05 blue
		4.17 4.04 blue
		3.82 3.86 blue
		4.61 4.53 blue
		4.84 4.95 blue
		3.48 3.51 blue
		4.21 4.33 blue
		4.29 4.43 blue
		3.77 3.85 blue
		3.81 3.88 blue
		3.49 3.52 blue
		4.1 4.3 blue
		4.51 4.42 blue
		4.04 4.17 blue
		3.51 3.58 blue
		4.62 4.8 blue
		4.04 4.39 blue
		4.08 4.4 blue
		3.61 3.67 blue
		3.64 3.87 blue
		4.09 4.02 blue
		3.69 3.73 blue
		3.79 3.92 blue
		4.81 4.9 blue
		4.38 3.14 blue
		4.27 2.97 blue
		3.53 2.53 blue
		4.36 3.11 blue
		3.57 2.75 blue
		4.61 4.8 blue
		4.15 2.94 blue
		4.62 3.36 blue
		3.6 3.68 blue
		3.46 2.52 blue
		4.71 4.93 blue
		4.05 2.94 blue
		4.12 3.05 blue
		4.17 4.31 blue
		4.81 3.49 blue
		4.23 4.47 blue
		4.49 3.13 blue
		4.41 4.77 blue
		3.95 2.85 blue
		4.41 3.22 blue
		4.0 4.09 blue
		4.35 3.12 blue
		3.77 3.86 blue
		4.31 3.1 blue
		3.98 4.22 blue
		4.43 3.19 blue
		3.76 2.82 blue
		4.18 4.14 blue
		4.4 3.13 blue
		3.94 4.06 blue
		3.75 2.79 blue
		3.98 4.11 blue
		3.57 2.63 blue
		3.55 2.57 blue
		3.98 4.08 blue
		3.58 2.6 blue
		4.36 4.29 blue
		4.52 3.12 blue
		4.42 3.21 blue
		3.97 4.11 blue
		3.97 2.93 blue
		4.66 4.83 blue
		4.04 3.0 blue
		3.46 2.51 blue
		3.97 4.13 blue
		3.52 2.56 blue
		4.35 4.51 blue
		3.85 2.81 blue
		4.64 3.2 blue
		4.09 4.26 blue
		3.72 2.72 blue
		4.11 4.2 blue
		4.81 3.44 blue
		4.62 3.27 blue
		3.69 3.77 blue
		4.3 3.03 blue
		3.46 3.49 blue
		3.46 2.49 blue
		3.83 3.98 blue
		4.67 3.37 blue
		4.28 4.25 blue
		3.7 2.68 blue
		4.33 3.34 blue
		4.74 4.92 blue
		3.51 2.57 blue
		4.82 4.99 blue
		4.58 3.32 blue
		4.54 3.29 blue
		4.77 5.01 blue
		4.06 3.14 blue
		3.66 3.95 blue
		4.16 3.0 blue
		4.4 3.18 blue
		4.66 4.92 blue
		4.29 3.04 blue
		3.61 3.67 blue
		4.51 3.13 blue
		3.76 3.84 blue
		3.76 2.84 blue
		4.04 3.18 blue
		4.48 4.64 blue
		3.75 2.75 blue
		3.65 3.77 blue
		3.71 2.78 blue
		4.09 4.06 blue
		4.69 3.41 blue
		3.66 2.68 blue
		3.87 3.98 blue
		3.86 2.73 blue
		4.02 4.14 blue
		3.61 2.81 blue
		4.64 3.35 blue
		3.53 3.61 blue
		4.8 3.38 blue
		3.83 3.92 blue
		3.82 2.74 blue
		4.14 4.25 blue
		3.56 2.55 blue
		4.77 4.89 blue
		3.59 2.77 blue
		3.96 2.86 blue
		4.12 4.14 blue
		4.75 3.4 blue
		3.77 3.88 blue
		3.76 2.79 blue
		4.28 3.06 blue
		4.38 4.59 blue
		4.18 3.02 blue
		4.28 4.26 blue
		4.26 3.12 blue
		4.75 4.95 blue
		4.04 2.88 blue
		3.92 2.93 blue
		4.03 4.19 blue
		3.9 2.91 blue
		3.81 2.75 blue
		4.68 4.92 blue
		4.2 3.03 blue
		3.66 3.75 blue
		4.29 2.92 blue
		3.73 3.98 blue
		4.3 3.11 blue
		3.85 2.8 blue
		3.53 3.55 blue
		4.56 3.17 blue
		3.59 3.71 blue
		4.77 3.44 blue
		3.96 4.13 blue
		4.34 3.12 blue
		3.58 3.63 blue
		4.3 4.44 blue
		3.72 3.59 blue
		3.98 4.05 blue
		4.05 4.22 blue
		4.63 3.35 blue
		3.79 2.72 blue
		4.01 4.16 blue
		4.39 3.12 blue
		3.92 4.07 blue
		0.31 0.32 blue
		1.9 1.95 blue
		1.91 1.97 blue
		1.93 1.98 blue
		1.87 1.91 blue
		2.08 2.14 blue
		2.0 1.98 blue
		1.92 2.03 blue
		1.9 1.95 blue
		1.99 2.09 blue
		1.9 1.97 blue
		1.91 2.0 blue
		1.93 1.99 blue
		1.95 2.02 blue
		1.95 2.01 blue
		1.92 1.97 blue
		1.9 2.02 blue
		1.83 1.81 blue
		1.83 1.87 blue
		1.85 1.87 blue
		1.85 1.88 blue
		1.75 1.78 blue
		1.89 1.91 blue
		1.75 1.76 blue
		1.85 1.87 blue
		1.8 1.8 blue
		1.77 1.81 blue
		1.97 1.99 blue
		1.85 1.86 blue
		2.03 2.07 blue
		1.77 1.8 blue
		1.76 1.8 blue
		1.76 1.79 blue
		1.76 1.81 blue
		1.87 1.91 blue
		1.87 1.89 blue
		1.77 1.81 blue
		1.93 1.97 blue
		1.84 1.89 blue
		1.86 1.9 blue
		1.78 1.8 blue
		1.88 1.92 blue
		1.97 1.99 blue
		1.87 1.9 blue
		2.0 2.0 blue
		1.91 2.0 blue
		1.99 2.01 blue
		4.86 5.13 blue
		5.62 6.17 blue
		6.14 6.79 blue
		4.89 5.14 blue
		5.0 5.32 blue
		5.59 5.96 blue
		5.5 5.9 blue
		5.82 6.24 blue
		5.3 5.61 blue
		5.58 5.8 blue
		4.86 5.19 blue
		5.72 6.1 blue
		5.83 6.31 blue
		5.04 5.46 blue
		5.69 6.36 blue
		5.56 5.94 blue
		4.9 5.3 blue
		5.21 5.58 blue
		5.34 5.79 blue
		5.31 5.64 blue
		5.89 6.33 blue
		6.26 6.62 blue
		5.7 6.24 blue
		5.3 3.21 blue
		5.2 5.58 blue
		5.72 6.07 blue
		5.22 3.14 blue
		5.96 6.4 blue
		5.8 6.23 blue
		4.8 5.12 blue
		664.3 646.82 green
		0.85 0.85 green
		0.49 0.5 green
		7343.43 7944.41 green
		9467.85 9505.71 green
		74.52 44.22 green
		748.39 759.95 green
		1216.94 970.28 green
		153.16 159.51 green
		5010.67 5015.6 green
		2.16 2.18 green
		145.46 142.89 green
		765.18 747.83 green
		16962.58 17065.89 green
		168.34 101.69 blue
		4741.04 4724.13 blue
		4752.37 1740.9 blue
		1214.31 790.86 blue
		15662.06 15674.05 blue
		2.25 2.21 blue
		8805.11 8841.39 blue
		153.17 159.77 blue
		8633.17 9192.68 blue
		128.52 228.18 blue
		166.89 180.19 blue
		4242.84 1533.57 blue
		1256.56 2726.85 blue
		1.71 1.79 blue
		4731.45 4721.34 blue
		1.61 2.44 blue
		169.35 101.13 blue
		1.41 1.4 blue
		2907.4 1043.5 blue
		1251.42 2702.61 blue
		1.06 1.07 blue
		8801.0 8843.46 blue
		167.27 179.45 blue
		682.53 778.74 blue
		8623.02 9191.97 blue
		691.29 686.98 blue
		16.39 10.04 blue
		1.38 1.41 blue
		1.06 1.07 blue
		690.24 683.22 blue
		72.77 78.45 blue
		139.84 146.23 blue
		679.58 778.76 blue
		16.48 9.85 blue
		3027.62 2986.25 blue
		10187.3 15618.29 blue
	};
	\end{axis}
	\end{tikzpicture}
	\caption{
		Comparison of verifying the propagation with RUP or POL for instances with at least 10 reductions found by \boundstren.
		Each $\times$ marks an instance.
		The $x$-axis gives the time for verifying with RUP and the $y$-axis gives the time for verifying with POL.
		Green $+$ mark optimization instances and blue $\times$ mark decision instances.
	}
	\label{fig:add_vs_rup}
\end{figure}


% FIXME: transactions costs can be negative which is not handle by log scale
\begin{figure}[ht]
	\centering
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
		\begin{axis}[
		scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
		ylabel=Overhead per transaction,
		xlabel=Reductions+model-clean-up,
		xmin=-0.1,
		ymin=-0.1,
		xmode=log,
		ymode=log,
		grid=both,
		grid style={line width=.1pt, draw=gray!10},
		major grid style={line width=.2pt,draw=gray!50},
		minor tick num=5,
		xtick={1,10,100,1000,10000, 100000, 1000000, 10000000, 100000000},
		ytick={0,0.1,0.01,0.001,0.0001, 0.00001, 0.000001, 0.0000001, 0.00000001, 0.000000001},
		]
		\addplot[domain=1:100000000, pbred] {0.0001662686567164177};
		\addplot[scatter,only marks, scatter src=explicit symbolic]
		table[meta=label] {
			x y label
			15000000 0.2 peer
			15000000 0.0000001 peer
			1396 1.862464183381089e-05 green
			697 9.899569583931132e-05 green
			705 1.843971631205674e-05 green
			1816 2.588105726872247e-05 green
			1902 4.837013669821241e-05 green
			10 0.0002 green
			58 3.4482758620689657e-05 green
			669 2.541106128550075e-05 green
			4484 0.00021074933095450491 green
			5064 0.0002010268562401264 green
			4501 8.087091757387248e-05 green
			4527 0.00018776231499889552 green
			4822 8.855246785566155e-05 green
			4432 0.0002048736462093863 green
			5429 0.00023908638791674339 green
			4916 0.00020077298616761596 green
			4778 8.267057346169945e-05 green
			4723 0.00020008469193309337 green
			4808 8.19467554076539e-05 green
			4788 0.0001954887218045113 green
			4992 0.0001979166666666667 green
			5115 0.000233822091886608 green
			4954 7.973354864755754e-05 green
			4840 0.0002239669421487603 green
			4839 8.782806364951436e-05 green
			5105 0.00022115572967678748 green
			4666 0.00021710244320617233 green
			4742 7.908055672711936e-05 green
			4758 0.00020407734342160568 green
			4917 0.00022371364653243846 green
			5088 8.706761006289308e-05 green
			4849 0.00021612703650237164 green
			5593 0.0002435186840693724 green
			5858 0.00023062478661659268 green
			2682 9.955257270693512e-05 green
			5552 0.0002379322766570605 green
			2809 0.00011391954432182271 green
			5441 0.00022900202168718985 green
			4289 7.274422942410819e-05 green
			2458 9.804719283970708e-05 green
			5171 0.00019996132276155483 green
			5758 0.00010177144841959015 green
			5450 0.00025944954128440367 green
			5947 0.0002661846309063393 green
			5058 0.00010083036773428232 green
			5096 0.00022664835164835166 green
			22 4.545454545454546e-05 green
			96 2.0833333333333333e-05 green
			11005 3.034984098137209e-05 green
			10442 1.6280406052480383e-05 green
			11838 2.6524750802500428e-05 green
			11985 3.045473508552357e-05 green
			13078 3.410307386450525e-05 green
			10319 1.7055916270956493e-05 green
			13235 3.845863241405366e-05 green
			10689 2.703714098606045e-05 green
			12967 3.686280558340404e-05 green
			12944 1.4215080346106316e-05 green
			12309 3.8427167113494195e-05 green
			13367 3.785441759557118e-05 green
			10808 1.7579570688378985e-05 green
			10677 2.7535824669851084e-05 green
			13669 3.065330309459361e-05 green
			10604 2.036967182195399e-05 green
			13631 1.9734428875357633e-05 green
			13351 3.2057523780990214e-05 green
			14274 2.487039372285274e-05 green
			13378 3.4011062939153824e-05 green
			12350 3.287449392712548e-05 green
			10788 1.2699295513533557e-05 green
			10929 3.669137158019947e-05 green
			11804 3.6089461199593354e-05 green
			10986 2.3939559439286375e-05 green
			12243 1.4457240872335216e-05 green
			10788 2.576937337782722e-05 green
			13181 3.4898717851452845e-05 green
			11128 3.801222142343638e-05 green
			10815 3.698566805362922e-05 green
			12947 2.0931489920444884e-05 green
			10805 3.294770939379916e-05 green
			10984 3.304806991988347e-05 green
			12362 2.9768645850186046e-05 green
			12213 6.714157045770888e-06 green
			11992 3.8609072715143425e-05 green
			10689 2.497895032276173e-05 green
			11842 2.3982435399425757e-05 green
			10963 3.429718142844111e-05 green
			10732 3.0376444278792404e-05 green
			13475 1.766233766233766e-05 green
			11901 3.319048819426939e-05 green
			13164 2.9626253418413865e-05 green
			11479 1.9949472950605442e-05 green
			13212 3.436270057523462e-05 green
			13329 5.626828719333797e-06 green
			11525 3.0368763557483718e-05 green
			12262 3.9716196379057246e-05 green
			13312 2.0357572115384624e-05 green
			10451 2.9279494785188016e-05 green
			12024 3.4098469727212237e-05 green
			12638 4.597246399746795e-05 green
			10932 2.671057446030004e-05 green
			11787 3.792313565792823e-05 green
			10598 1.3304397056048312e-05 green
			2845 2.460456942003515e-05 green
			3237 1.637318504788384e-05 green
			2782 1.976994967649173e-05 green
			2648 1.0951661631419928e-05 green
			3089 7.76950469407576e-06 green
			3468 2.0472895040369073e-05 green
			3445 1.4513788098693755e-05 green
			3599 1.2225618227285353e-05 green
			3462 1.9930675909878686e-05 green
			3966 2.1432173474533526e-05 green
			2506 1.1971268954509166e-05 green
			3334 1.6196760647870424e-05 green
			3109 1.6082341588935346e-05 green
			2692 1.3001485884101032e-05 green
			2703 1.8497965223825386e-05 green
			2372 2.9510961214165287e-06 green
			2909 8.937779305603308e-06 green
			2972 1.3458950201884265e-05 green
			3506 1.1123787792355955e-05 green
			3109 1.4795754261820516e-05 green
			2461 1.2190166598943518e-05 green
			2973 1.3454423141607797e-05 green
			3133 2.234280242578998e-05 green
			3206 2.1210230817217717e-05 green
			2689 1.7478616586091478e-05 green
			3399 9.708737864077678e-06 green
			2995 1.5692821368948244e-05 green
			3329 2.0126164013217182e-05 green
			2620 2.061068702290076e-05 green
			9044 3.217602830605927e-05 green
			9782 2.647720302596605e-05 green
			9883 1.8719012445613684e-05 green
			9238 4.286642130331239e-05 green
			9998 2.0004000800160028e-05 green
			8983 3.261716575754203e-05 green
			8321 2.8962865040259582e-05 green
			8994 2.5239048254391826e-05 green
			9279 3.1253367819808174e-05 green
			9178 2.8982349095663545e-05 green
			10112 3.490901898734177e-05 green
			8903 3.448275862068965e-05 green
			9974 3.248445959494685e-05 green
			9791 3.748340312531917e-05 green
			9108 2.5581906016688612e-05 green
			7688 3.420915712799168e-05 green
			9081 3.9202730976764675e-05 green
			9317 2.618868734571214e-05 green
			8108 2.1830291070547584e-05 green
			7858 3.168745227793331e-05 green
			8173 1.6395448427749897e-05 green
			8009 2.6969659133474837e-05 green
			9460 2.44186046511628e-05 green
			9942 2.3033594850130766e-05 green
			10149 2.3056458764410284e-05 green
			8239 2.342517295788323e-05 green
			9966 2.879791290387316e-05 green
			9592 2.55421184320267e-05 green
			9668 2.482416218452627e-05 green
			7607 3.483633495464704e-05 green
			8408 2.7235965746907706e-05 green
			7921 3.1814164878171944e-05 green
			5498 2.655511094943616e-05 green
			5401 2.758748379929642e-05 green
			5341 1.3480621606440754e-05 green
			5659 1.4843611945573416e-05 green
			5829 2.3331617773202952e-05 green
			6264 2.4106002554278403e-05 green
			5648 2.0007082152974504e-05 green
			6320 2.674050632911393e-05 green
			5641 3.261833008331856e-05 green
			5245 2.2116301239275498e-05 green
			6650 3.383458646616541e-05 green
			6785 1.5475313190862194e-05 green
			6032 2.2214854111405836e-05 green
			6320 3.1329113924050645e-05 green
			5172 1.9528228924980684e-05 green
			6564 3.09262644728824e-05 green
			5567 3.197413328543202e-05 green
			5507 1.2711094970037943e-06 green
			6788 3.786093105480259e-05 green
			5969 1.725582174568604e-05 green
			5784 2.662517289073306e-05 green
			6241 2.78801474122737e-05 green
			6631 2.880410194540794e-05 green
			261 0.0 green
			305 0.00035737704918032786 green
			16198 0.0004614767255216693 green
			9880 -3.0364372469635653e-07 green
			1344 0.0013058035714285713 green
			7615 3.9395929087327644e-06 green
			12261 6.280075034662752e-06 green
			272 0.00034926470588235296 green
			6846 0.0003032427695004382 green
			4192 2.7671755725190865e-05 green
			35 8.57142857142858e-05 green
			2784 6.824712643678162e-06 green
			11173 4.5735254631701414e-05 green
			4553 1.5374478365912576e-06 green
			9 -0.00044444444444444447 green
			39 5.128205128205133e-05 green
			5381 7.991079724958193e-06 green
			36 0.00011111111111111112 green
			274 -4.7445255474452544e-05 green
			4 -0.0005 green
			135480 0.0491474756421612 green
			60 1.666666666666668e-05 green
			5261 2.471013115377305e-06 green
			1693 0.0012575310100413468 green
			15453 0.0014355788520028475 green
			9516 2.0491803278688525e-05 green
			62329 3.288998700444417e-06 green
			3528 0.003586451247165533 green
			152 2.6315789473684212e-05 green
			21 0.00019047619047619048 green
			41 9.75609756097561e-05 green
			98 7.142857142857143e-05 green
			56 5.3571428571428575e-05 green
			76 1.3157894736842106e-05 green
			25 8e-05 green
			37 8.108108108108108e-05 green
			48 0.00010416666666666667 green
			52 0.00011538461538461537 green
			22 0.00040909090909090913 green
			82 3.6585365853658535e-05 green
			72 5.555555555555556e-05 green
			30 0.0001 green
			49 0.00012244897959183673 green
			82 2.4390243902439026e-05 green
			28 7.142857142857143e-05 green
			45 0.00011111111111111112 green
			61 9.836065573770493e-05 green
			36 -0.0006666666666666666 green
			23 8.695652173913044e-05 green
			21 9.523809523809524e-05 green
			90 3.3333333333333335e-05 green
			25 0.0005600000000000001 green
			29 6.896551724137931e-05 green
			77 7.792207792207792e-05 green
			100 2e-05 green
			66 3.0303030303030302e-05 green
			30 0.0002666666666666667 green
			56 7.142857142857143e-05 green
			21 0.00019047619047619048 green
			92 3.260869565217392e-05 green
			97 4.1237113402061855e-05 green
			54 7.407407407407407e-05 green
			30 0.0001 green
			59 6.779661016949152e-05 green
			24 0.000125 green
			134 2.9850746268656717e-05 green
			87 5.747126436781609e-05 green
			27 0.0 green
			94 2.1276595744680852e-05 green
			23 0.00013043478260869567 green
			36 5.555555555555556e-05 green
			45 6.666666666666667e-05 green
			74 4.054054054054054e-05 green
			77 5.194805194805195e-05 green
			22 9.090909090909092e-05 green
			36 5.555555555555556e-05 green
			31 6.451612903225807e-05 green
			47 0.0004893617021276595 green
			43 6.976744186046511e-05 green
			76 0.00014473684210526314 green
			135 3.7037037037037037e-05 green
			28 7.142857142857143e-05 green
			51 7.843137254901961e-05 green
			33 0.00018181818181818183 green
			39 2.5641025641025643e-05 green
			21 9.523809523809524e-05 green
			36 8.333333333333333e-05 green
			95 0.000431578947368421 green
			2565 3.898635477582847e-06 green
			2649 1.5100037750094363e-06 green
			2649 -4.907512268780674e-06 green
			2649 2.6425066062665153e-06 green
			2565 -3.898635477582847e-06 green
			2565 5.068226120857699e-06 green
			2565 7.407407407407408e-06 green
			2649 1.887504718761796e-06 green
			2649 1.1325028312570791e-06 green
			2649 4.530011325028311e-06 green
			2649 9.060022650056626e-06 green
			2649 1.5100037750094363e-06 green
			2649 3.7750094375235944e-06 green
			2649 2.6425066062665153e-06 green
			2649 3.7750094375235944e-06 green
			2565 7.79727095516569e-06 green
			2649 -4.152510381275954e-06 green
			242 4.132231404958678e-06 green
			4050 2.2222222222222225e-06 green
			730 -1.3698630136986313e-06 green
			6547 1.8329005651443415e-06 green
			242 4.132231404958678e-06 green
			4062 1.969473165928115e-06 green
			730 -4.109589041095889e-06 green
			4062 -2.4618414574101416e-06 green
			730 -6.849315068493152e-06 green
			22 4.545454545454546e-05 green
			3082 -1.2978585334198572e-06 green
			242 8.264462809917356e-06 green
			3082 -6.489292667099292e-07 green
			1142 2.6269702276707553e-06 green
			2302 -2.6064291920069513e-06 green
			2282 0.0 green
			4050 1.7283950617283954e-06 green
			242 2.4793388429752075e-05 green
			2282 7.887817703768623e-06 green
			730 -8.219178082191783e-06 green
			242 4.132231404958678e-06 green
			5458 1.6489556614144378e-06 green
			730 -2.7397260273972607e-05 green
			242 8.264462809917352e-06 green
			242 0.0 green
			730 1.3698630136986302e-06 green
			842 8.313539192399049e-06 green
			666 -1.9519519519519517e-05 green
			746 4.021447721179619e-06 green
			841 9.512485136741975e-06 green
			723 1.7980636237897654e-05 green
			630 -2.063492063492063e-05 green
			175 3.428571428571428e-05 green
			560 1.7857142857142874e-06 green
			410 2.4390243902439044e-06 green
			99 0.00011111111111111112 green
			173 -7.514450867052021e-05 green
			326 6.13496932515338e-06 green
			375 7.999999999999998e-06 green
			279 -3.584229390681007e-06 green
			450 6.666666666666665e-06 green
			430 0.0 green
			321 3.115264797507791e-06 green
			432 2.314814814814809e-06 green
			760 9.210526315789472e-06 green
			2168 4.612546125461258e-06 green
			1974 -4.0526849037487375e-06 green
			1339 8.215085884988805e-06 green
			204298 5.99124807878687e-06 green
			366221 5.8325437372515495e-06 green
			186045 2.7627724475261364e-06 green
			365536 5.651974087367591e-06 green
			374099 5.773872691453331e-06 green
			385274 5.865955138420968e-06 green
			415713 5.7058595713869906e-06 green
			197649 5.894287347773073e-06 green
			395761 5.710517206091555e-06 green
			363822 5.881997240408772e-06 green
			413026 5.689714448969315e-06 green
			389225 5.793564133855739e-06 green
			194598 5.8839248090936185e-06 green
			402796 5.474235096674247e-06 green
			397741 5.689632197837286e-06 green
			417690 2.6335320452967507e-06 green
			412833 2.7226505633028364e-06 green
			199531 6.014103071703144e-06 green
			310072 5.992156660388554e-06 green
			438208 5.620618519059442e-06 green
			13512 0.0021070159857904083 green
			32930 0.00034482235044032796 green
			17020 1.1927144535840188e-05 green
			6993 0.005162734162734163 green
			17130 1.1150029188558085e-05 green
			13512 0.002128478389579633 green
			7488 1.6025641025641026e-05 green
			7494 1.788097144382172e-05 green
			4254 1.9981194170192753e-05 green
			1087 6.2557497700092e-05 green
			7489 1.0148217385498725e-05 green
			6995 0.005033881343817013 green
			6995 0.00170421729807005 green
			7488 1.2686965811965809e-05 green
			6994 0.005104804117815271 green
			7489 1.8159967952997726e-05 green
			7384 1.1646803900325026e-05 green
			17136 1.3947245564892623e-05 green
			17129 1.4303228442991418e-05 green
			6880 0.005089970930232559 green
			612 0.023511437908496732 green
			4254 7.992477668077099e-06 green
			1087 5.7037718491260346e-05 green
			1087 6.2557497700092e-05 green
			612 0.07008660130718955 green
			6974 0.005139804989962718 green
			612 0.0718921568627451 green
			32822 0.00034123453781000545 green
			13512 0.002119819419775015 green
			17104 1.0056127221702525e-05 green
			173517 1.4932254476506631e-05 green
			71284 1.3102519499466935e-05 green
			71281 1.9416113690885348e-05 green
			173489 1.0358005406682848e-05 green
			37291 9.787884476147065e-06 green
			71287 5.050009118071961e-07 green
			173506 1.345774785886367e-05 green
			37267 1.9346875251563037e-05 green
			173494 9.187637612828117e-06 green
			71296 9.734066427289036e-06 green
			37290 5.819254491820878e-06 green
			70392 7.287759972724172e-06 green
			173487 1.1580118395038242e-05 green
			37291 1.7859537153736838e-05 green
			71297 1.3324543809697304e-06 green
			3287 2.7076361423790815e-05 green
			173487 1.4058690276504869e-05 green
			173511 -1.043161528663884e-06 green
			37284 1.5797661195150746e-05 green
			37284 2.084003862246538e-05 green
			173488 1.4450567186203078e-05 green
			173530 1.2683685818014179e-05 green
			173512 1.2627368712250444e-05 green
			37284 8.099989271537426e-06 green
			37291 2.1318816872703867e-05 green
			173484 1.2750455373406187e-05 green
			71292 6.522470964484092e-06 green
			37284 2.9369166398455117e-05 green
			71281 1.2724288379792651e-05 green
			37290 1.4802896218825459e-05 green
			6549 2.2598870056497175e-05 blue
			5720 2.3951048951048952e-05 blue
			6160 2.435064935064935e-05 blue
			7042 2.2010792388525987e-05 blue
			8813 2.4168841484171114e-05 blue
			6940 2.1469740634005762e-05 blue
			6632 2.110977080820265e-05 blue
			5946 1.765893037336024e-05 blue
			7182 1.9910888331940963e-05 blue
			7072 2.262443438914027e-05 blue
			7102 2.154322725992678e-05 blue
			7510 2.503328894806924e-05 blue
			6202 1.9348597226701065e-05 blue
			6719 2.6343205834201515e-05 blue
			7116 2.501405283867341e-05 blue
			5816 2.699449793672627e-05 blue
			5898 2.3228212953543575e-05 blue
			6001 1.933011164805866e-05 blue
			6663 2.1161638901395767e-05 blue
			6807 1.983252534156016e-05 blue
			11463 2.0064555526476487e-05 blue
			12006 2.2072297184740963e-05 blue
			13446 2.997173880708017e-05 blue
			17683 2.301645648362834e-05 blue
			12822 3.3224145999064115e-05 blue
			17988 3.3633533466755614e-05 blue
			16331 2.3819729349090685e-05 blue
			15596 2.9558861246473454e-05 blue
			13402 2.6563199522459338e-05 blue
			12144 2.3386034255599472e-05 blue
			13509 3.242282922496113e-05 blue
			12937 3.0996367009353016e-05 blue
			15161 3.027504782006464e-05 blue
			12120 3.2095709570957076e-05 blue
			12100 2.297520661157025e-05 blue
			12521 2.8032904720070286e-05 blue
			14499 2.648458514380303e-05 blue
			13681 3.2526862071486e-05 blue
			13690 3.842220598977356e-05 blue
			14230 2.8320449754040762e-05 blue
			14315 2.6266154383513798e-05 blue
			15405 2.9016553067185977e-05 blue
			13594 3.038105046343975e-05 blue
			13581 3.2250938811575e-05 blue
			14997 3.4606921384276866e-05 blue
			11368 2.6038001407459534e-05 blue
			12206 1.3026380468621991e-05 blue
			12490 2.5860688550840672e-05 blue
			13436 2.8803215242631744e-05 blue
			13098 1.4658726523133298e-05 blue
			13397 3.135030230648653e-05 blue
			15036 3.2987496674647503e-05 blue
			12927 1.52394213661329e-05 blue
			11972 2.6561977948546605e-05 blue
			15634 1.790968402200333e-05 blue
			13412 3.19862809424396e-05 blue
			8648 2.2895467160037003e-05 blue
			10675 3.156908665105387e-05 blue
			11946 2.578268876611418e-05 blue
			12064 1.6661140583554382e-05 blue
			9003 2.177052093746529e-05 blue
			8957 1.3843920955677126e-05 blue
			11225 1.3630289532293987e-05 blue
			8754 2.421750057116747e-05 blue
			10614 2.967778405879028e-05 blue
			10546 1.336999810354637e-05 blue
			8287 2.3651502353083144e-05 blue
			9608 1.1032472939217318e-05 blue
			10737 2.6729999068641145e-05 blue
			8602 2.6854219948849103e-05 blue
			9439 3.0829537027227455e-05 blue
			10609 3.1576962955980767e-05 blue
			3345 6.87593423019432e-06 blue
			3138 9.241555130656469e-06 blue
			3440 1.2499999999999999e-05 blue
			4193 1.9317910803720484e-05 blue
			4117 1.967452028175856e-05 blue
			2893 1.0024196335983408e-05 blue
			4510 1.3747228381374722e-05 blue
			5747 1.7226378980337568e-05 blue
			3375 1.5111111111111112e-05 blue
			3458 1.3302486986697515e-05 blue
			3297 1.759175007582651e-05 blue
			4564 1.7309377738825594e-05 blue
			3141 1.814708691499522e-05 blue
			3500 1.942857142857143e-05 blue
			3178 1.2271869100062933e-05 blue
			3881 1.597526410718887e-05 blue
			3539 1.8366770274088725e-05 blue
			3568 2.2141255605381167e-05 blue
			3146 1.3986013986013988e-05 blue
			2900 1.6206896551724137e-05 blue
			3768 1.7250530785562634e-05 blue
			3217 1.5853279452906432e-05 blue
			3238 2.2853613341568868e-05 blue
			730 2.1917808219178083e-05 blue
			69 0.0002463768115942029 blue
			270 -5.925925925925926e-05 blue
			122 -8.19672131147536e-06 blue
			5085 7.472959685349062e-06 blue
			232144 5.130436280929079e-06 blue
			12357 3.237031641984301e-06 blue
			7346 1.0345766403484899e-05 blue
			162131 5.501723914612232e-06 blue
			21068 5.64837668501993e-06 blue
			163494 1.551127258492667e-05 blue
			3752 5.597014925373139e-06 blue
			4348 3.4958601655933767e-05 blue
			239736 5.005506056662329e-06 blue
			237914 5.1615289558411865e-06 blue
			239628 5.174687432186555e-06 blue
			88008 5.874465957640216e-06 blue
			91359 8.110859357042e-06 blue
			657884 5.289686327680868e-06 blue
			9549 7.749502565713683e-06 blue
			5046 5.152596115735241e-06 blue
			4570 9.846827133479208e-06 blue
			7587 5.667589297482526e-06 blue
			140 7.142857142857143e-06 blue
			38 2.6315789473684212e-05 blue
			116 8.620689655172414e-06 blue
			40 5e-05 blue
			138 1.4492753623188407e-05 blue
			48 4.1666666666666665e-05 blue
			52 3.846153846153846e-05 blue
			124 1.6129032258064517e-05 blue
			180 5.555555555555556e-06 blue
			52 3.846153846153846e-05 blue
			166 1.2048192771084337e-05 blue
			196 5.102040816326531e-06 blue
			42 4.761904761904762e-05 blue
			46 4.347826086956522e-05 blue
			174 1.1494252873563218e-05 blue
			58 3.4482758620689657e-05 blue
			52 3.846153846153846e-05 blue
			168 1.1904761904761905e-05 blue
			58 3.4482758620689657e-05 blue
			162 6.17283950617284e-06 blue
			128 1.5625e-05 blue
			36 5.555555555555556e-05 blue
			172 5.8139534883720935e-06 blue
			50 0.0001 blue
			110 0.00011818181818181818 blue
			48 4.1666666666666665e-05 blue
			34 5.882352941176471e-05 blue
			46 0.0 blue
			102 1.9607843137254903e-05 blue
			142 1.4084507042253522e-05 blue
			54 1.8518518518518518e-05 blue
			54 3.7037037037037037e-05 blue
			200 0.0 blue
			52 3.846153846153846e-05 blue
			56 5.3571428571428575e-05 blue
			176 1.1363636363636365e-05 blue
			32 3.125e-05 blue
			146 5.479452054794521e-05 blue
			52 3.846153846153846e-05 blue
			144 1.388888888888889e-05 blue
			42 4.761904761904762e-05 blue
			44 4.545454545454546e-05 blue
			152 1.3157894736842106e-05 blue
			48 2.0833333333333333e-05 blue
			154 1.2987012987012988e-05 blue
			48 4.1666666666666665e-05 blue
			52 -1.923076923076923e-05 blue
			134 0.00015671641791044775 blue
			42 4.761904761904762e-05 blue
			182 5.494505494505494e-06 blue
			46 4.347826086956522e-05 blue
			120 8.333333333333334e-06 blue
			170 1.7647058823529414e-05 blue
			44 4.545454545454546e-05 blue
			126 7.936507936507936e-06 blue
			62 1.6129032258064517e-05 blue
			1 0.003 blue
			46 6.521739130434783e-05 blue
			58 1.7241379310344828e-05 blue
			156 2.5641025641025643e-05 blue
			46 4.347826086956522e-05 blue
			38 5.2631578947368424e-05 blue
			44 4.545454545454546e-05 blue
			50 2e-05 blue
			178 1.1235955056179776e-05 blue
			50 2e-05 blue
			54 3.7037037037037037e-05 blue
			54 3.7037037037037037e-05 blue
			136 2.9411764705882354e-05 blue
			44 0.0 blue
			160 1.25e-05 blue
			190 5.263157894736842e-06 blue
			60 3.3333333333333335e-05 blue
			122 8.19672131147541e-06 blue
			46 4.347826086956522e-05 blue
			48 0.00016666666666666666 blue
			130 1.5384615384615384e-05 blue
			50 4e-05 blue
			54 1.8518518518518518e-05 blue
			54 3.7037037037037037e-05 blue
			184 5.4347826086956525e-06 blue
			56 3.571428571428572e-05 blue
			50 2e-05 blue
			50 4e-05 blue
			186 0.0 blue
			132 3.787878787878788e-05 blue
			150 6.666666666666667e-06 blue
			56 -1.785714285714286e-05 blue
			188 1.0638297872340426e-05 blue
			52 1.923076923076923e-05 blue
			194 -5.154639175257732e-06 blue
			44 4.545454545454546e-05 blue
			890 -1.0112359550561806e-05 blue
			1469 3.4036759700476545e-06 blue
			2104 8.555133079847903e-06 blue
			2297 5.659555942533733e-06 blue
			2666 9.00225056264066e-06 blue
			2523 8.719778042013475e-06 blue
			2611 1.1106855610877059e-05 blue
			2611 1.0340865568747608e-05 blue
			2645 8.695652173913044e-06 blue
			2650 1.0188679245283019e-05 blue
			2610 9.578544061302683e-06 blue
			2531 9.482418016594231e-06 blue
			2621 4.196871423120944e-06 blue
			2520 8.333333333333334e-06 blue
			2609 8.432349559218092e-06 blue
			2519 9.527590313616515e-06 blue
			2581 1.0073614877954283e-05 blue
			2442 6.9615069615069606e-06 blue
			2466 9.7323600973236e-06 blue
			2544 7.861635220125786e-06 blue
			2483 8.457511075312124e-06 blue
			2647 9.066868152625614e-06 blue
			2538 5.910165484633569e-06 blue
			2595 5.780346820809248e-06 blue
			2619 9.16380297823597e-06 blue
			2602 1.0760953112990006e-05 blue
			2461 7.314099959366111e-06 blue
			2544 9.827044025157234e-06 blue
			2608 9.96932515337423e-06 blue
			2487 7.639726578206674e-06 blue
			2526 9.501187648456057e-06 blue
			2461 6.095083299471759e-06 blue
			2603 8.067614291202459e-06 blue
			2631 7.98175598631699e-06 blue
			2595 1.1175337186897882e-05 blue
			2546 1.2568735271013355e-05 blue
			2666 6.751687921980496e-06 blue
			2582 1.665375677769171e-05 blue
			2581 1.0461061604029444e-05 blue
			2456 8.550488599348534e-06 blue
			2566 1.1301636788776305e-05 blue
			2525 1.3465346534653463e-05 blue
			2513 9.55033824114604e-06 blue
			2525 1.1881188118811881e-05 blue
			2604 9.984639016897082e-06 blue
			2567 1.2076353720296066e-05 blue
			2579 5.4284606436603344e-06 blue
			2471 3.642250101173613e-06 blue
			2626 4.95049504950495e-06 blue
			2611 7.659900421294523e-06 blue
			2589 1.0428736964078793e-05 blue
			2587 6.571318129107073e-06 blue
			2665 7.879924953095683e-06 blue
			2525 7.524752475247524e-06 blue
			2532 4.739336492890995e-06 blue
			2598 8.468052347959967e-06 blue
			2577 6.596818005432673e-06 blue
			2608 5.368098159509202e-06 blue
			2564 8.970358814352575e-06 blue
			2668 6.746626686656671e-06 blue
			2565 1.01364522417154e-05 blue
			2581 7.361487795428127e-06 blue
			2608 9.585889570552148e-06 blue
			2580 3.875968992248063e-06 blue
			2611 7.659900421294523e-06 blue
			2566 1.0132501948558067e-05 blue
			2611 5.744925315970893e-06 blue
			2526 1.1480601741884402e-05 blue
			2633 8.355488036460312e-06 blue
			2511 1.2743926722421346e-05 blue
			2638 4.92797573919636e-06 blue
			2502 1.1191047162270183e-05 blue
			2570 1.245136186770428e-05 blue
			2621 5.341472720335751e-06 blue
			2511 8.761449621664674e-06 blue
			2538 1.0638297872340426e-05 blue
			2525 6.336633663366337e-06 blue
			2561 7.418976962124171e-06 blue
			2480 4.435483870967743e-06 blue
			2566 7.0148090413094315e-06 blue
			2608 8.052147239263803e-06 blue
			2575 9.70873786407767e-06 blue
			2609 4.9827520122652365e-06 blue
			2586 6.960556844547565e-06 blue
			2620 1.2595419847328245e-05 blue
			2591 3.8595137012736405e-06 blue
			2603 1.0756819054936613e-05 blue
			2574 3.885003885003886e-06 blue
			2509 5.978477481068154e-06 blue
			2577 9.701202949165697e-06 blue
			2542 7.474429583005508e-06 blue
			2611 8.808885484488702e-06 blue
			2522 3.965107057890564e-06 blue
			2601 1.2302960399846214e-05 blue
			2563 9.754194303550527e-06 blue
			2614 8.033664881407803e-06 blue
			2555 1.5655577299412916e-05 blue
			2667 5.999250093738283e-06 blue
			2596 9.63020030816641e-06 blue
			2509 5.57991231566361e-06 blue
			2597 6.546014632268001e-06 blue
			2448 4.493464052287581e-06 blue
			2521 4.760015866719556e-06 blue
			2526 9.501187648456055e-06 blue
			2680 4.850746268656717e-06 blue
			2589 8.497489378138279e-06 blue
			2501 4.798080767692923e-06 blue
			2627 3.0452988199467088e-06 blue
			2658 9.781790820165538e-06 blue
			2480 4.032258064516128e-06 blue
			2671 1.0482965181579932e-05 blue
			2640 5.681818181818183e-06 blue
			2647 6.4223649414431425e-06 blue
			2661 7.891770011273957e-06 blue
			2600 8.846153846153846e-06 blue
			2494 8.01924619085806e-06 blue
			2571 1.0501750291715286e-05 blue
			2603 4.610065309258548e-06 blue
			2621 7.249141549027088e-06 blue
			2576 9.70496894409938e-06 blue
			2583 8.904374758033294e-06 blue
			2601 4.61361014994233e-06 blue
			2591 9.262832883056735e-06 blue
			2621 9.919877909194964e-06 blue
			2628 7.990867579908674e-06 blue
			2631 1.1022424933485365e-05 blue
			2490 6.827309236947792e-06 blue
			2557 8.212749315604223e-06 blue
			2530 9.486166007905138e-06 blue
			2548 1.0596546310832023e-05 blue
			2670 8.614232209737828e-06 blue
			2567 8.570315543435916e-06 blue
			2633 8.735282947208507e-06 blue
			2529 9.094503756425464e-06 blue
			2543 1.0224144710971293e-05 blue
			2471 5.2610279239174424e-06 blue
			2637 8.722032612817595e-06 blue
			2470 6.4777327935222675e-06 blue
			2583 6.968641114982579e-06 blue
			2544 7.861635220125786e-06 blue
			2589 6.952491309385863e-06 blue
			2586 8.894044856921888e-06 blue
			2482 5.237711522965351e-06 blue
			2654 9.042954031650339e-06 blue
			2509 4.782781984854524e-06 blue
			2634 7.97266514806378e-06 blue
			2540 7.874015748031496e-06 blue
			2658 7.148231753197893e-06 blue
			2507 1.1567610690067811e-05 blue
			2542 4.327301337529504e-06 blue
			2570 6.22568093385214e-06 blue
			2630 9.885931558935359e-06 blue
			2619 6.8728522336769755e-06 blue
			2586 1.2374323279195669e-05 blue
			2611 7.659900421294523e-06 blue
			2601 1.114955786236063e-05 blue
			2547 8.244994110718492e-06 blue
			2541 7.4773711137347514e-06 blue
			2572 8.942457231726285e-06 blue
			2523 8.719778042013477e-06 blue
			2579 4.265219077161692e-06 blue
			2631 9.502090459901178e-06 blue
			2597 7.3161340007701205e-06 blue
			2497 8.00961153384061e-06 blue
			2547 3.9261876717707115e-06 blue
			2576 9.316770186335403e-06 blue
			2588 7.727975270479132e-06 blue
			2549 4.707728520988623e-06 blue
			2459 7.726718178121187e-06 blue
			2635 4.174573055028463e-06 blue
			2518 8.737092930897538e-06 blue
			2664 6.381381381381382e-06 blue
			2556 9.389671361502347e-06 blue
			2611 7.659900421294523e-06 blue
			2492 8.828250401284108e-06 blue
			2629 8.748573602130088e-06 blue
			2519 9.527590313616516e-06 blue
			2551 9.800078400627205e-06 blue
			2565 9.746588693957115e-06 blue
			2598 8.468052347959969e-06 blue
			2522 3.965107057890563e-06 blue
			2550 7.4509803921568615e-06 blue
			2617 6.4959877722583114e-06 blue
			2546 1.178318931657502e-05 blue
			691 4.196816208393632e-05 blue
			395 2.2784810126582277e-05 blue
			273 2.197802197802197e-05 blue
			233 6.0085836909871244e-05 blue
			187 5.8823529411764714e-05 blue
			771 5.188067444876788e-06 blue
			203 1.9704433497536946e-05 blue
			443 2.708803611738149e-05 blue
			763 2.0969855832241154e-05 blue
			377 5.305039787798409e-06 blue
			779 8.985879332477526e-06 blue
			675 3.111111111111112e-05 blue
			283 0.0 blue
			803 3.8605230386052304e-05 blue
			795 1.2578616352201252e-05 blue
			219 9.58904109589041e-05 blue
			329 9.118541033434648e-06 blue
			345 2.6086956521739135e-05 blue
			203 2.955665024630542e-05 blue
			643 6.220839813374811e-06 blue
			337 1.1869436201780416e-05 blue
			267 0.0 blue
			683 8.78477306002928e-06 blue
			195 7.179487179487179e-05 blue
			195 3.076923076923077e-05 blue
			651 -4.60829493087558e-06 blue
			659 7.587253414264043e-06 blue
			241 1.6597510373443984e-05 blue
			361 -1.1080332409972299e-05 blue
			214 0.00011682242990654206 blue
			627 1.2759170653907497e-05 blue
			667 1.199400299850075e-05 blue
			787 8.894536213468877e-06 blue
			219 8.219178082191782e-05 blue
			259 -6.563706563706563e-05 blue
			275 5.454545454545455e-05 blue
			635 7.874015748031503e-06 blue
			243 8.23045267489712e-06 blue
			225 4.444444444444441e-06 blue
			747 2.6773761713520773e-06 blue
			451 8.869179600886918e-06 blue
			227 4.405286343612331e-06 blue
			211 4.739336492890999e-06 blue
			369 1.626016260162601e-05 blue
			211 4.739336492890991e-06 blue
			699 1.144492131616595e-05 blue
			353 2.54957507082153e-05 blue
			427 2.1077283372365342e-05 blue
			235 3.404255319148936e-05 blue
			808 0.0009715346534653465 blue
			715 6.99300699300699e-06 blue
			417 1.6786570743405274e-05 blue
			385 1.2987012987012984e-05 blue
			819 3.663003663003666e-06 blue
			257 5.0583657587548636e-05 blue
			435 2.0689655172413797e-05 blue
			755 1.7218543046357614e-05 blue
			411 1.21654501216545e-05 blue
			811 8.631319358816267e-06 blue
			723 4.1493775933609995e-06 blue
			731 6.8399452804377435e-06 blue
			249 4.0160642570281094e-06 blue
			209 2.8708133971291875e-05 blue
			707 1.5558698727015563e-05 blue
			265 7.547169811320757e-05 blue
			739 1.623815967523681e-05 blue
			113 2.6548672566371683e-05 blue
			313 1.2779552715654946e-05 blue
			96 1.0416666666666666e-05 blue
			137 0.0 blue
			170 1.1764705882352942e-05 blue
			154 6.493506493506494e-06 blue
			257 1.5564202334630352e-05 blue
			241 4.149377593360993e-06 blue
			194 1.030927835051546e-05 blue
			210 4.285714285714286e-05 blue
			146 1.3698630136986302e-05 blue
			337 5.934718100890203e-06 blue
			249 1.2048192771084342e-05 blue
			113 4.424778761061947e-05 blue
			67 4.477611940298508e-05 blue
			177 2.2598870056497175e-05 blue
			87 2.2988505747126437e-05 blue
			96 6.25e-05 blue
			84 5.9523809523809524e-05 blue
			193 2.0725388601036267e-05 blue
			185 1.0810810810810807e-05 blue
			209 9.569377990430622e-06 blue
			111 0.00017117117117117117 blue
			329 1.8237082066869297e-05 blue
			95 0.00023157894736842107 blue
			217 4.60829493087558e-06 blue
			248 0.00011693548387096775 blue
			106 3.7735849056603776e-05 blue
			313 3.19488817891373e-06 blue
			84 3.571428571428572e-05 blue
			129 7.751937984496124e-05 blue
			225 8e-05 blue
			112 4.464285714285714e-05 blue
			256 1.5625e-05 blue
			225 4.444444444444448e-06 blue
			153 1.3071895424836602e-05 blue
			249 0.0 blue
			305 1.3114754098360657e-05 blue
			89 2.2471910112359552e-05 blue
			281 2.4911032028469753e-05 blue
			305 2.2950819672131146e-05 blue
			281 7.117437722419923e-06 blue
			119 2.5210084033613446e-05 blue
			98 2.0408163265306123e-05 blue
			176 5.681818181818182e-05 blue
			71 4.225352112676056e-05 blue
			168 2.976190476190476e-05 blue
			184 5.4347826086956525e-06 blue
			128 0.0001484375 blue
			136 1.4705882352941177e-05 blue
			121 1.652892561983471e-05 blue
			135 4.4444444444444447e-05 blue
			329 3.0395136778115495e-05 blue
			122 1.639344262295082e-05 blue
			97 1.0309278350515464e-05 blue
			273 1.0989010989010992e-05 blue
			98 3.061224489795918e-05 blue
			265 1.1320754716981136e-05 blue
			81 6.17283950617284e-05 blue
			233 -4.7210300429184545e-05 blue
			113 1.7699115044247787e-05 blue
			313 -2.8753993610223633e-05 blue
			257 7.782101167315176e-06 blue
			297 3.36700336700337e-06 blue
			177 5.649717514124294e-06 blue
			138 2.8985507246376814e-05 blue
			119 2.5210084033613446e-05 blue
			216 1.8518518518518518e-05 blue
			232 -8.620689655172414e-05 blue
			128 1.5625e-05 blue
			217 4.60829493087558e-06 blue
			345 1.7391304347826082e-05 blue
			80 2.5e-05 blue
			105 3.80952380952381e-05 blue
			185 5.405405405405405e-06 blue
			161 1.2422360248447205e-05 blue
			72 0.00011111111111111112 blue
			86 5.8139534883720933e-05 blue
			225 1.7777777777777777e-05 blue
			265 3.39622641509434e-05 blue
			75 4e-05 blue
			192 1.0416666666666663e-05 blue
			121 -5.785123966942149e-05 blue
			226 0.0 blue
			128 1.5625e-05 blue
			289 2.076124567474049e-05 blue
			80 2.5e-05 blue
			169 5.917159763313609e-06 blue
			353 2.8328611898017024e-06 blue
			169 1.1834319526627219e-05 blue
			84 2.380952380952381e-05 blue
			112 1.785714285714286e-05 blue
			233 6.437768240343348e-05 blue
			102 2.9411764705882354e-05 blue
			209 4.7846889952153066e-06 blue
			97 2.0618556701030927e-05 blue
			240 2.5e-05 blue
			88 2.272727272727273e-05 blue
			241 -4.149377593360996e-05 blue
			273 1.831501831501831e-05 blue
			105 1.904761904761905e-05 blue
			106 1.8867924528301888e-05 blue
			114 8.771929824561403e-06 blue
			104 -5.769230769230769e-05 blue
			129 1.5503875968992248e-05 blue
			209 0.0 blue
			289 1.038062283737024e-05 blue
			127 7.874015748031496e-05 blue
			234 0.0001282051282051282 blue
			85 2.3529411764705884e-05 blue
			89 2.2471910112359552e-05 blue
			65 0.0 blue
			105 9.523809523809525e-06 blue
			137 1.4598540145985402e-05 blue
			98 1.0204081632653061e-05 blue
			113 8.849557522123894e-06 blue
			297 1.6835016835016837e-05 blue
			233 2.1459227467811157e-05 blue
			152 6.578947368421053e-06 blue
			145 6.896551724137931e-06 blue
			114 8.771929824561403e-06 blue
			241 7.883817427385891e-05 blue
			217 4.60829493087558e-06 blue
			106 9.433962264150944e-06 blue
			297 3.36700336700337e-06 blue
			321 2.4922118380062307e-05 blue
			103 1.941747572815534e-05 blue
			297 6.734006734006735e-05 blue
			241 4.1493775933609995e-06 blue
			130 7.692307692307692e-06 blue
			273 1.465201465201466e-05 blue
			321 1.5576323987538943e-05 blue
			233 0.0 blue
			218 9.174311926605506e-06 blue
			200 6e-05 blue
			88 2.272727272727273e-05 blue
			193 0.00013989637305699483 blue
			144 1.388888888888889e-05 blue
			120 0.00021666666666666666 blue
			112 1.785714285714286e-05 blue
			305 4.9180327868852456e-05 blue
			120 8.333333333333334e-06 blue
			104 -9.615384615384616e-06 blue
			257 -2.3346303501945533e-05 blue
			160 1.8750000000000002e-05 blue
			201 9.950248756218906e-06 blue
			86 4.651162790697675e-05 blue
			64 3.125e-05 blue
			53 3.7735849056603776e-05 blue
			83 1.2048192771084337e-05 blue
			208 1.923076923076923e-05 blue
			249 6.827309236947791e-05 blue
			225 7.555555555555556e-05 blue
			224 1.785714285714286e-05 blue
			281 3.5587188612099613e-06 blue
			161 2.4844720496894403e-05 blue
			127 1.5748031496062993e-05 blue
			145 1.3793103448275862e-05 blue
			305 3.2786885245901667e-06 blue
			186 4.301075268817205e-05 blue
			87 5.747126436781609e-05 blue
			79 2.5316455696202533e-05 blue
			114 4.385964912280701e-05 blue
			264 7.196969696969696e-05 blue
			178 1.1235955056179776e-05 blue
			90 6.666666666666667e-05 blue
			122 0.00014754098360655736 blue
			265 7.169811320754718e-05 blue
			153 6.535947712418301e-06 blue
			162 1.8518518518518515e-05 blue
			289 8.304498269896194e-05 blue
			89 1.1235955056179776e-05 blue
			96 0.00019791666666666666 blue
			123 0.00038211382113821136 blue
			80 0.0 blue
			201 0.00011940298507462687 blue
			217 1.8433179723502303e-05 blue
			1 0.0 blue
			1 0.002 blue
			1 0.001 blue
			1 0.001 blue
			1 0.001 blue
			1 0.003 blue
			1 0.002 blue
			1 0.001 blue
			1 0.001 blue
			1 0.002 blue
			1 0.002 blue
			1 0.002 blue
			1 0.0 blue
			1 0.001 blue
			1 0.001 blue
			1 0.001 blue
			1 0.003 blue
			1 0.001 blue
			1 -0.004 blue
			1 0.013 blue
			1 0.002 blue
			1 0.011 blue
			1 0.001 blue
			1 0.001 blue
			1 0.001 blue
			11 0.00027272727272727274 blue
			1 0.001 blue
			21 0.0002380952380952381 blue
			34 0.0 blue
			131 3.816793893129769e-05 blue
			116 8.620689655172414e-06 blue
			129 0.0 blue
			120 3.3333333333333335e-05 blue
			232 2.586206896551724e-05 blue
			70 7.142857142857145e-05 blue
			17 0.00011764705882352942 blue
			69 0.00011594202898550725 blue
			22 9.090909090909092e-05 blue
			452 8.849557522123894e-06 blue
			127 3.937007874015746e-05 blue
			21 4.761904761904762e-05 blue
			900 5.222222222222222e-05 blue
			133 4.511278195488726e-05 blue
			18 0.0002777777777777778 blue
			38 0.0 blue
			66 -6.0606060606060605e-05 blue
			33 9.090909090909098e-05 blue
			228 0.00011403508771929826 blue
			65 0.00018461538461538463 blue
			456 2.4122807017543866e-05 blue
			37 5.4054054054054006e-05 blue
			883 3.1710079275198195e-05 blue
			1 0.001 blue
			1 0.002 blue
			1 0.001 blue
			1 0.004 blue
			1 0.002 blue
			1 0.002 blue
			1 0.001 blue
			1 0.002 blue
			1 0.003 blue
			1 0.002 blue
			1 0.002 blue
			474 1.4767932489451475e-05 blue
			470 8.510638297872333e-06 blue
			468 2.136752136752137e-05 blue
			466 2.1459227467811164e-05 blue
			479 2.505219206680584e-05 blue
			469 3.411513859275053e-05 blue
			464 2.801724137931034e-05 blue
			456 3.94736842105263e-05 blue
			475 8.42105263157894e-06 blue
			474 4.219409282700425e-06 blue
			459 8.714596949891075e-06 blue
			468 2.1367521367521357e-05 blue
			472 1.0593220338983045e-05 blue
			471 2.7600849256900223e-05 blue
			462 1.9480519480519483e-05 blue
			474 2.1097046413502112e-05 blue
			446 1.5695067264573988e-05 blue
			463 1.727861771058314e-05 blue
			441 2.267573696145125e-05 blue
			462 1.73160173160173e-05 blue
			446 1.7937219730941705e-05 blue
			448 1.5624999999999997e-05 blue
			442 2.0361990950226248e-05 blue
			463 2.1598272138228933e-05 blue
			441 4.535147392290254e-06 blue
			445 1.5730337078651683e-05 blue
			459 3.921568627450979e-05 blue
			444 1.1261261261261256e-05 blue
			466 2.1459227467811147e-05 blue
			447 2.0134228187919465e-05 blue
			444 1.3513513513513525e-05 blue
			443 9.029345372460489e-06 blue
			443 1.580135440180587e-05 blue
			466 1.931330472103003e-05 blue
			465 1.5053763440860229e-05 blue
			443 2.031602708803612e-05 blue
			461 1.7353579175705003e-05 blue
			462 3.4632034632034636e-05 blue
			445 1.797752808988764e-05 blue
			449 2.00445434298441e-05 blue
			438 1.8264840182648402e-05 blue
			464 4.956896551724139e-05 blue
			442 2.0361990950226248e-05 blue
			458 1.528384279475984e-05 blue
			454 1.982378854625551e-05 blue
			466 1.7167381974248913e-05 blue
			754 2.2546419098143238e-05 blue
			787 2.287166454891997e-05 blue
			815 2.453987730061352e-05 blue
			755 2.649006622516557e-05 blue
			760 2.1052631578947386e-05 blue
			783 2.0434227330779074e-05 blue
			789 2.91508238276299e-05 blue
			797 2.5094102885821818e-05 blue
			761 2.890932982917213e-05 blue
			772 -2.590673575129536e-06 blue
			756 1.058201058201059e-05 blue
			791 2.5284450063211146e-05 blue
			802 2.4937655860349115e-05 blue
			751 3.195739014647138e-05 blue
			810 1.60493827160494e-05 blue
			800 2.3749999999999988e-05 blue
			756 2.3809523809523814e-05 blue
			757 1.8494055482166465e-05 blue
			768 1.5624999999999977e-05 blue
			762 2.6246719160104974e-05 blue
			800 2.874999999999999e-05 blue
			813 1.4760147601476027e-05 blue
			812 2.0935960591133023e-05 blue
			761 3.153745072273324e-05 blue
			785 2.2929936305732504e-05 blue
			785 2.038216560509556e-05 blue
			756 7.275132275132276e-05 blue
			805 1.987577639751551e-05 blue
			799 1.877346683354191e-05 blue
			751 2.6631158455392816e-05 blue
		};
		\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
		\begin{axis}[
		scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
		ylabel=Overhead per transaction,
		xlabel=Reductions+model-clean-up,
		xmode=log,
		ymode=log,
		grid=both,
		grid style={line width=.1pt, draw=gray!10},
		major grid style={line width=.2pt,draw=gray!50},
		minor tick num=5,
		xtick={1,10,100,1000,10000, 100000, 1000000, 10000000, 100000000},
		ytick={0,0.1,0.01,0.001,0.0001, 0.00001, 0.000001, 0.0000001, 0.00000001, 0.000000001},
		]
		\addplot[domain=1:100000000, pbred] {0.00025274999999999994 };
		\addplot[scatter,only marks, scatter src=explicit symbolic]%
		table[meta=label] {
			x y label
			15000000 0.2 peer
			15000000 0.0000001 peer
			197 3.553299492385783e-05 green
			424687 6.498903898635936e-06 green
			4612 0.00593733738074588 green
			2 0.0085 green
			27346 0.014614422584655892 green
			6751 7.998814990371795e-06 green
			1474 1.35685210312076e-05 green
			59611 0.0916516414755666 green
			39424 1.065340909090909e-06 green
			7022 9.399031614924526e-06 green
			1 0.016999999999999998 green
			125076 0.007659023313825193 green
			174432 4.213676389653275e-06 green
			4882 0.006106718557968045 green
			1 0.017 green
			4898 0.0023527970600244995 green
			36 0.00030555555555555555 green
			13 0.0006923076923076924 green
			174 0.00014367816091954023 green
			62 0.0003548387096774192 green
			11 0.0008181818181818183 green
			36668 0.0002276644485655067 green
			24245 0.0013703856465250568 green
			67 0.002791044776119403 green
			3 0.005666666666666667 green
			18900 8.148148148148143e-06 green
			51204 1.3592688071244429e-05 green
			181 0.0002154696132596685 green
			31582 4.147932366537901e-06 green
			16 0.0008125000000000001 green
			1 0.016999999999999998 green
			92 0.0001956521739130435 green
			226 0.00010176991150442478 green
			50769 0.006120014181882644 green
			24 0.0018333333333333333 green
			309 0.0019158576051779934 green
			19305 0.00010981610981610983 green
			7970 0.010051317440401506 green
			12548 7.252151737328658e-06 green
			6960 1.5804597701149419e-06 green
			658 0.03551975683890578 green
			79962 0.1330552137265201 green
			40 0.001 green
			36 0.00036111111111111115 green
			968 7.231404958677685e-06 green
			440 9.090909090909035e-06 green
			3 0.001666666666666666 green
			98 9.183673469387756e-05 green
			72 0.00011111111111111112 green
			180 1.666666666666668e-05 green
			92620 2.548045778449579e-06 green
			279345 4.375592904830944e-05 green
			52001 9.48058691179016e-06 green
			851 1.2925969447708578e-05 green
			15320 0.44628844647519583 green
			16817818 0.0006405935062443891 green
			63626 0.00689295256656084 green
			39 -2.5641025641025663e-05 green
			35011 0.008423524035303191 green
			87340 0.019595065262193727 green
			1570734 0.006866538828343946 green
			309 0.001854368932038835 green
			10500 2.9523809523809525e-06 green
			6553 3.815046543567832e-06 green
			233180 2.1914400892014756e-06 green
			440 9.0909090909091e-06 green
			154 0.00014935064935064937 green
			118 0.015635593220338983 green
			2060 3.8834951456310716e-06 green
			2801 8.211353088182791e-06 green
			88623 0.00062015503875969 green
			586368 2.1437049770792404e-06 green
			440 1.5909090909090924e-05 green
			120 0.0007666666666666655 green
			8159 0.00045814438043877934 green
			86 3.488372093023251e-05 green
			480 4.1666666666666635e-06 green
			2694 0.002340386043058649 green
			2 -0.008500000000000002 green
			31387 1.5643419250007967e-05 green
			40 2.500000000000002e-05 green
			70467 0.00027536293584230916 green
			6125 0.0030907755102040817 green
			450 0.00017777777777777743 green
			14306 6.535719278624354e-05 green
			8605 3.590935502614759e-05 green
			1557 0.0008516377649325626 green
			1556 0.009052699228791775 green
			13 7.692307692307693e-05 green
			2726 0.0974402054292003 green
			4385 0.5556549600912201 green
			24360 0.002744334975369458 green
			3 0.0013333333333333346 green
			3 0.007666666666666668 green
			423 5.91016548463357e-05 green
			203169 0.0006198337344772087 green
			36 2.7777777777777803e-05 blue
			8253 4.604386283775601e-06 blue
			1062 3.7664783427495325e-06 blue
			1570734 3.467805497302535e-05 blue
			22761 9.621721365493582e-06 blue
			16820374 2.0555072081036942e-05 blue
			19305 3.833203833203832e-06 blue
			2214 -1.2195121951219511e-05 blue
			81091 2.4219703789569727e-05 blue
			88656 1.4505504421584552e-05 blue
			53 9.433962264150952e-05 blue
			465 -2.3655913978494616e-05 blue
			968 9.297520661157025e-06 blue
			16 0.0001250000000000001 blue
			10306 7.859499320784009e-06 blue
			286332 6.003520388919157e-06 blue
			1474 8.819538670284937e-06 blue
			3 -0.0013333333333333346 blue
			203019 1.4939488422265894e-05 blue
			3 0.0006666666666666673 blue
			481 1.0395010395010397e-05 blue
			92 5.43478260869565e-05 blue
			423 -1.182033096926715e-05 blue
			440 6.818181818181824e-06 blue
			424713 6.522051361743105e-07 blue
			36 0.0005 blue
			174 1.724137931034482e-05 blue
			1570734 3.521729331637311e-05 blue
			360 8.333333333333322e-06 blue
			586368 2.2306810740013098e-06 blue
			3 0.00033333333333333365 blue
			39424 4.565746753246754e-07 blue
			3 -0.00033333333333333365 blue
			18900 7.407407407407408e-06 blue
			2060 3.3980582524271874e-06 blue
			197 1.01522842639594e-05 blue
			125076 2.2202500879465286e-05 blue
			1372 1.5306122448979605e-05 blue
			1 0.002 blue
			7326 1.3650013650013661e-07 blue
			6616 8.917775090689129e-06 blue
			6413 7.328863246530485e-06 blue
			27574 0.00010995865670559223 blue
			15670 3.7013401403956613e-06 blue
			6149 7.643519271426249e-06 blue
			125076 2.216252518468771e-05 blue
			2801 6.0692609782220626e-06 blue
			18900 4.497354497354501e-06 blue
			586368 2.1539374590700724e-06 blue
			16820374 8.322585454996451e-06 blue
			9 -0.00033333333333333327 blue
			13 7.692307692307693e-05 blue
			50134 5.545139027406551e-06 blue
			424713 6.710413855945077e-07 blue
			10500 3.2380952380952385e-06 blue
			92 2.1739130434782627e-05 blue
			16497 1.7639570831060214e-05 blue
			17110 1.163062536528346e-05 blue
			1474 5.427408412483044e-06 blue
			27574 0.00011144556466236309 blue
			86 1.1627906976744197e-05 blue
			40 0.00032500000000000004 blue
			2694 2.1529324424647364e-05 blue
			30049 2.595760258244867e-05 blue
			5 0.007400000000000001 blue
			53 0.00018867924528301905 blue
			14576 1.1525795828759604e-05 blue
			31387 1.554783827699366e-05 blue
			6130 1.566068515497553e-05 blue
			440 1.1363636363636373e-05 blue
			60794 9.194986347336911e-06 blue
			154 3.896103896103895e-05 blue
			4608 4.774305555555557e-06 blue
			451 6.208425720620848e-05 blue
			3 0.0006666666666666661 blue
			7 -0.0005714285714285715 blue
			19305 3.4706034706034694e-06 blue
			57208 1.1466927702419243e-05 blue
			220 4.5454545454545465e-05 blue
			4899 2.1637068789548883e-05 blue
			7 0.0014285714285714284 blue
			81091 -2.5563872686241477e-05 blue
			36676 1.3360235576398735e-05 blue
			88661 1.4222713481688676e-05 blue
			8253 1.211680600993579e-06 blue
			57457 3.078824164157543e-05 blue
			3 0.0006666666666666673 blue
			5 0.029800000000000004 blue
			309 1.2944983818770227e-05 blue
			87912 5.5851305851305816e-06 blue
			632 1.5822784810126596e-06 blue
			16497 3.6976419955143323e-06 blue
			36 0.00016666666666666663 blue
			5 0.0064 blue
			2214 1.4453477868112015e-05 blue
			851 1.5276145710928316e-05 blue
			251 -7.171314741035856e-05 blue
			1 0.001 blue
			9206 7.820986313273952e-06 blue
			56647 1.0768443165569226e-05 blue
			166 1.8072289156626502e-05 blue
			440 1.1363636363636373e-05 blue
			6130 1.598694942903752e-05 blue
			39424 6.594967532467532e-07 blue
			8605 4.067402672864613e-06 blue
			10500 2.6666666666666664e-06 blue
			311 3.2154340836012835e-06 blue
			36676 1.1778819936743372e-05 blue
			5622 -0.00010690145855567398 blue
			91 -6.593406593406592e-05 blue
			30049 2.702252986788246e-05 blue
			8605 4.8808832074375365e-06 blue
			2127 0.00017254348848142923 blue
			309 1.2944983818770227e-05 blue
			851 1.527614571092832e-05 blue
			197 -1.01522842639594e-05 blue
			166 2.4096385542168674e-05 blue
			6616 1.1336154776299771e-05 blue
			2471 7.770133549170375e-05 blue
			2694 2.078693392724573e-05 blue
			51206 4.122563762059135e-05 blue
			31582 4.8761953011208926e-06 blue
			174432 4.104751421757475e-06 blue
			9 0.0013333333333333333 blue
			440 4.54545454545455e-06 blue
			4684 7.258753202391119e-06 blue
			423 7.09219858156029e-06 blue
			440 2.272727272727275e-06 blue
			2060 4.854368932038839e-06 blue
			40 0.00012500000000000003 blue
			50134 5.764551003311127e-06 blue
			5 0.0142 blue
			3 0.0013333333333333333 blue
			24360 4.146141215106731e-06 blue
			70486 6.22818715773345e-06 blue
			560 7.142857142857143e-06 blue
			24360 1.2725779967159266e-06 blue
			6751 6.813805362168569e-06 blue
			251 -1.1952191235059758e-05 blue
			945 3.915343915343916e-05 blue
			36 -0.00016666666666666663 blue
			309 6.472491909385119e-06 blue
			174432 4.156347459181801e-06 blue
			309 6.472491909385119e-06 blue
			91 1.0989010989010999e-05 blue
			1 0.001 blue
			14306 4.124143715923387e-06 blue
			6553 2.8994353731115513e-06 blue
			87544 1.691720734716257e-05 blue
			1372 1.5306122448979605e-05 blue
			311 3.2154340836012835e-06 blue
			2471 7.770133549170375e-05 blue
			7023 6.407518154634771e-06 blue
			6751 6.813805362168569e-06 blue
			968 1.136363636363636e-05 blue
			4132 4.114230396902225e-05 blue
			945 2.9629629629629627e-05 blue
			1 0.001 blue
			440 9.0909090909091e-06 blue
			5622 -0.0008356456776947668 blue
			70486 6.072127798428057e-06 blue
			10542 2.048947068867388e-05 blue
			7336 5.452562704471101e-07 blue
			66 6.060606060606056e-05 blue
			57457 3.056198548479733e-05 blue
			174 3.448275862068966e-05 blue
			72 4.166666666666666e-05 blue
			22761 6.941698519397231e-06 blue
			98048 6.670202349869452e-06 blue
			60794 6.859229529229855e-06 blue
			464 -4.3103448275862105e-06 blue
			4684 5.764304013663534e-06 blue
			66 3.030303030303033e-05 blue
			31387 1.5388536655303152e-05 blue
			233180 2.225748348915002e-06 blue
			2127 0.0001081335213916314 blue
			560 3.5714285714285714e-06 blue
			7023 7.119464616260858e-06 blue
			14306 4.124143715923387e-06 blue
			4898 1.7762351980400162e-05 blue
			1 0.002 blue
			31582 2.0264707744917976e-06 blue
			19090 7.752750130958618e-06 blue
			5 0.0025999999999999994 blue
			72 2.7777777777777803e-05 blue
			16 0.00031250000000000006 blue
			155 1.9354838709677414e-05 blue
			360 8.888888888888889e-05 blue
			4132 3.654404646660208e-05 blue
			203015 1.6171218875452557e-05 blue
			87 2.298850574712638e-05 blue
			51204 9.745332395906563e-06 blue
		};
		\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\caption{
		Overhead per applied reductions including model-clean-up on \pb (left) and \miplib (right) on instances with more than 1 seconds in \veripb.
		Each $\times$ marks an instance.
		The $y$-axis gives the time for presolving and
		the $x$-axis gives the time for verifying. Green $+$ mark optimization instances and blue $\times$ mark decision instances.
		The 99\% quantile for the decision instances is marked by a red line. 
	}
	\label{fig:secondspertransactions}
\end{figure}

\begin{figure}[ht]
	\centering
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
			\begin{axis}[
				scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
				ylabel=certifying (time),
				xlabel=default (time),
				xmode=log,
				ymode=log,
				grid=both,
				grid style={line width=.1pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				minor tick num=5,
				xtick={0.001,0.01,0.1,1,10,100,1000},
				ytick={0.001,0.01,0.1,1,10,100,1000},
			]
				\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x });
				\addplot[scatter,only marks, scatter src=explicit symbolic]
				table[meta=label] {
					x y label
					1000 1000 peer
					0.032 0.058 green
					0.001 0.005 green
					0.006 0.075 green
					0.002 0.003 green
					0.001 0.003 green
					0.007 0.02 green
					0.006 0.011 green
					0.023 0.07 green
					0.013 0.006 green
					0.02 0.112 green
					0.002 0.004 green
					0.001 0.003 green
					0.002 0.004 green
					0.006 0.023 green
					0.007 0.012 green
					0.004 0.006 green
					0.003 0.006 green
					0.079 1.024 green
					0.09 1.108 green
					0.082 0.446 green
					0.091 0.941 green
					0.081 0.508 green
					0.074 0.982 green
					0.104 1.402 green
					0.011 0.015 green
					0.083 1.07 green
					0.084 0.479 green
					0.086 1.031 green
					0.075 0.469 green
					0.084 1.02 green
					0.116 1.104 green
					0.093 1.289 green
					0.073 0.468 green
					0.076 1.16 green
					0.076 0.501 green
					0.074 1.203 green
					0.067 1.08 green
					0.09 0.465 green
					0.068 1.039 green
					0.076 1.176 green
					0.081 0.524 green
					0.011 0.019 green
					0.032 0.516 green
					0.072 1.12 green
					0.013 0.018 green
					0.08 1.442 green
					0.096 1.447 green
					0.042 0.309 green
					0.076 1.397 green
					0.047 0.367 green
					0.092 1.338 green
					0.08 0.392 green
					0.031 0.272 green
					0.033 0.852 green
					0.055 1.089 green
					0.088 0.674 green
					0.076 1.49 green
					0.026 0.645 green
					0.092 1.675 green
					0.093 0.603 green
					0.081 1.236 green
					0.001 0.006 green
					0.001 0.002 green
					0.001 0.007 green
					0.002 0.004 green
					1.044 1.378 green
					1.202 1.372 green
					1.131 1.445 green
					1.433 1.798 green
					1.556 2.002 green
					0.965 1.141 green
					1.234 1.743 green
					1.178 1.467 green
					2.641 3.119 green
					3.157 3.341 green
					0.629 1.102 green
					1.144 1.65 green
					0.892 1.082 green
					1.191 1.485 green
					1.283 1.702 green
					0.718 0.934 green
					1.197 1.466 green
					2.308 2.736 green
					3.231 3.586 green
					1.221 1.676 green
					1.733 2.139 green
					1.102 1.239 green
					0.655 1.056 green
					0.522 0.948 green
					1.083 1.346 green
					1.299 1.476 green
					1.583 1.861 green
					1.795 2.255 green
					0.573 0.996 green
					0.882 1.282 green
					1.876 2.147 green
					0.905 1.261 green
					0.594 0.957 green
					1.334 1.702 green
					2.265 2.347 green
					0.884 1.347 green
					1.152 1.419 green
					1.612 1.896 green
					0.667 1.043 green
					1.677 2.003 green
					2.749 2.987 green
					1.258 1.653 green
					2.407 2.797 green
					1.06 1.289 green
					1.854 2.308 green
					3.025 3.1 green
					1.072 1.422 green
					0.955 1.442 green
					1.748 2.019 green
					0.649 0.955 green
					0.998 1.408 green
					2.669 3.25 green
					1.263 1.555 green
					0.716 1.163 green
					1.081 1.222 green
					0.172 0.242 green
					0.355 0.408 green
					0.32 0.375 green
					0.317 0.346 green
					0.438 0.462 green
					0.504 0.575 green
					0.406 0.456 green
					0.462 0.506 green
					0.286 0.355 green
					0.757 0.842 green
					0.27 0.3 green
					0.458 0.512 green
					0.296 0.346 green
					0.385 0.42 green
					0.152 0.202 green
					0.346 0.353 green
					0.432 0.458 green
					0.424 0.464 green
					0.332 0.371 green
					0.301 0.347 green
					0.228 0.258 green
					0.327 0.367 green
					0.29 0.36 green
					0.246 0.314 green
					0.237 0.284 green
					0.712 0.745 green
					0.275 0.322 green
					0.301 0.368 green
					0.303 0.357 green
					0.493 0.784 green
					1.157 1.416 green
					1.178 1.363 green
					0.863 1.259 green
					1.495 1.695 green
					0.793 1.086 green
					0.832 1.073 green
					0.984 1.211 green
					1.321 1.611 green
					0.644 0.91 green
					1.319 1.672 green
					0.558 0.865 green
					1.32 1.644 green
					1.036 1.403 green
					1.336 1.569 green
					0.753 1.016 green
					0.652 1.008 green
					1.701 1.945 green
					1.33 1.507 green
					0.442 0.691 green
					0.883 1.017 green
					0.857 1.073 green
					1.629 1.86 green
					1.575 1.804 green
					2.352 2.586 green
					0.636 0.829 green
					1.622 1.909 green
					1.073 1.318 green
					1.661 1.901 green
					0.706 0.971 green
					0.922 1.151 green
					0.444 0.696 green
					0.609 0.755 green
					0.429 0.578 green
					0.716 0.788 green
					0.684 0.768 green
					0.67 0.806 green
					0.538 0.689 green
					0.636 0.749 green
					0.728 0.897 green
					0.465 0.649 green
					0.709 0.825 green
					0.653 0.878 green
					1.42 1.525 green
					0.624 0.758 green
					0.718 0.916 green
					0.981 1.082 green
					0.602 0.805 green
					0.485 0.663 green
					0.683 0.69 green
					0.63 0.887 green
					0.49 0.593 green
					0.532 0.686 green
					1.182 1.356 green
					1.037 1.228 green
					0.006 0.006 green
					0.012 0.121 green
					0.014 0.016 green
					0.805 8.28 green
					0.003 0.026 green
					0.005 0.006 green
					0.011 0.035 green
					0.049 0.046 green
					0.019 0.01 green
					0.042 1.797 green
					0.503 0.589 green
					0.016 0.046 green
					0.008 0.012 green
					0.021 0.02 green
					0.084 0.161 green
					0.022 0.117 green
					0.034 0.029 green
					0.018 0.017 green
					0.046 2.122 green
					2.385 2.501 green
					0.026 0.029 green
					0.045 0.064 green
					0.659 1.17 green
					0.029 0.036 green
					0.021 0.017 green
					0.335 0.338 green
					0.019 0.021 green
					0.347 0.39 green
					0.016 0.02 green
					0.059 0.062 green
					0.032 0.021 green
					0.051 0.038 green
					0.015 0.011 green
					0.012 0.01 green
					0.963 6659.463 green
					0.009 0.01 green
					0.028 0.041 green
					0.658 2.787 green
					1.398 23.582 green
					0.178 0.373 green
					0.157 0.164 green
					11.624 11.829 green
					0.144 12.797 green
					0.003 0.005 green
					0.014 0.015 green
					2.769 5.463 green
					0.164 0.154 green
					0.002 0.003 green
					0.321 0.298 green
					0.221 0.21 green
					0.304 0.309 green
					0.294 0.278 green
					0.001 0.005 green
					0.001 0.005 green
					0.002 0.006 green
					0.001 0.008 green
					0.002 0.005 green
					0.002 0.003 green
					0.002 0.004 green
					0.002 0.005 green
					0.002 0.007 green
					0.003 0.009 green
					0.011 0.02 green
					0.001 0.004 green
					0.001 0.005 green
					0.002 0.005 green
					0.002 0.008 green
					0.001 0.003 green
					0.002 0.004 green
					0.002 0.007 green
					0.002 0.008 green
					0.031 0.007 green
					0.002 0.004 green
					0.002 0.004 green
					0.002 0.005 green
					0.002 0.016 green
					0.002 0.004 green
					0.002 0.008 green
					0.001 0.003 green
					0.001 0.003 green
					0.002 0.01 green
					0.002 0.006 green
					0.001 0.005 green
					0.001 0.004 green
					0.002 0.006 green
					0.002 0.006 green
					0.002 0.005 green
					0.002 0.006 green
					0.001 0.004 green
					0.001 0.005 green
					0.001 0.006 green
					0.004 0.004 green
					0.001 0.003 green
					0.002 0.005 green
					0.002 0.004 green
					0.002 0.005 green
					0.001 0.004 green
					0.003 0.007 green
					0.002 0.004 green
					0.003 0.005 green
					0.002 0.004 green
					0.002 0.025 green
					0.001 0.004 green
					0.003 0.014 green
					0.002 0.007 green
					0.002 0.004 green
					0.002 0.006 green
					0.002 0.008 green
					0.004 0.005 green
					0.001 0.003 green
					0.002 0.005 green
					0.002 0.043 green
					0.031 0.041 green
					0.041 0.045 green
					0.056 0.043 green
					0.035 0.042 green
					0.05 0.04 green
					0.031 0.044 green
					0.047 0.066 green
					0.038 0.043 green
					0.037 0.04 green
					0.039 0.051 green
					0.032 0.056 green
					0.039 0.043 green
					0.031 0.041 green
					0.036 0.043 green
					0.039 0.049 green
					0.032 0.052 green
					0.058 0.047 green
					0.002 0.003 green
					0.003 0.004 green
					0.006 0.005 green
					0.018 0.005 green
					0.025 0.034 green
					0.028 0.02 green
					0.02 0.019 green
					0.002 0.003 green
					0.002 0.005 green
					0.024 0.021 green
					0.008 0.015 green
					0.026 0.039 green
					0.044 0.056 green
					0.007 0.008 green
					0.027 0.024 green
					0.019 0.017 green
					0.018 0.011 green
					0.027 0.035 green
					0.021 0.02 green
					0.003 0.004 green
					0.012 0.022 green
					0.007 0.007 green
					0.002 0.003 green
					0.023 0.02 green
					0.044 0.034 green
					0.044 0.043 green
					0.024 0.02 green
					0.002 0.003 green
					0.004 0.005 green
					0.015 0.009 green
					0.003 0.003 green
					0.013 0.012 green
					0.024 0.019 green
					0.002 0.003 green
					0.026 0.022 green
					0.017 0.018 green
					0.004 0.006 green
					0.004 0.005 green
					0.025 0.023 green
					0.006 0.007 green
					0.058 0.07 green
					0.022 0.025 green
					0.028 0.022 green
					0.034 0.035 green
					0.019 0.019 green
					0.034 0.029 green
					0.003 0.004 green
					0.012 0.027 green
					0.014 0.021 green
					0.003 0.004 green
					0.018 0.024 green
					0.026 0.026 green
					0.012 0.015 green
					0.002 0.004 green
					0.027 0.027 green
					0.029 0.019 green
					0.005 0.005 green
					0.003 0.004 green
					0.011 0.017 green
					0.001 0.004 green
					0.022 0.015 green
					0.01 0.015 green
					0.006 0.017 green
					0.018 0.036 green
					0.025 0.019 green
					0.004 0.005 green
					0.004 0.006 green
					0.003 0.004 green
					0.004 0.004 green
					0.002 0.002 green
					0.005 0.006 green
					0.003 0.019 green
					0.037 0.046 green
					0.009 0.008 green
					0.05 0.03 green
					0.01 0.045 green
					0.007 0.009 green
					0.001 0.003 green
					0.033 0.035 green
					0.03 0.022 green
					0.008 0.008 green
					0.006 0.007 green
					0.014 0.01 green
					0.008 0.039 green
					0.003 0.004 green
					0.008 0.011 green
					0.007 0.009 green
					0.001 0.005 green
					0.005 0.007 green
					0.004 0.003 green
					0.004 0.006 green
					0.034 0.035 green
					0.002 0.023 green
					0.026 0.03 green
					0.021 0.032 green
					0.025 0.027 green
					0.001 0.002 green
					0.052 0.059 green
					0.06 0.047 green
					0.056 0.059 green
					0.051 0.059 green
					0.051 0.064 green
					0.059 0.046 green
					0.021 0.027 green
					0.039 0.04 green
					0.028 0.029 green
					0.014 0.025 green
					0.037 0.024 green
					0.023 0.025 green
					0.02 0.023 green
					0.027 0.026 green
					0.021 0.024 green
					0.024 0.024 green
					0.022 0.023 green
					0.021 0.022 green
					0.054 0.061 green
					0.161 0.171 green
					0.165 0.157 green
					0.106 0.117 green
					0.327 1.551 green
					0.293 2.429 green
					0.356 0.87 green
					0.817 2.883 green
					0.285 2.445 green
					0.309 2.569 green
					0.736 3.108 green
					0.315 1.48 green
					0.523 2.783 green
					0.32 2.46 green
					0.464 2.814 green
					0.601 2.856 green
					0.321 1.466 green
					0.697 2.902 green
					0.364 2.627 green
					0.534 1.634 green
					0.901 2.025 green
					0.331 1.531 green
					0.324 2.182 green
					0.785 3.248 green
					0.242 28.712 green
					0.189 11.544 green
					0.181 0.384 green
					0.272 36.375 green
					0.175 0.366 green
					0.249 29.009 green
					0.295 0.415 green
					0.231 0.365 green
					0.266 0.351 green
					0.248 0.316 green
					0.281 0.357 green
					0.287 35.499 green
					0.288 12.209 green
					0.274 0.369 green
					0.284 35.987 green
					0.229 0.365 green
					0.21 0.296 green
					0.183 0.422 green
					0.178 0.423 green
					0.242 35.261 green
					0.303 14.692 green
					0.319 0.353 green
					0.246 0.308 green
					0.245 0.313 green
					0.306 43.199 green
					0.259 36.104 green
					0.412 44.41 green
					0.752 11.952 green
					0.246 28.889 green
					0.178 0.35 green
					8.033 10.624 green
					12.651 13.585 green
					12.438 13.822 green
					8.311 10.108 green
					14.609 14.974 green
					13.052 13.088 green
					7.94 10.275 green
					2.172 2.893 green
					8.004 9.598 green
					13.179 13.873 green
					14.831 15.048 green
					2.037 2.55 green
					7.704 9.713 green
					14.863 15.529 green
					13.473 13.568 green
					15.606 15.695 green
					7.507 9.946 green
					8.343 8.162 green
					14.1 14.689 green
					14.047 14.824 green
					7.52 10.027 green
					8.446 10.647 green
					8.053 10.244 green
					14.04 14.342 green
					14.336 15.131 green
					7.924 10.136 green
					13.353 13.818 green
					13.905 15.0 green
					12.303 13.21 green
					14.578 15.13 green
					0.012 0.003 blue
					0.029 0.152 blue
					0.041 0.189 blue
					0.033 0.17 blue
					0.033 0.183 blue
					0.032 0.187 blue
					0.298 0.511 blue
					0.032 0.181 blue
					0.021 0.115 blue
					0.036 0.176 blue
					0.02 0.12 blue
					0.076 0.181 blue
					0.034 0.177 blue
					0.032 0.192 blue
					0.035 0.188 blue
					0.027 0.177 blue
					0.039 0.227 blue
					0.055 0.175 blue
					0.015 0.069 blue
					0.069 0.246 blue
					0.037 0.215 blue
					0.015 0.054 blue
					0.015 0.076 blue
					0.017 0.1 blue
					0.015 0.075 blue
					0.036 0.193 blue
					0.072 0.209 blue
					0.037 0.158 blue
					0.015 0.076 blue
					0.02 0.117 blue
					0.016 0.086 blue
					0.054 0.17 blue
					0.038 0.179 blue
					0.033 0.168 blue
					0.016 0.087 blue
					0.056 0.295 blue
					0.061 0.291 blue
					0.076 0.341 blue
					0.343 0.746 blue
					0.077 0.457 blue
					0.198 0.605 blue
					0.128 0.554 blue
					2.501 3.106 blue
					0.055 0.265 blue
					0.3 0.689 blue
					0.455 0.916 blue
					0.105 0.461 blue
					0.41 0.694 blue
					0.169 0.607 blue
					0.085 0.486 blue
					0.178 0.637 blue
					1.862 2.251 blue
					0.095 0.373 blue
					0.429 0.78 blue
					0.821 1.205 blue
					0.263 0.708 blue
					0.375 0.901 blue
					0.269 0.672 blue
					0.118 0.494 blue
					0.256 0.703 blue
					0.181 0.594 blue
					0.097 0.535 blue
					0.688 1.207 blue
					0.08 0.376 blue
					0.062 0.392 blue
					0.074 0.233 blue
					0.193 0.516 blue
					0.973 1.36 blue
					0.392 0.584 blue
					0.105 0.525 blue
					0.038 0.201 blue
					0.557 1.053 blue
					0.161 0.358 blue
					0.049 0.29 blue
					0.089 0.407 blue
					0.823 1.103 blue
					0.068 0.355 blue
					0.272 0.701 blue
					0.03 0.171 blue
					0.066 0.264 blue
					0.046 0.17 blue
					0.069 0.406 blue
					0.064 0.372 blue
					0.865 1.066 blue
					0.031 0.126 blue
					0.071 0.267 blue
					0.035 0.19 blue
					0.077 0.201 blue
					0.037 0.271 blue
					0.041 0.248 blue
					0.033 0.143 blue
					0.069 0.222 blue
					0.036 0.179 blue
					0.066 0.278 blue
					0.061 0.376 blue
					0.037 0.224 blue
					0.049 0.307 blue
					0.071 0.212 blue
					0.032 0.158 blue
					0.054 0.25 blue
					0.041 0.194 blue
					0.023 0.107 blue
					0.073 0.179 blue
					0.068 0.355 blue
					0.056 0.287 blue
					0.069 0.36 blue
					0.04 0.13 blue
					0.081 0.416 blue
					0.024 0.047 blue
					0.024 0.053 blue
					0.016 0.04 blue
					0.009 0.026 blue
					0.016 0.071 blue
					0.021 0.064 blue
					0.065 0.146 blue
					0.02 0.101 blue
					0.034 0.063 blue
					0.01 0.025 blue
					0.088 0.15 blue
					0.033 0.132 blue
					0.019 0.07 blue
					0.023 0.069 blue
					0.036 0.094 blue
					0.056 0.135 blue
					0.021 0.078 blue
					0.017 0.085 blue
					0.023 0.062 blue
					0.053 0.115 blue
					0.035 0.1 blue
					0.009 0.044 blue
					0.008 0.024 blue
					0.018 0.097 blue
					0.017 0.066 blue
					0.041 0.085 blue
					0.021 0.068 blue
					0.041 0.106 blue
					0.02 0.071 blue
					0.018 0.092 blue
					0.013 0.029 blue
					0.022 0.039 blue
					0.027 0.011 blue
					0.051 0.05 blue
					0.242 0.249 blue
					0.202 0.196 blue
					0.198 0.192 blue
					0.973 0.92 blue
					0.2 0.238 blue
					5.731 5.848 blue
					0.175 0.175 blue
					0.583 1.774 blue
					6.264 6.535 blue
					0.148 0.134 blue
					0.194 0.234 blue
					1.081 1.157 blue
					73.965 74.857 blue
					0.924 1.043 blue
					104.158 106.694 blue
					0.233 0.235 blue
					0.173 0.194 blue
					0.183 0.335 blue
					0.148 0.157 blue
					0.438 1.638 blue
					0.812 0.821 blue
					0.418 1.646 blue
					1.085 1.089 blue
					0.398 1.638 blue
					0.722 1.239 blue
					11.304 11.395 blue
					4.918 4.917 blue
					0.113 0.105 blue
					0.827 1.568 blue
					0.172 0.181 blue
					0.151 0.151 blue
					0.965 0.96 blue
					0.015 0.012 blue
					0.129 0.13 blue
					0.949 0.999 blue
					1.704 5.184 blue
					0.19 0.198 blue
					0.888 0.962 blue
					0.942 0.961 blue
					0.828 0.862 blue
					0.966 0.971 blue
					1.078 1.094 blue
					0.17 0.179 blue
					0.189 0.201 blue
					0.235 0.261 blue
					0.165 0.21 blue
					4.427 4.497 blue
					19.851 20.617 blue
					0.035 0.039 blue
					0.809 0.852 blue
					0.177 0.174 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.003 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.002 0.003 blue
					0.002 0.004 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.002 0.008 blue
					0.001 0.003 blue
					0.001 0.004 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.002 0.017 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.005 blue
					0.002 0.003 blue
					0.003 0.004 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.011 blue
					0.002 0.004 blue
					0.001 0.004 blue
					0.002 0.004 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.003 0.004 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.005 blue
					0.001 0.004 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.005 blue
					0.001 0.003 blue
					0.001 0.006 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.001 0.004 blue
					0.001 0.002 blue
					0.002 0.004 blue
					0.002 0.004 blue
					0.001 0.003 blue
					0.001 0.023 blue
					0.003 0.004 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.002 0.004 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.001 0.004 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.001 0.006 blue
					0.001 0.004 blue
					0.002 0.015 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.003 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.002 blue
					0.001 0.006 blue
					0.001 0.002 blue
					0.002 0.004 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.003 0.02 blue
					0.003 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.006 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.004 blue
					0.001 0.002 blue
					0.001 0.004 blue
					0.002 0.004 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.004 0.012 blue
					0.001 0.003 blue
					0.001 0.006 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.002 0.004 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.008 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.016 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.005 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.003 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.002 0.002 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.002 0.015 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.003 0.003 blue
					0.003 0.002 blue
					0.001 0.005 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.023 blue
					0.001 0.003 blue
					0.003 0.004 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.003 0.003 blue
					0.001 0.002 blue
					0.001 0.007 blue
					0.002 0.004 blue
					0.001 0.005 blue
					0.001 0.003 blue
					0.003 0.003 blue
					0.002 0.004 blue
					0.002 0.003 blue
					0.001 0.004 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.001 0.005 blue
					0.001 0.002 blue
					0.001 0.004 blue
					0.002 0.003 blue
					0.002 0.005 blue
					0.002 0.005 blue
					0.002 0.003 blue
					0.002 0.005 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.003 0.003 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.006 blue
					0.001 0.004 blue
					0.003 0.003 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.006 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.001 0.004 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.001 0.004 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.006 blue
					0.002 0.006 blue
					0.003 0.003 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.003 0.004 blue
					0.001 0.005 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.009 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.002 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.007 blue
					0.001 0.01 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.008 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.003 0.004 blue
					0.002 0.003 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.003 0.003 blue
					0.001 0.005 blue
					0.001 0.002 blue
					0.001 0.006 blue
					0.002 0.007 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.003 0.002 blue
					0.003 0.005 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.004 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.07 0.061 blue
					0.108 0.113 blue
					0.155 0.173 blue
					0.167 0.18 blue
					0.017 0.041 blue
					0.017 0.039 blue
					0.017 0.046 blue
					0.015 0.042 blue
					0.019 0.042 blue
					0.018 0.045 blue
					0.016 0.041 blue
					0.02 0.044 blue
					0.033 0.044 blue
					0.019 0.04 blue
					0.018 0.04 blue
					0.017 0.041 blue
					0.016 0.042 blue
					0.021 0.038 blue
					0.02 0.044 blue
					0.02 0.04 blue
					0.02 0.041 blue
					0.019 0.043 blue
					0.024 0.039 blue
					0.024 0.039 blue
					0.018 0.042 blue
					0.015 0.043 blue
					0.019 0.037 blue
					0.016 0.041 blue
					0.017 0.043 blue
					0.019 0.038 blue
					0.017 0.041 blue
					0.024 0.039 blue
					0.02 0.041 blue
					0.02 0.041 blue
					0.019 0.048 blue
					0.016 0.048 blue
					0.024 0.042 blue
					0.02 0.063 blue
					0.017 0.044 blue
					0.017 0.038 blue
					0.017 0.046 blue
					0.017 0.051 blue
					0.02 0.044 blue
					0.016 0.046 blue
					0.016 0.042 blue
					0.016 0.047 blue
					0.019 0.033 blue
					0.028 0.037 blue
					0.017 0.03 blue
					0.016 0.036 blue
					0.017 0.044 blue
					0.02 0.037 blue
					0.017 0.038 blue
					0.021 0.04 blue
					0.016 0.028 blue
					0.021 0.043 blue
					0.019 0.036 blue
					0.017 0.031 blue
					0.018 0.041 blue
					0.018 0.036 blue
					0.016 0.042 blue
					0.017 0.036 blue
					0.016 0.041 blue
					0.023 0.033 blue
					0.016 0.036 blue
					0.019 0.045 blue
					0.018 0.033 blue
					0.02 0.049 blue
					0.019 0.041 blue
					0.017 0.049 blue
					0.017 0.03 blue
					0.017 0.045 blue
					0.015 0.047 blue
					0.021 0.035 blue
					0.017 0.039 blue
					0.015 0.042 blue
					0.024 0.04 blue
					0.016 0.035 blue
					0.023 0.034 blue
					0.022 0.04 blue
					0.017 0.038 blue
					0.018 0.043 blue
					0.02 0.033 blue
					0.015 0.033 blue
					0.015 0.048 blue
					0.018 0.028 blue
					0.018 0.046 blue
					0.019 0.029 blue
					0.017 0.032 blue
					0.016 0.041 blue
					0.018 0.037 blue
					0.019 0.042 blue
					0.018 0.028 blue
					0.016 0.048 blue
					0.024 0.049 blue
					0.016 0.037 blue
					0.016 0.056 blue
					0.017 0.033 blue
					0.017 0.042 blue
					0.023 0.037 blue
					0.02 0.037 blue
					0.027 0.038 blue
					0.016 0.028 blue
					0.02 0.044 blue
					0.019 0.032 blue
					0.02 0.042 blue
					0.017 0.029 blue
					0.026 0.034 blue
					0.02 0.046 blue
					0.021 0.031 blue
					0.021 0.049 blue
					0.019 0.034 blue
					0.019 0.036 blue
					0.024 0.045 blue
					0.016 0.039 blue
					0.019 0.039 blue
					0.018 0.045 blue
					0.019 0.031 blue
					0.025 0.044 blue
					0.017 0.042 blue
					0.017 0.04 blue
					0.021 0.033 blue
					0.016 0.04 blue
					0.016 0.042 blue
					0.017 0.038 blue
					0.017 0.046 blue
					0.017 0.034 blue
					0.022 0.043 blue
					0.02 0.044 blue
					0.017 0.044 blue
					0.018 0.041 blue
					0.017 0.039 blue
					0.017 0.04 blue
					0.016 0.039 blue
					0.018 0.044 blue
					0.019 0.032 blue
					0.021 0.044 blue
					0.022 0.038 blue
					0.016 0.034 blue
					0.02 0.04 blue
					0.02 0.038 blue
					0.018 0.041 blue
					0.019 0.032 blue
					0.023 0.047 blue
					0.018 0.03 blue
					0.017 0.038 blue
					0.02 0.04 blue
					0.018 0.037 blue
					0.018 0.047 blue
					0.019 0.03 blue
					0.025 0.041 blue
					0.017 0.043 blue
					0.018 0.036 blue
					0.019 0.051 blue
					0.019 0.039 blue
					0.017 0.046 blue
					0.015 0.036 blue
					0.016 0.035 blue
					0.019 0.042 blue
					0.019 0.041 blue
					0.024 0.035 blue
					0.019 0.044 blue
					0.016 0.035 blue
					0.019 0.039 blue
					0.024 0.034 blue
					0.017 0.041 blue
					0.024 0.044 blue
					0.021 0.033 blue
					0.021 0.04 blue
					0.02 0.031 blue
					0.02 0.042 blue
					0.025 0.042 blue
					0.016 0.04 blue
					0.018 0.038 blue
					0.015 0.037 blue
					0.019 0.042 blue
					0.018 0.042 blue
					0.017 0.042 blue
					0.015 0.04 blue
					0.016 0.038 blue
					0.021 0.031 blue
					0.024 0.043 blue
					0.017 0.034 blue
					0.017 0.047 blue
					0.05 0.079 blue
					0.014 0.023 blue
					0.012 0.018 blue
					0.009 0.023 blue
					0.006 0.017 blue
					0.064 0.068 blue
					0.008 0.012 blue
					0.018 0.03 blue
					0.063 0.079 blue
					0.014 0.016 blue
					0.064 0.071 blue
					0.045 0.066 blue
					0.015 0.015 blue
					0.07 0.101 blue
					0.066 0.076 blue
					0.009 0.03 blue
					0.091 0.461 blue
					0.012 0.015 blue
					0.011 0.02 blue
					0.008 0.014 blue
					0.043 0.047 blue
					0.01 0.014 blue
					0.022 0.022 blue
					0.049 0.055 blue
					0.008 0.022 blue
					0.007 0.013 blue
					0.056 0.053 blue
					0.045 0.05 blue
					0.011 0.015 blue
					0.019 0.015 blue
					0.013 0.038 blue
					0.039 0.047 blue
					0.046 0.054 blue
					0.072 0.079 blue
					0.01 0.028 blue
					0.038 0.021 blue
					0.013 0.028 blue
					0.031 0.902 blue
					0.043 0.048 blue
					0.011 0.013 blue
					0.01 0.011 blue
					0.062 0.064 blue
					0.019 0.023 blue
					0.01 0.011 blue
					0.009 0.01 blue
					0.012 0.018 blue
					0.01 0.011 blue
					0.049 0.057 blue
					0.012 0.021 blue
					0.016 0.025 blue
					0.01 0.018 blue
					0.094 0.879 blue
					0.056 0.061 blue
					0.016 0.023 blue
					0.014 0.019 blue
					0.074 0.077 blue
					0.004 0.022 blue
					0.013 0.026 blue
					0.016 0.025 blue
					0.059 0.072 blue
					0.014 0.019 blue
					0.068 0.075 blue
					0.061 0.064 blue
					0.066 0.071 blue
					0.012 0.013 blue
					0.011 0.017 blue
					0.054 0.065 blue
					0.013 0.024 blue
					0.015 0.035 blue
					0.057 0.069 blue
					0.004 0.007 blue
					0.014 0.018 blue
					0.003 0.004 blue
					0.001 0.005 blue
					0.006 0.006 blue
					0.006 0.008 blue
					0.005 0.006 blue
					0.001 0.003 blue
					0.012 0.016 blue
					0.01 0.011 blue
					0.0 0.002 blue
					0.007 0.009 blue
					0.002 0.016 blue
					0.008 0.017 blue
					0.005 0.007 blue
					0.016 0.018 blue
					0.011 0.014 blue
					0.0 0.003 blue
					0.001 0.004 blue
					0.002 0.007 blue
					0.001 0.002 blue
					0.002 0.005 blue
					0.006 0.01 blue
					0.002 0.004 blue
					0.001 0.007 blue
					0.001 0.003 blue
					0.001 0.006 blue
					0.007 0.011 blue
					0.007 0.009 blue
					0.008 0.01 blue
					0.003 0.022 blue
					0.001 0.003 blue
					0.017 0.023 blue
					0.003 0.025 blue
					0.009 0.01 blue
					0.011 0.04 blue
					0.003 0.007 blue
					0.017 0.018 blue
					0.002 0.005 blue
					0.0 0.029 blue
					0.004 0.014 blue
					0.009 0.027 blue
					0.002 0.003 blue
					0.003 0.008 blue
					0.001 0.005 blue
					0.011 0.015 blue
					0.009 0.01 blue
					0.005 0.007 blue
					0.012 0.012 blue
					0.017 0.021 blue
					0.0 0.002 blue
					0.002 0.004 blue
					0.001 0.006 blue
					0.014 0.021 blue
					0.001 0.002 blue
					0.016 0.023 blue
					0.028 0.03 blue
					0.004 0.007 blue
					0.003 0.005 blue
					0.006 0.016 blue
					0.001 0.005 blue
					0.002 0.005 blue
					0.006 0.011 blue
					0.007 0.008 blue
					0.004 0.023 blue
					0.004 0.006 blue
					0.004 0.006 blue
					0.0 0.002 blue
					0.004 0.01 blue
					0.002 0.004 blue
					0.016 0.026 blue
					0.004 0.006 blue
					0.003 0.004 blue
					0.013 0.016 blue
					0.0 0.005 blue
					0.0 0.005 blue
					0.0 0.002 blue
					0.003 0.006 blue
					0.013 0.016 blue
					0.002 0.007 blue
					0.023 0.012 blue
					0.003 0.005 blue
					0.03 0.021 blue
					0.001 0.004 blue
					0.012 0.014 blue
					0.001 0.002 blue
					0.015 0.016 blue
					0.006 0.007 blue
					0.001 0.008 blue
					0.004 0.008 blue
					0.004 0.007 blue
					0.001 0.003 blue
					0.001 0.006 blue
					0.008 0.012 blue
					0.001 0.003 blue
					0.031 0.011 blue
					0.004 0.006 blue
					0.009 0.01 blue
					0.029 0.005 blue
					0.017 0.023 blue
					0.002 0.004 blue
					0.003 0.007 blue
					0.007 0.008 blue
					0.002 0.002 blue
					0.005 0.007 blue
					0.001 0.009 blue
					0.0 0.003 blue
					0.001 0.005 blue
					0.001 0.005 blue
					0.002 0.007 blue
					0.009 0.013 blue
					0.011 0.02 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.007 0.009 blue
					0.012 0.005 blue
					0.011 0.011 blue
					0.004 0.006 blue
					0.015 0.021 blue
					0.001 0.003 blue
					0.0 0.002 blue
					0.006 0.007 blue
					0.018 0.019 blue
					0.006 0.008 blue
					0.002 0.004 blue
					0.003 0.005 blue
					0.01 0.025 blue
					0.003 0.006 blue
					0.0 0.002 blue
					0.008 0.009 blue
					0.003 0.005 blue
					0.01 0.016 blue
					0.0 0.002 blue
					0.002 0.004 blue
					0.019 0.009 blue
					0.013 0.018 blue
					0.002 0.004 blue
					0.003 0.005 blue
					0.003 0.004 blue
					0.01 0.004 blue
					0.004 0.006 blue
					0.008 0.008 blue
					0.027 0.03 blue
					0.004 0.014 blue
					0.015 0.045 blue
					0.002 0.004 blue
					0.0 0.003 blue
					0.002 0.004 blue
					0.003 0.003 blue
					0.003 0.004 blue
					0.004 0.006 blue
					0.003 0.004 blue
					0.003 0.004 blue
					0.016 0.021 blue
					0.01 0.015 blue
					0.005 0.006 blue
					0.005 0.006 blue
					0.003 0.004 blue
					0.011 0.03 blue
					0.009 0.01 blue
					0.003 0.004 blue
					0.0 0.002 blue
					0.0 0.002 blue
					0.016 0.017 blue
					0.015 0.023 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.003 0.005 blue
					0.015 0.035 blue
					0.001 0.004 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.011 0.012 blue
					0.004 0.005 blue
					0.013 0.017 blue
					0.016 0.021 blue
					0.01 0.01 blue
					0.001 0.004 blue
					0.009 0.011 blue
					0.007 0.019 blue
					0.002 0.004 blue
					0.007 0.034 blue
					0.005 0.007 blue
					0.004 0.03 blue
					0.003 0.005 blue
					0.0 0.01 blue
					0.0 0.002 blue
					0.001 0.003 blue
					0.0 0.002 blue
					0.016 0.031 blue
					0.004 0.005 blue
					0.005 0.004 blue
					0.0 0.002 blue
					0.017 0.011 blue
					0.0 0.004 blue
					0.005 0.008 blue
					0.008 0.01 blue
					0.001 0.005 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.008 0.012 blue
					0.0 0.002 blue
					0.011 0.028 blue
					0.009 0.026 blue
					0.009 0.013 blue
					0.014 0.015 blue
					0.005 0.009 blue
					0.004 0.006 blue
					0.005 0.007 blue
					0.016 0.017 blue
					0.001 0.002 blue
					0.007 0.015 blue
					0.002 0.007 blue
					0.002 0.004 blue
					0.004 0.009 blue
					0.012 0.031 blue
					0.006 0.008 blue
					0.002 0.008 blue
					0.004 0.022 blue
					0.013 0.032 blue
					0.005 0.006 blue
					0.006 0.009 blue
					0.015 0.039 blue
					0.0 0.002 blue
					0.003 0.004 blue
					0.003 0.005 blue
					0.003 0.022 blue
					0.004 0.051 blue
					0.0 0.002 blue
					0.003 0.003 blue
					0.0 0.002 blue
					0.008 0.032 blue
					0.009 0.013 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.002 0.002 blue
					0.002 0.004 blue
					0.001 0.005 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.005 blue
					0.001 0.011 blue
					0.001 0.002 blue
					0.002 0.005 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.003 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.004 0.005 blue
					0.001 0.002 blue
					0.003 0.006 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.004 0.005 blue
					0.002 0.004 blue
					0.002 0.004 blue
					0.001 0.003 blue
					0.004 0.004 blue
					0.003 0.004 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.005 0.008 blue
					0.003 0.004 blue
					0.008 0.004 blue
					0.002 0.015 blue
					0.002 0.004 blue
					0.005 0.016 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.003 0.004 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.001 0.006 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.006 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.001 0.005 blue
					0.002 0.003 blue
					0.003 0.003 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.003 0.003 blue
					0.003 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.003 0.006 blue
					0.001 0.002 blue
					0.001 0.002 blue
					0.004 0.006 blue
					0.004 0.003 blue
					0.001 0.004 blue
					0.001 0.016 blue
					0.001 0.003 blue
					0.001 0.004 blue
					0.002 0.022 blue
					0.001 0.005 blue
					0.001 0.003 blue
					0.002 0.005 blue
					0.001 0.003 blue
					0.001 0.004 blue
					0.002 0.004 blue
					0.002 0.042 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.002 0.005 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.004 0.024 blue
					0.002 0.004 blue
					0.002 0.009 blue
					0.002 0.003 blue
					0.002 0.004 blue
					0.001 0.042 blue
					0.001 0.003 blue
					0.001 0.004 blue
					0.001 0.002 blue
					0.002 0.004 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.002 0.003 blue
					0.001 0.004 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.003 0.007 blue
					0.004 0.01 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.004 0.01 blue
					0.002 0.004 blue
					0.002 0.006 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.002 0.009 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.004 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.002 0.003 blue
					0.002 0.007 blue
					0.001 0.002 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.002 0.004 blue
					0.001 0.002 blue
					0.002 0.004 blue
					0.001 0.002 blue
					0.002 0.004 blue
					0.004 0.004 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.003 0.007 blue
					0.001 0.003 blue
					0.004 0.022 blue
					0.002 0.005 blue
					0.002 0.004 blue
					0.001 0.002 blue
					0.001 0.004 blue
					0.011 0.002 blue
					0.002 0.004 blue
					0.003 0.008 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.007 blue
					0.002 0.003 blue
					0.001 0.003 blue
					0.002 0.005 blue
					0.002 0.006 blue
					0.002 0.004 blue
					0.001 0.003 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.008 0.008 blue
					0.039 0.044 blue
					0.005 0.006 blue
					0.075 0.075 blue
					0.003 0.007 blue
					0.009 0.015 blue
					0.024 0.029 blue
					0.004 0.006 blue
					0.016 0.024 blue
					0.003 0.005 blue
					0.025 0.029 blue
					0.038 0.043 blue
					0.005 0.006 blue
					0.067 0.114 blue
					0.061 0.067 blue
					0.003 0.008 blue
					0.009 0.009 blue
					0.027 0.023 blue
					0.026 0.029 blue
					0.015 0.041 blue
					0.02 0.032 blue
					0.031 0.042 blue
					0.02 0.022 blue
					0.036 0.064 blue
					0.001 0.004 blue
					0.001 0.002 blue
					0.002 0.005 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.005 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.002 blue
					0.001 0.004 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.001 0.003 blue
					0.011 0.018 blue
					0.015 0.03 blue
					0.018 0.017 blue
					0.015 0.025 blue
					0.014 0.033 blue
					0.018 0.017 blue
					0.006 0.008 blue
					0.029 0.023 blue
					0.012 0.024 blue
					0.017 0.024 blue
					0.009 0.011 blue
					0.008 0.009 blue
					0.004 0.044 blue
					0.019 0.02 blue
					0.007 0.021 blue
					0.014 0.016 blue
					0.018 0.033 blue
					0.022 0.018 blue
					0.017 0.023 blue
					0.013 0.031 blue
					0.019 0.019 blue
					0.004 0.007 blue
					0.009 0.023 blue
					0.012 0.012 blue
					0.02 0.015 blue
					0.005 0.006 blue
					0.046 0.053 blue
					0.047 0.051 blue
					0.045 0.055 blue
					0.045 0.055 blue
					0.047 0.059 blue
					0.049 0.065 blue
					0.049 0.062 blue
					0.041 0.059 blue
					0.057 0.061 blue
					0.053 0.055 blue
					0.053 0.057 blue
					0.05 0.06 blue
					0.049 0.054 blue
					0.055 0.068 blue
					0.045 0.054 blue
					0.055 0.065 blue
					0.056 0.063 blue
					0.064 0.072 blue
					0.051 0.061 blue
					0.063 0.071 blue
					0.055 0.063 blue
					0.057 0.064 blue
					0.054 0.063 blue
					0.061 0.071 blue
					0.059 0.061 blue
					0.056 0.063 blue
					0.058 0.076 blue
					0.057 0.062 blue
					0.064 0.074 blue
					0.055 0.064 blue
					0.052 0.058 blue
					0.055 0.059 blue
					0.055 0.062 blue
					0.064 0.073 blue
					0.063 0.07 blue
					0.051 0.06 blue
					0.062 0.07 blue
					0.06 0.076 blue
					0.052 0.06 blue
					0.058 0.067 blue
					0.042 0.05 blue
					0.062 0.085 blue
					0.054 0.063 blue
					0.061 0.068 blue
					0.058 0.067 blue
					0.064 0.072 blue
					0.111 0.128 blue
					0.146 0.164 blue
					0.183 0.203 blue
					0.11 0.13 blue
					0.121 0.137 blue
					0.144 0.16 blue
					0.157 0.18 blue
					0.156 0.176 blue
					0.126 0.148 blue
					0.151 0.149 blue
					0.121 0.129 blue
					0.148 0.168 blue
					0.161 0.181 blue
					0.107 0.131 blue
					0.179 0.192 blue
					0.16 0.179 blue
					0.113 0.131 blue
					0.123 0.137 blue
					0.14 0.152 blue
					0.125 0.145 blue
					0.16 0.183 blue
					0.187 0.199 blue
					0.179 0.196 blue
					0.122 0.146 blue
					0.15 0.168 blue
					0.144 0.16 blue
					0.115 0.17 blue
					0.165 0.181 blue
					0.164 0.179 blue
					0.107 0.127 blue
				};
			\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
			\begin{axis}[
				scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
				ylabel=certifying (time),
				xlabel=default (time),
				xmode=log,
				ymode=log,
				grid=both,
				grid style={line width=.1pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				minor tick num=5,
				xtick={0.001,0.01,0.1,1,10,100,1000},
				ytick={0.001,0.01,0.1,1,10,100,1000},
			]
				\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x });
				\addplot[scatter,only marks, scatter src=explicit symbolic]%
				table[meta=label] {
					x y label
					1000 1000 peer
					0.095 0.102 green
					0.008 0.023 green
					0.026 0.048 green
					1.088 3.848 green
					0.074 27.457 green
					0.094 0.111 green
					0.45 400.096 green
					0.128 0.182 green
					0.015 0.02 green
					0.095 0.115 green
					2.498 5465.944 green
					0.049 0.064 green
					0.081 0.123 green
					0.073 0.139 green
					0.001 0.018 green
					0.354 958.314 green
					0.107 0.842 green
					9.127 38.94 green
					0.002 0.019 green
					0.034 11.558 green
					0.015 0.026 green
					0.024 0.033 green
					0.641 0.664 green
					0.003 0.026 green
					0.031 0.048 green
					0.017 0.039 green
					0.015 0.04 green
					0.067 0.089 green
					0.023 0.032 green
					0.522 8.87 green
					4.824 38.049 green
					0.047 0.234 green
					0.014 0.031 green
					0.548 0.702 green
					4.691 5.387 green
					0.009 0.048 green
					0.003 0.02 green
					0.366 0.497 green
					1.177 1.274 green
					1.909 2.018 green
					0.02 0.033 green
					0.989 1.025 green
					0.001 0.018 green
					0.036 0.054 green
					0.007 0.03 green
					0.431 311.138 green
					0.015 0.059 green
					0.019 0.611 green
					2.11 2.16 green
					0.022 0.025 green
					0.209 2.329 green
					0.097 0.108 green
					8.387 88.496 green
					0.09 0.11 green
					0.022 0.024 green
					0.15 0.241 green
					0.079 0.09 green
					0.008 0.009 green
					0.231 23.603 green
					160.639 10800.0 green
					0.017 0.057 green
					0.026 0.039 green
					0.117 0.129 green
					0.047 0.054 green
					0.013 0.02 green
					0.139 0.143 green
					0.058 0.063 green
					0.02 0.029 green
					0.02 0.028 green
					0.053 0.056 green
					0.116 0.134 green
					0.164 0.4 green
					0.031 0.161 green
					0.028 0.026 green
					0.011 0.012 green
					1.51 13.733 green
					1.017 1.51 green
					0.022 0.023 green
					0.02 0.031 green
					0.001 0.003 green
					11.882 6849.021 green
					0.112 0.112 green
					0.002 0.003 green
					26.615 10800.0 green
					0.646 439.217 green
					0.043 0.005 green
					0.016 0.016 green
					0.014 0.013 green
					0.313 295.229 green
					1.343 1712.776 green
					0.023 0.028 green
					0.016 0.018 green
					1.117 10786.623 green
					0.018 0.591 green
					0.279 0.272 green
					0.025 0.029 green
					0.187 0.218 green
					0.032 0.057 green
					0.413 0.924 green
					0.09 0.094 green
					0.019 0.042 green
					0.325 2.17 green
					0.108 0.116 green
					0.01 0.012 green
					0.023 0.046 green
					0.012 0.013 green
					1.585 56.545 green
					1.258 2.515 green
					0.092 0.099 green
					1.247 1.339 green
					0.061 0.067 green
					0.008 0.007 green
					0.014 0.016 green
					0.508 4.246 green
					0.033 0.036 green
					0.111 0.103 green
					0.028 0.03 green
					0.012 0.013 green
					0.038 6.343 green
					0.035 0.018 green
					0.216 0.707 green
					0.034 0.035 green
					0.566 0.575 green
					0.012 0.02 green
					0.009 0.013 green
					0.29 19.694 green
					0.032 18.963 green
					1.362 1.394 green
					1.116 1.196 green
					0.216 0.223 green
					0.109 1.044 green
					0.049 0.358 green
					0.315 1.641 green
					0.239 0.24 green
					0.02 0.087 green
					0.149 14.235 green
					0.002 0.003 green
					0.016 0.021 green
					2.81 268.432 green
					54.754 2491.301 green
					0.405 67.257 green
					0.022 0.023 green
					0.03 0.034 green
					0.018 0.041 green
					0.04 0.065 green
					5.905 131.836 green
					0.015 0.016 blue
					0.689 0.727 blue
					0.249 0.253 blue
					1.131 55.601 blue
					4.336 4.555 blue
					0.232 0.226 blue
					4738.054 5083.798 blue
					0.021 0.012 blue
					0.221 0.295 blue
					0.022 0.023 blue
					0.06 0.033 blue
					0.01 0.005 blue
					187.779 189.743 blue
					2.002 3.288 blue
					0.315 0.32 blue
					0.046 0.035 blue
					0.043 0.052 blue
					0.019 0.021 blue
					0.124 0.205 blue
					0.788 2.507 blue
					0.089 0.102 blue
					0.041 0.037 blue
					0.03 0.031 blue
					6.65 9.683 blue
					0.023 0.025 blue
					0.028 0.033 blue
					0.035 0.04 blue
					0.042 0.037 blue
					0.132 0.135 blue
					0.982 1.259 blue
					0.015 0.033 blue
					0.031 0.032 blue
					0.004 0.015 blue
					0.016 0.019 blue
					1.124 56.441 blue
					0.056 0.059 blue
					1.232 2.54 blue
					0.033 0.034 blue
					0.574 0.59 blue
					0.014 0.029 blue
					0.016 0.014 blue
					0.012 0.014 blue
					0.087 0.105 blue
					0.012 0.011 blue
					0.537 0.677 blue
					0.121 0.128 blue
					0.119 0.123 blue
					0.088 0.09 blue
					0.451 3.228 blue
					0.006 0.008 blue
					0.216 0.217 blue
					0.024 0.025 blue
					0.313 0.334 blue
					0.001 0.003 blue
					0.023 0.026 blue
					0.018 0.019 blue
					0.032 0.013 blue
					0.016 0.015 blue
					8.352 8.411 blue
					0.032 0.079 blue
					0.114 0.114 blue
					0.449 3.481 blue
					0.585 0.589 blue
					0.059 0.051 blue
					0.012 0.02 blue
					0.075 0.133 blue
					0.018 0.065 blue
					0.455 3.227 blue
					0.024 0.024 blue
					0.027 0.044 blue
					0.184 0.182 blue
					0.591 0.676 blue
					1.24 2.503 blue
					0.143 0.124 blue
					4725.392 4865.381 blue
					0.012 0.014 blue
					0.23 0.177 blue
					0.008 0.01 blue
					0.02 0.017 blue
					0.024 0.038 blue
					0.089 0.093 blue
					0.002 0.003 blue
					0.402 0.68 blue
					0.938 1.223 blue
					0.184 0.218 blue
					0.015 0.023 blue
					1.369 1.408 blue
					0.01 0.011 blue
					0.037 0.039 blue
					0.634 0.65 blue
					14.705 14.996 blue
					0.134 0.333 blue
					2.089 2.122 blue
					0.09 0.098 blue
					0.014 0.014 blue
					0.416 3.489 blue
					0.037 0.038 blue
					0.018 0.031 blue
					0.046 0.104 blue
					0.494 1.274 blue
					0.028 0.065 blue
					0.291 0.301 blue
					0.915 0.918 blue
					0.002 0.003 blue
					0.083 0.251 blue
					0.214 0.702 blue
					0.055 0.151 blue
					0.087 0.092 blue
					6.457 7.016 blue
					0.021 0.027 blue
					0.114 0.136 blue
					1.123 1.151 blue
					0.02 0.022 blue
					0.004 0.005 blue
					0.023 0.019 blue
					0.009 0.009 blue
					0.221 0.288 blue
					0.023 0.028 blue
					0.836 1.492 blue
					0.019 0.012 blue
					0.031 0.041 blue
					0.216 0.232 blue
					0.035 0.141 blue
					0.564 0.572 blue
					0.027 0.037 blue
					185.721 183.648 blue
					0.653 1.143 blue
					0.971 1.041 blue
					2.031 3.292 blue
					0.705 0.715 blue
					0.898 2.667 blue
					0.031 0.029 blue
					0.022 0.054 blue
					0.015 0.017 blue
					0.106 0.255 blue
					0.019 0.023 blue
					0.041 0.044 blue
					10.576 11.067 blue
					0.032 0.033 blue
					15.007 15.068 blue
					0.02 0.026 blue
					0.01 0.042 blue
					0.022 0.054 blue
					0.023 0.036 blue
					0.125 0.126 blue
					0.038 0.02 blue
					0.025 0.027 blue
					0.007 0.008 blue
					0.01 0.011 blue
					0.002 0.003 blue
					0.072 0.144 blue
					0.011 0.01 blue
					0.86 1.47 blue
					0.019 0.015 blue
					0.029 0.032 blue
					0.089 0.094 blue
					0.02 0.029 blue
					0.054 0.152 blue
					0.083 0.109 blue
					0.009 0.012 blue
					0.09 0.101 blue
					0.051 0.086 blue
					0.179 0.207 blue
					0.019 0.019 blue
					0.01 0.011 blue
					0.694 1.126 blue
					0.003 0.008 blue
					0.004 0.007 blue
					127.585 126.984 blue
					0.018 0.019 blue
					0.026 0.02 blue
					0.022 0.024 blue
					0.496 1.308 blue
					0.051 0.093 blue
					3.496 3.863 blue
					0.024 0.028 blue
					0.021 0.034 blue
					0.01 0.008 blue
					0.008 0.009 blue
					0.095 0.093 blue
					0.029 0.033 blue
					8.327 8.402 blue
					0.032 0.026 blue
					1.888 1.887 blue
					0.008 0.012 blue
					0.677 0.869 blue
					0.048 0.104 blue
					0.012 0.018 blue
					0.028 0.024 blue
					28.237 30.348 blue
					0.471 0.625 blue
					0.104 0.82 blue
					0.02 0.032 blue
					0.091 0.093 blue
					0.029 0.013 blue
					0.024 0.046 blue
					0.071 0.105 blue
					0.031 0.034 blue
					0.012 0.019 blue
					0.09 0.091 blue
					0.122 0.132 blue
					0.018 0.023 blue
					0.398 0.687 blue
					0.058 0.129 blue
					0.68 0.647 blue
					0.179 0.167 blue
					0.086 0.088 blue
					0.019 0.012 blue
					0.022 0.033 blue
					0.016 0.02 blue
					0.339 0.44 blue
					0.406 0.845 blue
					1.329 1.331 blue
					0.011 0.015 blue
					0.341 0.372 blue
					0.125 0.171 blue
					0.012 0.013 blue
					0.015 0.018 blue
					0.02 0.017 blue
					2.029 2.119 blue
					0.162 0.199 blue
					0.027 0.021 blue
					0.019 0.021 blue
					0.1 0.825 blue
					0.018 0.02 blue
					0.023 0.024 blue
					0.001 0.002 blue
					0.113 0.172 blue
					0.032 0.051 blue
					10.082 11.563 blue
					0.003 0.005 blue
					0.311 0.332 blue
					0.01 0.011 blue
					0.671 0.863 blue
					0.069 0.078 blue
					0.015 0.018 blue
					0.078 0.123 blue
					0.167 0.176 blue
					0.122 0.168 blue
					0.035 0.005 blue
					0.042 0.053 blue
					9.232 9.402 blue
					0.023 0.025 blue
					0.169 0.197 blue
					0.002 0.003 blue
					0.134 0.138 blue
					0.163 0.181 blue
					0.228 0.24 blue
					132.873 128.175 blue
					0.022 0.018 blue
					0.9 0.891 blue
					0.408 0.836 blue
					0.113 0.329 blue
					0.017 0.021 blue
					0.975 0.997 blue
					0.05 0.054 blue
					0.892 2.648 blue
					0.018 0.024 blue
					0.104 0.107 blue
					0.027 0.03 blue
					4.367 4.525 blue
					0.062 0.066 blue
					0.151 0.805 blue
					6.45 6.867 blue
					0.035 0.027 blue
					0.048 0.046 blue
					0.078 0.105 blue
					0.012 0.036 blue
					0.051 0.053 blue
					0.221 0.704 blue
					0.417 0.936 blue
					3.6 3.83 blue
					0.011 0.013 blue
					0.073 0.123 blue
					0.07 0.071 blue
					1.867 1.912 blue
					0.113 0.172 blue
					0.038 0.125 blue
					0.002 0.004 blue
					0.507 0.571 blue
					0.029 0.035 blue
					0.123 0.271 blue
					0.017 0.03 blue
					0.03 0.032 blue
					0.07 0.081 blue
					0.228 0.245 blue
					0.024 0.029 blue
					0.019 0.022 blue
					0.06 0.092 blue
					9.222 9.373 blue
					6.459 9.742 blue
					0.035 0.037 blue
					0.006 0.041 blue
					4.803 5.302 blue
					0.021 0.013 blue
				};
			\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\caption{
		Distribution of running times for \papilo for parameter settings default and certifying on \pb (left) and \miplib (right).
		Each $\times$ marks an instance.
		The $y$-axis gives the time for presolving with certifying and
		the $x$-axis gives the time for default presolving.
		Green $+$ mark optimization instances and blue $\times$ mark decision instances.
	}\label{fig:default_vs_certify}
\end{figure}


\begin{figure}[ht]
	\centering
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
			\begin{axis}[
				scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
				ylabel=\veripb+\papilo (time),
				xlabel=\papilo (time),
				xmode=log,
				ymode=log,
				grid=both,
				grid style={line width=.1pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				minor tick num=5,
				xtick={0.01,0.1,1,10,100,1000},
				ytick={0.01,0.1,1,10,100,1000,10000},
			]
				\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x });
				\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x + 10});
				\addplot[scatter,only marks, scatter src=explicit symbolic]
				table[meta=label] {
					x y label
					1000 1000 peer
					0.058 2.078 green
					0.02 1.02 green
					0.07 2.83 green
					0.112 4.312 green
					0.023 1.133 green
					1.024 33.593999999999994 green
					1.108 36.27799999999999 green
					0.446 18.136 green
					0.941 28.921 green
					0.508 19.758 green
					0.982 34.19199999999999 green
					1.402 44.292 green
					1.07 33.19 green
					0.479 18.709 green
					1.031 33.980999999999995 green
					0.469 20.129 green
					1.02 33.29 green
					1.104 35.443999999999996 green
					1.289 41.379 green
					0.468 18.328 green
					1.16 37.349999999999994 green
					0.501 19.561 green
					1.203 38.573 green
					1.08 35.879999999999995 green
					0.465 18.404999999999998 green
					1.039 32.669 green
					1.176 38.146 green
					0.524 20.124000000000002 green
					0.516 13.406 green
					1.12 34.629999999999995 green
					1.442 46.082 green
					1.447 45.827 green
					0.309 9.418999999999999 green
					1.397 45.657 green
					0.367 11.076999999999998 green
					1.338 43.568 green
					0.392 13.402 green
					0.272 7.752000000000001 green
					0.852 22.822 green
					1.089 43.29899999999999 green
					0.674 27.284 green
					1.49 46.82 green
					0.645 15.925 green
					1.675 53.855 green
					0.603 24.453000000000003 green
					1.236 40.25599999999999 green
					1.378 212.148 green
					1.372 152.15200000000002 green
					1.445 211.745 green
					1.798 209.648 green
					2.002 290.672 green
					1.141 138.261 green
					1.743 324.793 green
					1.467 193.117 green
					3.119 297.25900000000007 green
					3.341 204.10100000000003 green
					1.102 303.61199999999997 green
					1.65 343.03 green
					1.082 150.172 green
					1.485 181.04500000000002 green
					1.702 301.732 green
					0.934 147.174 green
					1.466 276.73600000000005 green
					2.736 276.19599999999997 green
					3.586 283.61600000000004 green
					1.676 320.746 green
					2.139 296.069 green
					1.239 131.609 green
					1.056 249.216 green
					0.948 273.068 green
					1.346 175.466 green
					1.476 213.01600000000002 green
					1.861 204.131 green
					2.255 296.48499999999996 green
					0.996 267.996 green
					1.282 283.342 green
					2.147 234.697 green
					1.261 214.18099999999998 green
					0.957 221.877 green
					1.702 256.192 green
					2.347 220.097 green
					1.347 299.817 green
					1.419 158.43900000000002 green
					1.896 215.736 green
					1.043 247.243 green
					2.003 158.13299999999998 green
					2.987 271.987 green
					1.653 250.313 green
					2.797 248.197 green
					1.289 194.429 green
					2.308 265.368 green
					3.1 203.0 green
					1.422 211.272 green
					1.442 309.082 green
					2.019 257.039 green
					0.955 179.26500000000001 green
					1.408 276.498 green
					3.25 216.44000000000003 green
					1.555 185.385 green
					1.163 293.89300000000003 green
					1.222 155.452 green
					0.242 14.692 green
					0.408 14.787999999999998 green
					0.375 10.885000000000002 green
					0.346 10.686 green
					0.462 10.332 green
					0.575 18.095 green
					0.456 12.936 green
					0.506 19.306 green
					0.355 18.135 green
					0.842 20.092 green
					0.3 10.22 green
					0.512 15.972 green
					0.346 14.735999999999999 green
					0.42 11.780000000000001 green
					0.202 12.052 green
					0.353 8.583 green
					0.458 12.088000000000001 green
					0.464 17.823999999999998 green
					0.371 14.251000000000001 green
					0.347 15.806999999999999 green
					0.258 11.597999999999999 green
					0.367 14.107 green
					0.36 17.88 green
					0.314 18.864 green
					0.284 10.424000000000001 green
					0.745 22.265 green
					0.322 14.371999999999998 green
					0.368 23.328 green
					0.357 11.227 green
					0.784 142.454 green
					1.416 144.376 green
					1.363 127.143 green
					1.259 191.87899999999996 green
					1.695 110.77499999999999 green
					1.086 134.19600000000003 green
					1.073 131.483 green
					1.211 131.88100000000003 green
					1.611 125.051 green
					0.91 124.97 green
					1.672 163.862 green
					0.865 147.965 green
					1.644 159.38400000000001 green
					1.403 162.213 green
					1.569 123.489 green
					1.016 123.92600000000002 green
					1.008 172.008 green
					1.945 124.865 green
					1.507 81.747 green
					0.691 113.481 green
					1.017 74.647 green
					1.073 85.833 green
					1.86 123.52 green
					1.804 126.28399999999999 green
					2.586 154.00600000000003 green
					0.829 99.70899999999999 green
					1.909 133.689 green
					1.318 118.548 green
					1.901 135.101 green
					0.971 126.421 green
					1.151 124.431 green
					0.696 113.146 green
					0.755 45.685 green
					0.578 52.348000000000006 green
					0.788 31.138 green
					0.768 39.388 green
					0.806 46.916 green
					0.689 61.879 green
					0.749 36.889 green
					0.897 57.717 green
					0.649 60.93900000000001 green
					0.825 40.705000000000005 green
					0.878 69.10799999999999 green
					1.525 48.934999999999995 green
					0.758 47.508 green
					0.916 62.32599999999999 green
					1.082 35.792 green
					0.805 71.44500000000001 green
					0.663 55.513 green
					0.69 45.1 green
					0.887 92.107 green
					0.593 48.803 green
					0.686 56.386 green
					1.356 54.476 green
					1.228 59.188 green
					0.121 2.731 green
					8.28 1530.3799999999999 green
					0.046 2.586 green
					1.797 1106.977 green
					0.589 4.779 green
					0.046 6.566 green
					0.161 129.311 green
					0.117 2.447 green
					2.122 52.852 green
					2.501 20.401 green
					0.064 14.094000000000001 green
					1.17 62.760000000000005 green
					0.036 3.386 green
					0.338 1.7080000000000002 green
					0.39 72.75000000000001 green
					0.038 1.1380000000000001 green
					0.041 4.091 green
					2.787 2300.807 green
					23.582 754.5020000000001 green
					0.373 214.713 green
					0.164 1.4040000000000001 green
					11.829 300.389 green
					12.797 9351.607 green
					5.463 11.912999999999997 green
					0.041 1.6709999999999998 green
					0.045 1.705 green
					0.043 1.6929999999999998 green
					0.042 1.7620000000000002 green
					0.04 1.66 green
					0.044 1.644 green
					0.066 1.226 green
					0.043 1.683 green
					0.04 1.69 green
					0.051 1.781 green
					0.056 1.256 green
					0.043 1.6929999999999998 green
					0.041 1.681 green
					0.043 1.6929999999999998 green
					0.049 1.6989999999999998 green
					0.052 1.192 green
					0.047 1.6969999999999998 green
					0.059 1.3989999999999998 green
					0.059 1.3789999999999998 green
					0.061 2.851 green
					0.171 19.660999999999998 green
					0.157 15.807 green
					0.117 7.757 green
					1.551 238.23099999999997 green
					2.429 544.9989999999999 green
					0.87 149.99 green
					2.883 494.933 green
					2.445 545.865 green
					2.569 563.1389999999999 green
					3.108 573.6779999999999 green
					1.48 222.52 green
					2.783 555.563 green
					2.46 544.9100000000001 green
					2.814 596.5139999999999 green
					2.856 566.2760000000001 green
					1.466 212.06600000000003 green
					2.902 574.3620000000001 green
					2.627 569.307 green
					1.634 397.85400000000004 green
					2.025 399.885 green
					1.531 234.83100000000002 green
					2.182 458.502 green
					3.248 598.128 green
					28.712 4843.262000000001 green
					11.544 7456.934 green
					0.384 641.424 green
					36.375 3765.355 green
					0.366 352.436 green
					29.009 4844.269 green
					0.415 144.62499999999997 green
					0.365 277.815 green
					0.351 177.03099999999998 green
					0.316 81.456 green
					0.357 283.59700000000004 green
					35.499 3785.0689999999995 green
					12.209 1440.629 green
					0.369 278.439 green
					35.987 3742.447 green
					0.365 280.285 green
					0.296 276.986 green
					0.422 631.462 green
					0.423 637.2529999999999 green
					35.261 3777.121 green
					14.692 974.482 green
					0.353 174.023 green
					0.308 81.84800000000001 green
					0.313 80.233 green
					43.199 2608.259 green
					36.104 3766.0539999999996 green
					44.41 2601.16 green
					11.952 7393.572 green
					28.889 4847.099 green
					0.35 369.63 green
					10.624 10800 green
					10.108 10800 green
					14.974 9269.584 green
					10.275 10800 green
					2.893 9251.203 green
					9.598 10800 green
					15.048 9182.888 green
					9.713 10800 green
					15.529 9238.409 green
					15.695 1148.8749999999998 green
					9.946 10800 green
					8.162 10800 green
					14.689 5634.399 green
					14.824 9219.003999999999 green
					10.027 10800 green
					10.647 10800 green
					10.244 10800 green
					14.342 9220.181999999999 green
					15.131 9227.141 green
					10.136 10800 green
					15.0 9236.660000000002 green
					15.13 9243.76 green
					0.152 28.582 blue
					0.189 35.638999999999996 blue
					0.17 31.28 blue
					0.183 37.452999999999996 blue
					0.187 34.626999999999995 blue
					0.511 62.681000000000004 blue
					0.181 34.92099999999999 blue
					0.115 20.414999999999996 blue
					0.176 31.206 blue
					0.12 20.180000000000003 blue
					0.181 23.101 blue
					0.177 34.516999999999996 blue
					0.192 33.932 blue
					0.188 34.538000000000004 blue
					0.177 33.857 blue
					0.227 46.266999999999996 blue
					0.175 27.555 blue
					0.069 10.289000000000001 blue
					0.246 43.476 blue
					0.215 45.165000000000006 blue
					0.054 7.224 blue
					0.076 10.616 blue
					0.1 17.110000000000003 blue
					0.075 11.504999999999999 blue
					0.193 37.462999999999994 blue
					0.209 34.349000000000004 blue
					0.158 29.618000000000002 blue
					0.076 12.226 blue
					0.117 19.747 blue
					0.086 14.346 blue
					0.17 25.55 blue
					0.179 40.739 blue
					0.168 32.998 blue
					0.087 14.286999999999999 blue
					0.295 73.005 blue
					0.291 71.61099999999999 blue
					0.341 96.28099999999999 blue
					0.746 234.47600000000003 blue
					0.457 136.137 blue
					0.605 159.185 blue
					0.554 181.614 blue
					3.106 288.876 blue
					0.265 63.795 blue
					0.689 154.129 blue
					0.916 198.326 blue
					0.461 138.291 blue
					0.694 112.514 blue
					0.607 188.107 blue
					0.486 159.226 blue
					0.637 196.97699999999998 blue
					2.251 182.12099999999998 blue
					0.373 97.623 blue
					0.78 138.73 blue
					1.205 154.625 blue
					0.708 194.708 blue
					0.901 244.51100000000002 blue
					0.672 179.502 blue
					0.494 147.234 blue
					0.703 187.943 blue
					0.594 166.20399999999998 blue
					0.535 183.35500000000002 blue
					1.207 277.85699999999997 blue
					0.376 104.766 blue
					0.392 113.452 blue
					0.233 80.893 blue
					0.516 131.61599999999999 blue
					1.36 178.32 blue
					0.584 113.86399999999999 blue
					0.525 168.955 blue
					0.201 41.431 blue
					1.053 232.193 blue
					0.358 102.738 blue
					0.29 75.21000000000001 blue
					0.407 117.89699999999999 blue
					1.103 203.613 blue
					0.355 104.90500000000002 blue
					0.701 215.351 blue
					0.171 32.881 blue
					0.264 56.63400000000001 blue
					0.17 35.470000000000006 blue
					0.406 105.86600000000001 blue
					0.372 96.63199999999999 blue
					1.066 104.07600000000001 blue
					0.126 22.586000000000002 blue
					0.267 57.807 blue
					0.19 39.15 blue
					0.201 58.471 blue
					0.271 63.301 blue
					0.248 53.108 blue
					0.143 26.243 blue
					0.222 77.93199999999999 blue
					0.179 39.139 blue
					0.278 63.768 blue
					0.376 102.82600000000001 blue
					0.224 44.894 blue
					0.307 73.807 blue
					0.212 72.65200000000002 blue
					0.158 31.558000000000003 blue
					0.25 56.15 blue
					0.194 42.824000000000005 blue
					0.107 18.567 blue
					0.179 34.949000000000005 blue
					0.355 89.555 blue
					0.287 66.90700000000001 blue
					0.36 91.61 blue
					0.13 33.93 blue
					0.416 113.65599999999999 blue
					0.047 7.277 blue
					0.053 6.873 blue
					0.04 7.3100000000000005 blue
					0.026 2.3059999999999996 blue
					0.071 9.861 blue
					0.064 9.334000000000001 blue
					0.146 16.116 blue
					0.101 15.721 blue
					0.063 6.503 blue
					0.025 3.725 blue
					0.15 12.670000000000002 blue
					0.132 18.812 blue
					0.07 10.930000000000001 blue
					0.069 9.779000000000002 blue
					0.094 10.254 blue
					0.135 15.614999999999998 blue
					0.078 11.568 blue
					0.085 12.885000000000002 blue
					0.062 10.922 blue
					0.115 13.745 blue
					0.1 10.339999999999998 blue
					0.044 5.904 blue
					0.024 1.824 blue
					0.097 13.866999999999999 blue
					0.066 12.616000000000001 blue
					0.085 9.235000000000001 blue
					0.068 8.598 blue
					0.106 12.645999999999999 blue
					0.071 10.001000000000001 blue
					0.092 15.332 blue
					0.196 1.6660000000000001 blue
					0.192 1.6820000000000002 blue
					0.92 5.1899999999999995 blue
					0.238 6.468 blue
					5.848 55.958 blue
					0.175 1.4750000000000003 blue
					1.774 201.644 blue
					6.535 59.565 blue
					0.234 9.194 blue
					1.157 15.687000000000001 blue
					74.857 775.127 blue
					1.043 26.653 blue
					106.694 1353.774 blue
					0.235 2.085 blue
					0.194 4.723999999999999 blue
					0.335 5.725 blue
					0.157 1.307 blue
					1.638 212.46800000000002 blue
					0.821 7.371 blue
					1.646 211.166 blue
					1.089 9.649000000000001 blue
					1.638 211.80800000000002 blue
					1.239 98.959 blue
					11.395 108.76499999999999 blue
					4.917 46.06700000000001 blue
					1.568 123.388 blue
					0.181 1.4810000000000003 blue
					0.151 1.311 blue
					0.96 8.57 blue
					0.999 8.409 blue
					5.184 600.904 blue
					0.198 1.678 blue
					0.962 17.012 blue
					0.961 8.821 blue
					0.862 7.422000000000001 blue
					0.971 8.770999999999999 blue
					1.094 9.613999999999999 blue
					0.179 1.5090000000000001 blue
					0.201 1.681 blue
					0.261 6.641 blue
					0.21 5.63 blue
					4.497 41.867000000000004 blue
					20.617 185.03699999999998 blue
					0.852 14.142000000000001 blue
					0.174 1.484 blue
					0.061 5.001 blue
					0.113 10.523 blue
					0.173 20.993 blue
					0.18 25.07 blue
					0.041 5.001 blue
					0.039 3.9690000000000003 blue
					0.046 3.5759999999999996 blue
					0.042 4.862 blue
					0.042 4.752 blue
					0.045 4.745 blue
					0.041 4.541 blue
					0.044 3.974 blue
					0.044 4.504 blue
					0.04 3.68 blue
					0.04 3.81 blue
					0.041 4.071000000000001 blue
					0.042 4.492 blue
					0.038 3.518 blue
					0.044 3.524 blue
					0.04 4.0 blue
					0.041 3.551 blue
					0.043 5.043 blue
					0.039 4.019 blue
					0.039 3.839 blue
					0.042 4.502 blue
					0.043 4.933000000000001 blue
					0.037 3.497 blue
					0.041 4.311000000000001 blue
					0.043 4.423 blue
					0.038 3.838 blue
					0.041 3.8609999999999998 blue
					0.039 3.5090000000000003 blue
					0.041 4.291 blue
					0.041 4.4110000000000005 blue
					0.048 4.168 blue
					0.048 3.568 blue
					0.042 4.792 blue
					0.063 4.403 blue
					0.044 4.394 blue
					0.038 3.6479999999999997 blue
					0.046 3.856 blue
					0.051 4.021 blue
					0.044 3.724 blue
					0.046 3.916 blue
					0.042 4.882000000000001 blue
					0.047 3.1570000000000005 blue
					0.033 2.943 blue
					0.037 2.537 blue
					0.03 3.11 blue
					0.036 2.7560000000000002 blue
					0.044 4.784 blue
					0.037 2.957 blue
					0.038 3.368 blue
					0.04 3.6700000000000004 blue
					0.028 2.528 blue
					0.043 4.913 blue
					0.036 2.946 blue
					0.031 3.061 blue
					0.041 4.291 blue
					0.036 3.486 blue
					0.042 4.462 blue
					0.036 3.136 blue
					0.041 4.751 blue
					0.033 2.853 blue
					0.036 3.2260000000000004 blue
					0.045 4.085 blue
					0.033 3.123 blue
					0.049 3.859 blue
					0.041 3.111 blue
					0.049 4.2090000000000005 blue
					0.03 3.1999999999999997 blue
					0.045 2.835 blue
					0.047 4.127 blue
					0.035 3.145 blue
					0.039 4.0489999999999995 blue
					0.042 2.802 blue
					0.04 4.1000000000000005 blue
					0.035 2.6350000000000002 blue
					0.034 2.5839999999999996 blue
					0.04 4.07 blue
					0.038 2.608 blue
					0.043 4.283 blue
					0.033 3.133 blue
					0.033 3.203 blue
					0.048 4.098000000000001 blue
					0.028 2.938 blue
					0.046 4.816000000000001 blue
					0.029 2.999 blue
					0.032 2.522 blue
					0.041 4.111000000000001 blue
					0.037 2.577 blue
					0.042 4.502 blue
					0.028 2.8080000000000003 blue
					0.048 3.2180000000000004 blue
					0.049 4.2490000000000006 blue
					0.037 2.7270000000000003 blue
					0.056 4.196000000000001 blue
					0.033 3.443 blue
					0.042 3.282 blue
					0.037 3.757 blue
					0.037 3.037 blue
					0.038 3.478 blue
					0.028 2.498 blue
					0.044 3.974 blue
					0.032 3.382 blue
					0.042 4.242 blue
					0.029 2.6790000000000003 blue
					0.034 3.344 blue
					0.046 4.916 blue
					0.031 2.581 blue
					0.049 4.989000000000001 blue
					0.034 3.324 blue
					0.036 3.2960000000000003 blue
					0.045 5.005 blue
					0.039 3.1490000000000005 blue
					0.039 3.9390000000000005 blue
					0.045 3.015 blue
					0.031 3.1810000000000005 blue
					0.044 4.904 blue
					0.042 3.052 blue
					0.04 3.65 blue
					0.033 3.143 blue
					0.04 3.82 blue
					0.042 2.852 blue
					0.038 3.188 blue
					0.046 4.626 blue
					0.034 2.764 blue
					0.043 3.7630000000000003 blue
					0.044 2.794 blue
					0.044 4.053999999999999 blue
					0.041 3.431 blue
					0.039 2.6890000000000005 blue
					0.04 3.96 blue
					0.039 2.7390000000000003 blue
					0.044 4.124 blue
					0.032 2.8120000000000003 blue
					0.044 3.3640000000000003 blue
					0.038 3.598 blue
					0.034 3.384 blue
					0.04 3.9 blue
					0.038 2.738 blue
					0.041 4.2410000000000005 blue
					0.032 2.562 blue
					0.047 4.887 blue
					0.03 2.78 blue
					0.038 2.868 blue
					0.04 4.13 blue
					0.037 3.417 blue
					0.047 3.8770000000000002 blue
					0.03 2.77 blue
					0.041 3.071 blue
					0.043 4.583 blue
					0.036 3.0260000000000002 blue
					0.051 4.261 blue
					0.039 3.1290000000000004 blue
					0.046 4.936000000000001 blue
					0.036 2.886 blue
					0.035 2.9350000000000005 blue
					0.042 4.182 blue
					0.041 2.9210000000000003 blue
					0.035 2.7550000000000003 blue
					0.044 4.914 blue
					0.035 3.035 blue
					0.039 3.7390000000000003 blue
					0.034 2.9339999999999997 blue
					0.041 3.971 blue
					0.044 3.124 blue
					0.033 2.803 blue
					0.04 3.54 blue
					0.031 3.1510000000000002 blue
					0.042 3.702 blue
					0.042 3.452 blue
					0.04 4.11 blue
					0.038 3.128 blue
					0.037 3.617 blue
					0.042 4.432 blue
					0.042 3.582 blue
					0.042 4.032 blue
					0.04 4.2 blue
					0.038 3.358 blue
					0.031 2.7210000000000005 blue
					0.043 4.1530000000000005 blue
					0.034 3.134 blue
					0.047 4.067 blue
					0.068 1.218 blue
					0.071 1.211 blue
					0.076 1.2160000000000002 blue
					0.461 109.311 blue
					0.038 1.358 blue
					0.079 1.199 blue
					0.902 179.802 blue
					0.064 1.0939999999999999 blue
					0.879 166.61899999999997 blue
					0.061 1.081 blue
					0.077 1.237 blue
					0.022 3.242 blue
					0.072 1.1320000000000001 blue
					0.075 1.235 blue
					0.064 1.084 blue
					0.071 1.071 blue
					0.017 1.4569999999999999 blue
					0.044 7.364 blue
					0.075 48.495000000000005 blue
					0.029 1.049 blue
					0.024 1.914 blue
					0.029 2.3489999999999998 blue
					0.043 22.743 blue
					0.114 17.114 blue
					0.067 42.827000000000005 blue
					0.023 1.263 blue
					0.032 2.082 blue
					0.042 3.262 blue
					0.064 8.154 blue
					0.053 1.9729999999999999 blue
					0.051 2.001 blue
					0.055 2.015 blue
					0.055 1.9449999999999998 blue
					0.059 2.1690000000000005 blue
					0.065 2.025 blue
					0.062 2.0719999999999996 blue
					0.059 1.9889999999999999 blue
					0.061 2.131 blue
					0.055 1.9949999999999999 blue
					0.057 2.037 blue
					0.06 2.02 blue
					0.054 2.054 blue
					0.068 2.0479999999999996 blue
					0.054 1.994 blue
					0.065 2.065 blue
					0.063 1.833 blue
					0.072 1.9020000000000001 blue
					0.061 1.891 blue
					0.071 1.9109999999999998 blue
					0.063 1.813 blue
					0.064 1.944 blue
					0.063 1.793 blue
					0.071 1.901 blue
					0.061 1.821 blue
					0.063 1.843 blue
					0.076 2.026 blue
					0.062 1.8920000000000001 blue
					0.074 2.1039999999999996 blue
					0.064 1.834 blue
					0.058 1.818 blue
					0.059 1.809 blue
					0.062 1.822 blue
					0.073 1.9429999999999998 blue
					0.07 1.92 blue
					0.06 1.83 blue
					0.07 2.0 blue
					0.076 1.916 blue
					0.06 1.92 blue
					0.067 1.837 blue
					0.05 1.93 blue
					0.085 2.035 blue
					0.063 1.9229999999999998 blue
					0.068 2.028 blue
					0.067 2.027 blue
					0.072 2.042 blue
					0.128 5.168 blue
					0.164 6.223999999999999 blue
					0.203 6.853000000000001 blue
					0.13 5.18 blue
					0.137 5.367000000000001 blue
					0.16 6.01 blue
					0.18 5.97 blue
					0.176 6.296 blue
					0.148 5.658 blue
					0.149 5.849 blue
					0.129 5.229000000000001 blue
					0.168 6.1579999999999995 blue
					0.181 6.3709999999999996 blue
					0.131 5.501 blue
					0.192 6.422000000000001 blue
					0.179 5.9990000000000006 blue
					0.131 5.341 blue
					0.137 5.627000000000001 blue
					0.152 5.8420000000000005 blue
					0.145 5.685 blue
					0.183 6.393 blue
					0.199 6.689 blue
					0.196 6.296 blue
					0.146 3.306 blue
					0.168 5.638 blue
					0.16 6.12 blue
					0.17 3.2600000000000002 blue
					0.181 6.461 blue
					0.179 6.279000000000001 blue
					0.127 5.167 blue
				};
			\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
			\begin{axis}[
				scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
				ylabel=\veripb+\papilo (time),
				xlabel=\papilo (time),
				xmode=log,
				ymode=log,
				grid=both,
				grid style={line width=.1pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				minor tick num=5,
				xtick={0.01,0.1,1,10,100,1000},
				ytick={0.01,0.1,1,10,100,1000,10000},
			]
				\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x});
				\draw[domain=-100:100, smooth, variable=\x, black] plot ({\x}, {\x + 10});
				\addplot[scatter,only marks, scatter src=explicit symbolic]%
				table[meta=label] {
					x y label
					1000 1000 peer
					-0.01 -0.01 peer
					0.102 1.292 green
					3.848 169.568 green
					27.457 674.1070000000001 green
					400.096 10800 green
					0.182 12.772 green
					0.115 1.165 green
					0.123 6.923 green
					0.139 11.568999999999999 green
					958.314 10800 green
					0.842 257.702 green
					38.94 7923.0599999999995 green
					11.558 430.908 green
					0.664 1.7340000000000004 green
					0.089 45.769 green
					8.87 488.24 green
					0.234 8.744 green
					0.702 55.002 green
					5.387 322.24699999999996 green
					0.497 70.107 green
					1.274 4.614 green
					2.018 3.6979999999999995 green
					1.025 10.885 green
					0.054 1.1540000000000001 green
					311.138 8254.108 green
					0.059 17.149 green
					0.611 15.631000000000002 green
					2.16 22.41 green
					2.329 472.889 green
					88.496 9592.015999999998 green
					0.241 44.221 green
					0.09 3.05 green
					23.603 503.563 green
					0.057 1.4369999999999998 green
					0.054 7.784 green
					0.143 1.473 green
					0.029 3.6390000000000002 green
					0.028 1.158 green
					0.4 47.4 green
					0.161 27.041 green
					13.733 772.183 green
					1.51 970.91 green
					0.031 1.1309999999999998 green
					295.229 6939.409 green
					1712.776 10800 green
					0.591 14.891 green
					0.272 1.332 green
					0.218 5.228 green
					0.057 4.987 green
					0.924 98.31400000000001 green
					2.17 963.04 green
					0.116 3.086 green
					0.046 159.46599999999998 green
					56.545 5070.205000000001 green
					2.515 243.045 green
					1.339 15.419 green
					4.246 200.796 green
					0.03 2.17 green
					6.343 149.07299999999998 green
					0.707 77.47699999999999 green
					0.035 1.335 green
					0.575 3.3550000000000004 green
					0.02 1.22 green
					19.694 766.744 green
					18.963 473.033 green
					1.394 3.654 green
					1.196 6.925999999999998 green
					0.223 2.6029999999999998 green
					1.044 197.924 green
					0.358 61.428 green
					0.087 13.886999999999999 green
					14.235 1480.2849999999999 green
					67.257 1566.997 green
					0.065 2.6350000000000002 green
					0.727 430.367 blue
					0.253 492.91299999999995 blue
					55.601 10800 blue
					0.226 2.616 blue
					0.295 453.695 blue
					0.033 101.713 blue
					189.743 10800 blue
					3.288 4725.548 blue
					0.32 34.839999999999996 blue
					0.035 9.295 blue
					0.052 7.692 blue
					0.205 1740.715 blue
					2.507 791.877 blue
					0.102 1.562 blue
					0.033 2.193 blue
					0.037 1.9769999999999999 blue
					1.259 195.819 blue
					56.441 10800 blue
					0.059 1.539 blue
					2.54 242.99999999999997 blue
					0.59 3.8200000000000003 blue
					0.029 13.578999999999999 blue
					0.105 7.255 blue
					0.677 52.427 blue
					0.128 3.048 blue
					0.09 1.3 blue
					3.228 10800 blue
					0.217 2.6270000000000002 blue
					8.411 8847.791 blue
					0.079 8.099 blue
					3.481 10800 blue
					0.589 3.8190000000000004 blue
					0.02 1.27 blue
					0.133 8.793 blue
					0.065 7.805000000000001 blue
					3.227 10800 blue
					0.044 159.734 blue
					0.676 52.446 blue
					2.503 245.40300000000002 blue
					0.124 1.4140000000000001 blue
					0.68 9192.08 blue
					1.223 196.28300000000002 blue
					0.218 5.168 blue
					1.408 4.068 blue
					0.65 1.9 blue
					14.996 10800 blue
					0.333 228.193 blue
					2.122 22.812 blue
					0.098 1.558 blue
					3.489 10800 blue
					0.031 1.541 blue
					0.104 180.144 blue
					1.274 10800 blue
					0.065 5.375 blue
					0.301 34.871 blue
					0.251 1533.6209999999999 blue
					0.702 79.772 blue
					0.151 10800 blue
					7.016 10800 blue
					0.136 5.266 blue
					1.151 6.501 blue
					0.288 452.038 blue
					1.492 2726.3520000000003 blue
					0.041 1.681 blue
					0.232 493.052 blue
					0.141 10800 blue
					0.572 3.3920000000000003 blue
					183.648 10800 blue
					1.143 434.143 blue
					1.041 11.141000000000002 blue
					3.292 4722.772000000001 blue
					0.715 430.085 blue
					2.667 10800 blue
					0.054 26.013999999999996 blue
					0.255 22.395 blue
					0.023 16.692999999999998 blue
					11.067 10800 blue
					0.033 2.423 blue
					15.068 10800 blue
					0.054 101.17399999999999 blue
					0.036 1.116 blue
					0.126 1.436 blue
					0.02 1.42 blue
					0.144 1043.444 blue
					1.47 2702.0699999999997 blue
					0.032 13.122 blue
					0.152 10800 blue
					0.109 7.139 blue
					0.101 3.361 blue
					0.086 59.395999999999994 blue
					0.207 5.2170000000000005 blue
					0.011 1.081 blue
					1.126 440.496 blue
					126.984 10800 blue
					1.308 10800 blue
					0.093 59.303 blue
					3.863 10800 blue
					0.028 16.087999999999997 blue
					0.034 1.104 blue
					0.093 1.303 blue
					0.033 13.083 blue
					8.402 8849.851999999999 blue
					1.887 3.557 blue
					0.869 10800 blue
					0.104 179.394 blue
					0.018 1.208 blue
					30.348 984.6379999999999 blue
					0.625 80.085 blue
					0.82 216.19 blue
					0.046 26.285999999999998 blue
					0.105 778.695 blue
					0.034 1.974 blue
					0.132 3.0720000000000005 blue
					0.023 1.543 blue
					0.687 9191.366999999998 blue
					0.129 11.008999999999999 blue
					0.647 1.9069999999999998 blue
					0.167 1.227 blue
					0.44 1929.17 blue
					0.845 687.065 blue
					1.331 4.010999999999999 blue
					0.015 10.055 blue
					0.372 1923.112 blue
					0.171 12.721 blue
					0.017 1.4269999999999998 blue
					2.119 22.948999999999998 blue
					0.199 402.05899999999997 blue
					0.021 16.161 blue
					0.825 221.695 blue
					0.02 16.740000000000002 blue
					0.172 192.28199999999998 blue
					0.051 4.941 blue
					11.563 10800 blue
					0.011 1.081 blue
					0.863 10800 blue
					0.123 11.342999999999998 blue
					0.176 5.676 blue
					0.168 12.448 blue
					0.053 7.723 blue
					9.402 8963.222 blue
					0.197 404.667 blue
					0.181 1.241 blue
					128.175 10800 blue
					0.836 683.306 blue
					0.329 78.54899999999999 blue
					0.997 10.786999999999999 blue
					0.054 111.654 blue
					2.648 10800 blue
					0.03 1.17 blue
					0.805 146.515 blue
					6.867 10800 blue
					0.046 6.656000000000001 blue
					0.105 778.715 blue
					0.036 13.485999999999999 blue
					0.053 111.93299999999999 blue
					0.704 76.654 blue
					0.936 96.30600000000001 blue
					3.83 10800 blue
					0.013 9.853 blue
					0.123 11.523 blue
					1.912 3.5819999999999994 blue
					0.172 191.87199999999999 blue
					0.125 10800 blue
					0.571 74.381 blue
					0.271 2986.121 blue
					0.03 2.0399999999999996 blue
					9.373 3845.333 blue
					0.037 5.637 blue
					5.302 323.562 blue
				};
			\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\caption{
		Distribution of running times for \papilo and \papilo+\veripb on \pb (left) and \miplib (right) on instances with more than 1 seconds in \veripb{} and less than 30 minutes in \papilo.
		Instances hitting the time-limit are \textbf{included}.
		Each $\times$ marks an instance.
		The $y$-axis gives the time for presolving and
		the $x$-axis gives the time for verifying. Green $+$ mark optimization instances and blue $\times$ mark decision instances.
	}\label{fig:figure}
\end{figure}


\begin{table}[ht]
	\centering
	\small
	\begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}lrrr}
		\toprule
		& instances &  default & RUP & POL \\
		\midrule
		\pb-dec & 1398 & 0.050 & 0.076 & 0.078\\[-0.5ex]
		% default:  https://rubberband.zib.de/result/AYwgmpDMz5ZsptQZOoY5
		% RUP:		https://rubberband.zib.de/result/AYwu4u25z5ZsptQZOsKe
		% ADD:		https://rubberband.zib.de/result/AYwrtDe9z5ZsptQZOrta
		
		\miplib-dec&  295 & 0.500 & 0.633 & 0.792 \\[-0.5ex] 
		% default:  https://rubberband.zib.de/file/AYwgmPzez5ZsptQZOoR4
		% RUP:		https://rubberband.zib.de/result/AYwu4kbLz5ZsptQZOsFz
		% ADD:		https://rubberband.zib.de/result/AYwrsu4Lz5ZsptQZOreB
		
		\pb-opt &  532 & 0.442 & 0.807 & 0.831 \\[-0.5ex]
		% default:  https://rubberband.zib.de/result/AYwgO8Hvz5ZsptQZOn1X
		% RUP:		https://rubberband.zib.de/result/AYwu451nz5ZsptQZOsgY
		% ADD:		https://rubberband.zib.de/result/AYwrs4DMz5ZsptQZOrlC
		
		\miplib-opt&  145 & 0.414 & 1.956 & 1.984 \\[-0.5ex] 
		% supportcase11,ivu06-big
		% default:  https://rubberband.zib.de/result/AYwgmY3Nz5ZsptQZOoWj
		% RUP:		https://rubberband.zib.de/result/AYwu4gwaz5ZsptQZOsDd
		% ADD: 		https://rubberband.zib.de/result/AYwrsxvVz5ZsptQZOris
		\bottomrule
	\end{tabular*}
	\caption{Runtime comparison of default \papilo}\label{tab:table}
\end{table}


\begin{figure}[ht]
	\centering
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
		\begin{axis}[
		scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
		ylabel=Overhead per transaction,
		xlabel=Transactions,
		xmode=log,
		ymode=log,
		grid=both,
		grid style={line width=.1pt, draw=gray!10},
		major grid style={line width=.2pt,draw=gray!50},
		minor tick num=5,
		xtick={1,10,100,1000,10000, 100000, 1000000, 10000000, 100000000},
		ytick={0,0.1,0.01,0.001,0.0001, 0.00001, 0.000001, 0.0000001, 0.00000001},
		]
		\addplot[scatter,only marks, scatter src=explicit symbolic]
		table[meta=label] {
			x y label
			1375 1.8909090909090912e-05 green
			676 0.00010207100591715975 green
			642 2.0249221183800623e-05 green
			1780 2.6404494382022476e-05 green
			1869 4.922418405564473e-05 green
			5 0.0004 green
			50 4e-05 green
			648 2.623456790123457e-05 green
			4247 0.00022251000706380975 green
			4830 0.00021076604554865424 green
			4277 8.51063829787234e-05 green
			4335 0.000196078431372549 green
			4617 9.248429716265973e-05 green
			4250 0.00021364705882352943 green
			5017 0.0002587203508072553 green
			4549 0.0002169707628050121 green
			4587 8.611292783954653e-05 green
			4538 0.00020824151608638165 green
			4538 8.682238871749668e-05 green
			4412 0.00021214868540344516 green
			4603 0.00021464262437540736 green
			4733 0.00025269385167969575 green
			4576 8.631993006993007e-05 green
			4661 0.00023256811842952153 green
			4590 9.259259259259259e-05 green
			4874 0.00023163725892490767 green
			4487 0.00022576331624693562 green
			4323 8.674531575294934e-05 green
			4554 0.00021321914800175666 green
			4719 0.00023310023310023307 green
			4903 9.035284519681827e-05 green
			4459 0.00023503027584660237 green
			5149 0.0002645173820159254 green
			5537 0.00024399494310998736 green
			2423 0.00011019397441188609 green
			5058 0.0002611704230921313 green
			2485 0.00012877263581488935 green
			5133 0.00024274303526203 green
			4072 7.662082514734774e-05 green
			2233 0.00010792655620241828 green
			4231 0.00024438666981800995 green
			5467 0.00010718858606182551 green
			5184 0.00027276234567901234 green
			5628 0.00028127221037668797 green
			4816 0.00010589700996677741 green
			4816 0.00023982558139534884 green
			5 0.0002 green
			58 3.4482758620689657e-05 green
			3200 0.00010437499999999995 green
			2632 6.45896656534955e-05 green
			2804 0.00011198288159771757 green
			3142 0.00011616804583068109 green
			2872 0.000155292479108635 green
			2733 6.439809732894257e-05 green
			2989 0.0001702910672465708 green
			2941 9.826589595375728e-05 green
			2803 0.00017053157331430618 green
			2925 6.290598290598296e-05 green
			3235 0.00014621329211746524 green
			3261 0.0001551671266482674 green
			3098 6.132989025177536e-05 green
			2915 0.00010085763293310465 green
			3355 0.0001248882265275708 green
			2938 7.35194009530293e-05 green
			3216 8.364427860696515e-05 green
			3039 0.00014083580125041144 green
			4027 8.815495406009436e-05 green
			3124 0.0001456466069142125 green
			3295 0.00012321699544764786 green
			2979 4.598858677408527e-05 green
			3189 0.0001257447475697711 green
			2966 0.00014362778152393794 green
			3130 8.402555910543135e-05 green
			3289 5.38157494679234e-05 green
			3108 8.944658944658945e-05 green
			2902 0.00015851137146795312 green
			3252 0.0001300738007380074 green
			3004 0.00013315579227696407 green
			2929 9.252304540798905e-05 green
			2938 0.00012117086453369635 green
			3154 0.00011509194673430564 green
			3411 0.00010788625036646141 green
			3220 2.5465838509316723e-05 green
			3113 0.0001487311275297141 green
			2919 9.146968139773899e-05 green
			2989 9.501505520240876e-05 green
			3192 0.00011779448621553881 green
			3009 0.00010834164174144236 green
			3195 7.449139280125195e-05 green
			2942 0.00013426240652617268 green
			3069 0.00012707722385141743 green
			2646 8.654572940287221e-05 green
			2951 0.00015384615384615377 green
			3014 2.488387524883881e-05 green
			2685 0.00013035381750465543 green
			3144 0.00015489821882951654 green
			3008 9.009308510638302e-05 green
			2754 0.00011111111111111109 green
			3094 0.00013251454427925014 green
			2564 0.0002265990639625585 green
			2983 9.788803218236675e-05 green
			2866 0.0001559665038381019 green
			2911 4.843696324287187e-05 green
			906 7.72626931567329e-05 green
			760 6.973684210526315e-05 green
			708 7.768361581920903e-05 green
			837 3.4647550776583e-05 green
			890 2.6966292134831485e-05 green
			912 7.78508771929824e-05 green
			875 5.714285714285713e-05 green
			968 4.545454545454544e-05 green
			906 7.6158940397351e-05 green
			1419 5.990133897110639e-05 green
			733 4.092769440654839e-05 green
			876 6.164383561643834e-05 green
			888 5.6306306306306294e-05 green
			860 4.069767441860462e-05 green
			867 5.7670126874279144e-05 green
			638 1.0971786833855809e-05 green
			777 3.346203346203349e-05 green
			1106 3.6166365280289366e-05 green
			1540 2.532467532467531e-05 green
			847 5.4309327036599744e-05 green
			714 4.201680672268908e-05 green
			849 4.7114252061248504e-05 green
			895 7.82122905027933e-05 green
			899 7.563959955506118e-05 green
			885 5.3107344632768346e-05 green
			953 3.462749213011545e-05 green
			779 6.033376123234915e-05 green
			787 8.513341804320204e-05 green
			777 6.94980694980695e-05 green
			2258 0.00012887511071744907 green
			2284 0.0001133975481611208 green
			2330 7.93991416309013e-05 green
			2512 0.00015764331210191078 green
			2329 8.587376556462e-05 green
			2200 0.0001331818181818182 green
			2422 9.950454170107348e-05 green
			2356 9.634974533106964e-05 green
			2620 0.00011068702290076338 green
			2494 0.0001066559743384122 green
			2370 0.0001489451476793249 green
			2382 0.00012888329135180517 green
			2357 0.00013746287653797193 green
			2234 0.00016427931960608772 green
			2362 9.86452159187129e-05 green
			2108 0.0001247628083491461 green
			2477 0.00014372224465078722 green
			2603 9.373799462159047e-05 green
			2357 7.509546033092907e-05 green
			2129 0.0001169563175199624 green
			2435 5.503080082135519e-05 green
			2300 9.391304347826086e-05 green
			2723 8.48329048843188e-05 green
			2292 9.991273996509602e-05 green
			2387 9.80310012568077e-05 green
			2354 8.198810535259132e-05 green
			2273 0.00012626484821821378 green
			2826 8.669497523000711e-05 green
			2098 0.00011439466158245949 green
			1938 0.0001367389060887513 green
			2596 8.821263482280431e-05 green
			2220 0.00011351351351351349 green
			1673 8.726838015540945e-05 green
			1593 9.353421217827995e-05 green
			1543 4.666234607906679e-05 green
			1764 4.76190476190476e-05 green
			1364 9.97067448680352e-05 green
			1757 8.594194649971538e-05 green
			1777 6.359032076533483e-05 green
			1902 8.885383806519455e-05 green
			1838 0.00010010881392818281 green
			1519 7.636603028308097e-05 green
			1562 0.00014404609475032008 green
			1789 5.86920067076579e-05 green
			1604 8.354114713216959e-05 green
			1842 0.00010749185667752447 green
			1443 6.999306999307006e-05 green
			1501 0.00013524317121918724 green
			1588 0.0001120906801007557 green
			1628 4.299754299754236e-06 green
			1626 0.00015805658056580567 green
			1495 6.88963210702341e-05 green
			1441 0.0001068702290076336 green
			1697 0.00010253388332351217 green
			1544 0.00012370466321243528 green
			9 0.0 green
			297 0.000367003367003367 green
			16196 0.00046153371202766114 green
			9880 -3.0364372469635653e-07 green
			1344 0.0013058035714285713 green
			184 0.00016304347826086955 green
			11177 6.889147356177865e-06 green
			38 0.0025 green
			4064 0.0005108267716535433 green
			4192 2.7671755725190865e-05 green
			35 8.57142857142858e-05 green
			2334 8.140531276778064e-06 green
			10645 4.8003757632691394e-05 green
			1799 3.8910505836575854e-06 green
			9 -0.00044444444444444447 green
			39 5.128205128205133e-05 green
			5370 8.007448789571701e-06 green
			36 0.00011111111111111112 green
			274 -4.7445255474452544e-05 green
			4 -0.0005 green
			135472 0.04915037793787646 green
			60 1.666666666666668e-05 green
			2076 6.26204238921002e-06 green
			1693 0.0012575310100413468 green
			7453 0.0029765195223399976 green
			9505 2.0515518148342977e-05 green
			333 0.0006156156156156158 green
			3528 0.003586451247165533 green
			144 2.777777777777778e-05 green
			13 0.0003076923076923077 green
			33 0.00012121212121212121 green
			90 7.777777777777778e-05 green
			48 6.25e-05 green
			68 1.4705882352941177e-05 green
			17 0.00011764705882352942 green
			29 0.00010344827586206896 green
			40 0.000125 green
			44 0.00013636363636363634 green
			14 0.0006428571428571429 green
			74 4.054054054054054e-05 green
			64 6.25e-05 green
			22 0.00013636363636363637 green
			41 0.00014634146341463414 green
			74 2.7027027027027027e-05 green
			20 0.0001 green
			37 0.00013513513513513514 green
			53 0.00011320754716981132 green
			28 -0.0008571428571428572 green
			15 0.00013333333333333334 green
			13 0.00015384615384615385 green
			82 3.6585365853658535e-05 green
			17 0.0008235294117647059 green
			21 9.523809523809524e-05 green
			69 8.695652173913044e-05 green
			92 2.173913043478261e-05 green
			58 3.4482758620689657e-05 green
			22 0.00036363636363636367 green
			48 8.333333333333333e-05 green
			13 0.0003076923076923077 green
			84 3.571428571428572e-05 green
			89 4.4943820224719104e-05 green
			46 8.695652173913044e-05 green
			22 0.00013636363636363637 green
			51 7.843137254901961e-05 green
			16 0.0001875 green
			126 3.1746031746031745e-05 green
			79 6.329113924050633e-05 green
			19 0.0 green
			86 2.3255813953488374e-05 green
			15 0.0002 green
			28 7.142857142857143e-05 green
			37 8.108108108108108e-05 green
			66 4.545454545454546e-05 green
			69 5.797101449275363e-05 green
			14 0.00014285714285714287 green
			28 7.142857142857143e-05 green
			23 8.695652173913044e-05 green
			39 0.0005897435897435898 green
			35 8.571428571428571e-05 green
			68 0.00016176470588235293 green
			127 3.937007874015748e-05 green
			20 0.0001 green
			43 9.30232558139535e-05 green
			25 0.00024 green
			31 3.2258064516129034e-05 green
			13 0.00015384615384615385 green
			28 0.00010714285714285715 green
			87 0.00047126436781609187 green
			1723 5.803830528148579e-06 green
			1779 2.2484541877459227e-06 green
			1779 -7.307476110174257e-06 green
			1779 3.934794828555368e-06 green
			1723 -5.803830528148579e-06 green
			1723 7.54497968659315e-06 green
			1723 1.10272780034823e-05 green
			1779 2.8105677346824044e-06 green
			1779 1.6863406408094451e-06 green
			1779 6.745362563237772e-06 green
			1779 1.3490725126475549e-05 green
			1779 2.2484541877459227e-06 green
			1779 5.621135469364813e-06 green
			1779 3.934794828555368e-06 green
			1779 5.621135469364813e-06 green
			1723 1.1607661056297154e-05 green
			1779 -6.183249016301294e-06 green
			240 4.166666666666667e-06 green
			4048 2.223320158102767e-06 green
			728 -1.3736263736263749e-06 green
			6545 1.8334606569900694e-06 green
			240 4.166666666666667e-06 green
			4060 1.9704433497536957e-06 green
			728 -4.12087912087912e-06 green
			4060 -2.463054187192117e-06 green
			728 -6.86813186813187e-06 green
			22 4.545454545454546e-05 green
			3080 -1.2987012987012988e-06 green
			240 8.333333333333334e-06 green
			3080 -6.493506493506499e-07 green
			1140 2.6315789473684232e-06 green
			2300 -2.6086956521739137e-06 green
			2280 0.0 green
			4048 1.7292490118577078e-06 green
			240 2.5000000000000008e-05 green
			2280 7.894736842105263e-06 green
			728 -8.241758241758244e-06 green
			240 4.166666666666667e-06 green
			5456 1.649560117302053e-06 green
			728 -2.747252747252748e-05 green
			240 8.33333333333333e-06 green
			240 0.0 green
			728 1.3736263736263736e-06 green
			842 8.313539192399049e-06 green
			666 -1.9519519519519517e-05 green
			746 4.021447721179619e-06 green
			841 9.512485136741975e-06 green
			723 1.7980636237897654e-05 green
			630 -2.063492063492063e-05 green
			175 3.428571428571428e-05 green
			560 1.7857142857142874e-06 green
			410 2.4390243902439044e-06 green
			99 0.00011111111111111112 green
			173 -7.514450867052021e-05 green
			326 6.13496932515338e-06 green
			375 7.999999999999998e-06 green
			279 -3.584229390681007e-06 green
			450 6.666666666666665e-06 green
			430 0.0 green
			321 3.115264797507791e-06 green
			432 2.314814814814809e-06 green
			760 9.210526315789472e-06 green
			2168 4.612546125461258e-06 green
			1974 -4.0526849037487375e-06 green
			1339 8.215085884988805e-06 green
			12377 9.889310818453584e-05 green
			29325 7.28388746803069e-05 green
			14946 3.4390472367188544e-05 green
			32745 6.309360207665292e-05 green
			28507 7.577086329673412e-05 green
			35139 6.4316002162839e-05 green
			32255 7.353898620368935e-05 green
			14217 8.194415136808046e-05 green
			35570 6.353668822041045e-05 green
			34238 6.250365091418892e-05 green
			36990 6.353068396864017e-05 green
			30984 7.277949909630777e-05 green
			14596 7.844614963003563e-05 green
			36223 6.087292604146537e-05 green
			31951 7.082720415636443e-05 green
			30672 3.586332811684924e-05 green
			33982 3.3076334530045314e-05 green
			16603 7.227609468168403e-05 green
			24385 7.619438179208529e-05 green
			30848 7.984310165975104e-05 green
			608 0.04682565789473684 green
			608 0.018675986842105263 green
			17017 1.1929247223364871e-05 green
			606 0.05957590759075908 green
			17127 1.1151982250248146e-05 green
			608 0.047302631578947374 green
			7485 1.6032064128256513e-05 green
			7491 1.7888132425577356e-05 green
			4251 1.9995295224653014e-05 green
			1084 6.273062730627307e-05 green
			7486 1.0152284263959385e-05 green
			608 0.05791447368421053 green
			608 0.01960690789473684 green
			7485 1.2692050768203069e-05 green
			607 0.05881878088962109 green
			7486 1.816724552497996e-05 green
			7381 1.1651537732014631e-05 green
			17133 1.3949687737115507e-05 green
			17126 1.4305733971738877e-05 green
			493 0.07103245436105478 green
			609 0.02362725779967159 green
			4251 7.998118089861203e-06 green
			1084 5.719557195571956e-05 green
			1084 6.273062730627307e-05 green
			609 0.07043185550082103 green
			587 0.06106473594548552 green
			609 0.07224630541871921 green
			500 0.0224 green
			608 0.04711019736842106 green
			17101 1.005789135138296e-05 green
			173517 1.4932254476506631e-05 green
			71284 1.3102519499466935e-05 green
			71281 1.9416113690885348e-05 green
			173489 1.0358005406682848e-05 green
			37291 9.787884476147065e-06 green
			71287 5.050009118071961e-07 green
			173506 1.345774785886367e-05 green
			37267 1.9346875251563037e-05 green
			173494 9.187637612828117e-06 green
			71296 9.734066427289036e-06 green
			37290 5.819254491820878e-06 green
			70392 7.287759972724172e-06 green
			173487 1.1580118395038242e-05 green
			37291 1.7859537153736838e-05 green
			71297 1.3324543809697304e-06 green
			3287 2.7076361423790815e-05 green
			173487 1.4058690276504869e-05 green
			173511 -1.043161528663884e-06 green
			37284 1.5797661195150746e-05 green
			37284 2.084003862246538e-05 green
			173488 1.4450567186203078e-05 green
			173530 1.2683685818014179e-05 green
			173512 1.2627368712250444e-05 green
			37284 8.099989271537426e-06 green
			37291 2.1318816872703867e-05 green
			173484 1.2750455373406187e-05 green
			71292 6.522470964484092e-06 green
			37284 2.9369166398455117e-05 green
			71281 1.2724288379792651e-05 green
			37290 1.4802896218825459e-05 green
			1285 0.00011517509727626458 blue
			1209 0.00011331679073614559 blue
			1079 0.00013901760889712696 blue
			1125 0.0001377777777777778 blue
			2765 7.703435804701628e-05 blue
			972 0.00015329218106995885 blue
			1476 9.485094850948508e-05 blue
			1627 6.45359557467732e-05 blue
			1407 0.00010163468372423596 blue
			1139 0.0001404741000877963 blue
			1195 0.00012803347280334728 blue
			1470 0.00012789115646258503 blue
			1703 7.046388725778038e-05 blue
			1535 0.00011530944625407165 blue
			1224 0.00014542483660130717 blue
			1365 0.00011501831501831502 blue
			1525 8.983606557377049e-05 blue
			1559 7.440667094291214e-05 blue
			1475 9.559322033898304e-05 blue
			1611 8.379888268156425e-05 blue
			2502 9.192645883293364e-05 blue
			2869 9.236667828511677e-05 blue
			2922 0.00013791923340177958 blue
			7131 5.7074744075164767e-05 blue
			2434 0.0001750205423171734 blue
			6136 9.859843546284224e-05 blue
			4881 7.969678344601515e-05 blue
			3603 0.0001279489314460172 blue
			2918 0.00012200137080191913 blue
			3250 8.738461538461538e-05 blue
			3026 0.00014474553866490416 blue
			2513 0.00015957023477914843 blue
			3213 0.00014285714285714287 blue
			3189 0.00012198181248040131 blue
			3062 9.079033311561071e-05 blue
			3645 9.629629629629631e-05 blue
			4252 9.031044214487302e-05 blue
			3127 0.00014230892228973455 blue
			3235 0.000162596599690881 blue
			3786 0.0001064447966191231 blue
			2699 0.00013931085587254538 blue
			3543 0.00012616426756985604 blue
			3174 0.000130119722747322 blue
			3176 0.00013790931989924435 blue
			3109 0.00016693470569314897 blue
			2527 0.00011713494261970716 blue
			3068 5.182529335071709e-05 blue
			3359 9.615957130098243e-05 blue
			3052 0.00012680209698558327 blue
			2768 6.936416184971097e-05 blue
			3051 0.00013765978367748282 blue
			3073 0.00016140579238529122 blue
			2709 7.27205610926541e-05 blue
			3072 0.00010351562499999998 blue
			3833 7.304983042003653e-05 blue
			2934 0.0001462167689161554 blue
			1892 0.00010465116279069768 blue
			1723 0.00019558908879860709 blue
			2925 0.0001052991452991453 blue
			3111 6.460945033751208e-05 blue
			2376 8.24915824915825e-05 blue
			2228 5.565529622980252e-05 blue
			2404 6.364392678868552e-05 blue
			1966 0.00010783316378433368 blue
			1750 0.00018 blue
			1715 8.221574344023324e-05 blue
			1633 0.0001200244947948561 blue
			3068 3.455019556714472e-05 blue
			1799 0.0001595330739299611 blue
			1827 0.0001264367816091954 blue
			1851 0.00015721231766612642 blue
			1803 0.0001858014420410427 blue
			783 2.937420178799489e-05 blue
			1074 2.7001862197392923e-05 blue
			832 5.1682692307692305e-05 blue
			1602 5.056179775280898e-05 blue
			1171 6.917164816396242e-05 blue
			854 3.3957845433255264e-05 blue
			1931 3.210771620921802e-05 blue
			2833 3.494528768090364e-05 blue
			471 0.00010828025477707007 blue
			862 5.3364269141531327e-05 blue
			1050 5.5238095238095244e-05 blue
			1683 4.693998811645871e-05 blue
			604 9.437086092715232e-05 blue
			900 7.555555555555556e-05 blue
			602 6.478405315614617e-05 blue
			1275 4.8627450980392164e-05 blue
			1045 6.220095693779904e-05 blue
			895 8.8268156424581e-05 blue
			1027 4.2843232716650444e-05 blue
			737 6.377204884667571e-05 blue
			1069 6.0804490177736206e-05 blue
			702 7.264957264957263e-05 blue
			632 0.0001170886075949367 blue
			730 2.1917808219178083e-05 blue
			69 0.0002463768115942029 blue
			45 -0.00035555555555555557 blue
			118 -8.47457627118639e-06 blue
			101 0.00037623762376237603 blue
			154 0.007733766233766234 blue
			39 0.0010256410256410259 blue
			2 0.038000000000000034 blue
			27799 3.2087485161336594e-05 blue
			104 0.001144230769230768 blue
			50150 5.056829511465606e-05 blue
			12 0.0017500000000000016 blue
			12 0.012666666666666668 blue
			264 0.004545454545454545 blue
			366 0.003355191256830601 blue
			416 0.0029807692307692304 blue
			8970 5.763656633221852e-05 blue
			10137 7.309854986682451e-05 blue
			1221 0.0028501228501228507 blue
			101 0.0007326732673267322 blue
			6 0.0043333333333333375 blue
			38 0.0011842105263157891 blue
			185 0.00023243243243243204 blue
			140 7.142857142857143e-06 blue
			38 2.6315789473684212e-05 blue
			116 8.620689655172414e-06 blue
			40 5e-05 blue
			138 1.4492753623188407e-05 blue
			48 4.1666666666666665e-05 blue
			52 3.846153846153846e-05 blue
			124 1.6129032258064517e-05 blue
			180 5.555555555555556e-06 blue
			52 3.846153846153846e-05 blue
			166 1.2048192771084337e-05 blue
			196 5.102040816326531e-06 blue
			42 4.761904761904762e-05 blue
			46 4.347826086956522e-05 blue
			174 1.1494252873563218e-05 blue
			58 3.4482758620689657e-05 blue
			52 3.846153846153846e-05 blue
			168 1.1904761904761905e-05 blue
			58 3.4482758620689657e-05 blue
			162 6.17283950617284e-06 blue
			128 1.5625e-05 blue
			36 5.555555555555556e-05 blue
			172 5.8139534883720935e-06 blue
			50 0.0001 blue
			110 0.00011818181818181818 blue
			48 4.1666666666666665e-05 blue
			34 5.882352941176471e-05 blue
			46 0.0 blue
			102 1.9607843137254903e-05 blue
			142 1.4084507042253522e-05 blue
			54 1.8518518518518518e-05 blue
			54 3.7037037037037037e-05 blue
			200 0.0 blue
			52 3.846153846153846e-05 blue
			56 5.3571428571428575e-05 blue
			176 1.1363636363636365e-05 blue
			32 3.125e-05 blue
			146 5.479452054794521e-05 blue
			52 3.846153846153846e-05 blue
			144 1.388888888888889e-05 blue
			42 4.761904761904762e-05 blue
			44 4.545454545454546e-05 blue
			152 1.3157894736842106e-05 blue
			48 2.0833333333333333e-05 blue
			154 1.2987012987012988e-05 blue
			48 4.1666666666666665e-05 blue
			52 -1.923076923076923e-05 blue
			134 0.00015671641791044775 blue
			42 4.761904761904762e-05 blue
			182 5.494505494505494e-06 blue
			46 4.347826086956522e-05 blue
			120 8.333333333333334e-06 blue
			170 1.7647058823529414e-05 blue
			44 4.545454545454546e-05 blue
			126 7.936507936507936e-06 blue
			62 1.6129032258064517e-05 blue
			1 0.003 blue
			46 6.521739130434783e-05 blue
			58 1.7241379310344828e-05 blue
			156 2.5641025641025643e-05 blue
			46 4.347826086956522e-05 blue
			38 5.2631578947368424e-05 blue
			44 4.545454545454546e-05 blue
			50 2e-05 blue
			178 1.1235955056179776e-05 blue
			50 2e-05 blue
			54 3.7037037037037037e-05 blue
			54 3.7037037037037037e-05 blue
			136 2.9411764705882354e-05 blue
			44 0.0 blue
			160 1.25e-05 blue
			190 5.263157894736842e-06 blue
			60 3.3333333333333335e-05 blue
			122 8.19672131147541e-06 blue
			46 4.347826086956522e-05 blue
			48 0.00016666666666666666 blue
			130 1.5384615384615384e-05 blue
			50 4e-05 blue
			54 1.8518518518518518e-05 blue
			54 3.7037037037037037e-05 blue
			184 5.4347826086956525e-06 blue
			56 3.571428571428572e-05 blue
			50 2e-05 blue
			50 4e-05 blue
			186 0.0 blue
			132 3.787878787878788e-05 blue
			150 6.666666666666667e-06 blue
			56 -1.785714285714286e-05 blue
			188 1.0638297872340426e-05 blue
			52 1.923076923076923e-05 blue
			194 -5.154639175257732e-06 blue
			44 4.545454545454546e-05 blue
			760 -1.1842105263157905e-05 blue
			1339 3.734129947722184e-06 blue
			1974 9.118541033434645e-06 blue
			2167 5.9990770650669054e-06 blue
			1058 2.2684310018903593e-05 blue
			1043 2.109300095877277e-05 blue
			1163 2.4935511607910575e-05 blue
			1003 2.691924227318046e-05 blue
			1037 2.217936354869817e-05 blue
			1042 2.5911708253358925e-05 blue
			1034 2.4177949709864606e-05 blue
			1019 2.3552502453385668e-05 blue
			1045 1.0526315789473681e-05 blue
			1040 2.0192307692307694e-05 blue
			1129 1.9486271036315325e-05 blue
			1007 2.3833167825223435e-05 blue
			1005 2.5870646766169156e-05 blue
			994 1.7102615694164987e-05 blue
			1018 2.3575638506876224e-05 blue
			1032 1.937984496124031e-05 blue
			1035 2.028985507246377e-05 blue
			1039 2.3099133782483156e-05 blue
			1026 1.4619883040935671e-05 blue
			1115 1.3452914798206278e-05 blue
			1043 2.301054650047939e-05 blue
			994 2.816901408450704e-05 blue
			1013 1.7769002961500493e-05 blue
			1000 2.5e-05 blue
			1032 2.5193798449612397e-05 blue
			1007 1.8867924528301888e-05 blue
			1046 2.2944550669216063e-05 blue
			1013 1.4807502467917077e-05 blue
			1059 1.98300283286119e-05 blue
			1055 1.990521327014218e-05 blue
			1051 2.7592768791627025e-05 blue
			1098 2.9143897996357015e-05 blue
			1058 1.7013232514177696e-05 blue
			1038 4.1425818882466275e-05 blue
			1037 2.6036644165863062e-05 blue
			1008 2.0833333333333333e-05 blue
			1118 2.59391771019678e-05 blue
			1013 3.3563672260612036e-05 blue
			1033 2.323330106485963e-05 blue
			1045 2.8708133971291865e-05 blue
			996 2.6104417670682734e-05 blue
			991 3.1281533804238145e-05 blue
			1035 1.352657004830918e-05 blue
			1023 8.797653958944279e-06 blue
			1050 1.238095238095238e-05 blue
			1163 1.7196904557179705e-05 blue
			981 2.7522935779816508e-05 blue
			1043 1.629913710450623e-05 blue
			1057 1.986754966887417e-05 blue
			1045 1.8181818181818182e-05 blue
			1084 1.107011070110701e-05 blue
			990 2.2222222222222217e-05 blue
			1033 1.6456921587608903e-05 blue
			1064 1.3157894736842104e-05 blue
			1020 2.254901960784314e-05 blue
			1060 1.6981132075471696e-05 blue
			1021 2.546523016650343e-05 blue
			1005 1.8905472636815918e-05 blue
			1032 2.4224806201550387e-05 blue
			1068 9.363295880149815e-06 blue
			1035 1.9323671497584538e-05 blue
			1054 2.4667931688804553e-05 blue
			1035 1.4492753623188408e-05 blue
			1046 2.772466539196941e-05 blue
			1057 2.0813623462630086e-05 blue
			999 3.203203203203203e-05 blue
			1062 1.2241054613935968e-05 blue
			1022 2.73972602739726e-05 blue
			1058 3.0245746691871456e-05 blue
			1045 1.3397129186602873e-05 blue
			999 2.202202202202202e-05 blue
			1090 2.4770642201834864e-05 blue
			1013 1.579466929911155e-05 blue
			1113 1.7070979335130282e-05 blue
			1032 1.0658914728682174e-05 blue
			1054 1.707779886148008e-05 blue
			1160 1.8103448275862068e-05 blue
			1031 2.4248302618816682e-05 blue
			1033 1.2584704743465635e-05 blue
			1010 1.7821782178217823e-05 blue
			1108 2.9783393501805057e-05 blue
			1079 9.2678405931418e-06 blue
			995 2.814070351758794e-05 blue
			1030 9.708737864077671e-06 blue
			1061 1.413760603204524e-05 blue
			1065 2.347417840375587e-05 blue
			1094 1.736745886654479e-05 blue
			1035 2.2222222222222227e-05 blue
			1010 9.900990099009903e-06 blue
			1025 3.1219512195121955e-05 blue
			1019 2.4533856722276743e-05 blue
			1134 1.8518518518518518e-05 blue
			1011 3.956478733926805e-05 blue
			1059 1.5108593012275732e-05 blue
			1020 2.450980392156863e-05 blue
			1029 1.3605442176870747e-05 blue
			1053 1.614434947768281e-05 blue
			1000 1.1e-05 blue
			1073 1.1183597390493943e-05 blue
			1014 2.3668639053254434e-05 blue
			1072 1.2126865671641792e-05 blue
			1045 2.105263157894737e-05 blue
			1021 1.1753183153770813e-05 blue
			1051 7.611798287345389e-06 blue
			1050 2.4761904761904762e-05 blue
			1032 9.689922480620154e-06 blue
			1063 2.634054562558796e-05 blue
			1032 1.4534883720930235e-05 blue
			1039 1.63618864292589e-05 blue
			1053 1.994301994301994e-05 blue
			1088 2.113970588235294e-05 blue
			1014 1.9723865877712034e-05 blue
			1027 2.629016553067186e-05 blue
			1027 1.1684518013631937e-05 blue
			1013 1.875616979269496e-05 blue
			1032 2.4224806201550387e-05 blue
			1135 2.026431718061674e-05 blue
			1025 1.1707317073170731e-05 blue
			1111 2.1602160216021603e-05 blue
			1173 2.216538789428815e-05 blue
			1084 1.9372693726937268e-05 blue
			1055 2.748815165876777e-05 blue
			1010 1.6831683168316834e-05 blue
			1077 1.9498607242339832e-05 blue
			1050 2.2857142857142855e-05 blue
			1036 2.6061776061776057e-05 blue
			1062 2.1657250470809796e-05 blue
			1119 1.966041108132261e-05 blue
			1153 1.99479618386817e-05 blue
			1049 2.1925643469971403e-05 blue
			1031 2.521823472356935e-05 blue
			991 1.311806256306761e-05 blue
			1029 2.235179786200194e-05 blue
			1022 1.5655577299412916e-05 blue
			975 1.8461538461538465e-05 blue
			1064 1.8796992481203007e-05 blue
			1109 1.623083859332732e-05 blue
			1042 2.2072936660268717e-05 blue
			1034 1.2572533849129595e-05 blue
			1046 2.2944550669216063e-05 blue
			1061 1.1310084825636192e-05 blue
			1122 1.871657754010695e-05 blue
			1028 1.945525291828794e-05 blue
			1050 1.8095238095238094e-05 blue
			1027 2.823758519961052e-05 blue
			1062 1.0357815442561205e-05 blue
			1026 1.5594541910331384e-05 blue
			1054 2.466793168880455e-05 blue
			1075 1.6744186046511626e-05 blue
			1042 3.071017274472169e-05 blue
			1035 1.932367149758454e-05 blue
			993 2.9204431017119836e-05 blue
			1035 2.0289855072463767e-05 blue
			1029 1.8464528668610304e-05 blue
			1028 2.2373540856031132e-05 blue
			1011 2.176063303659743e-05 blue
			1099 1.0009099181073705e-05 blue
			1023 2.4437927663734112e-05 blue
			1053 1.804368471035138e-05 blue
			1017 1.9665683382497542e-05 blue
			1003 9.970089730807578e-06 blue
			1096 2.18978102189781e-05 blue
			1044 1.915708812260536e-05 blue
			1037 1.1571841851494697e-05 blue
			1011 1.8793273986152323e-05 blue
			1059 1.0387157695939564e-05 blue
			1038 2.1194605009633915e-05 blue
			1056 1.609848484848485e-05 blue
			1044 2.2988505747126437e-05 blue
			1035 1.932367149758454e-05 blue
			1044 2.1072796934865898e-05 blue
			1053 2.184235517568851e-05 blue
			1071 2.2408963585434178e-05 blue
			1039 2.4061597690086624e-05 blue
			1021 2.448579823702253e-05 blue
			990 2.222222222222222e-05 blue
			1010 9.9009900990099e-06 blue
			1006 1.8886679920477134e-05 blue
			1041 1.633045148895293e-05 blue
			1034 2.9013539651837524e-05 blue
			1 0.028999999999999998 blue
			1 0.009 blue
			1 0.005999999999999998 blue
			1 0.014 blue
			1 0.011000000000000001 blue
			1 0.0040000000000000036 blue
			1 0.004 blue
			1 0.012 blue
			1 0.016 blue
			1 0.002 blue
			1 0.006999999999999992 blue
			1 0.021000000000000005 blue
			1 0.0 blue
			1 0.031 blue
			1 0.009999999999999995 blue
			1 0.020999999999999998 blue
			1 0.002999999999999999 blue
			1 0.009000000000000001 blue
			1 0.006 blue
			1 0.0040000000000000036 blue
			1 0.004 blue
			1 0.0 blue
			1 0.005999999999999998 blue
			1 0.013999999999999999 blue
			1 0.005999999999999999 blue
			1 -0.0030000000000000027 blue
			1 0.0050000000000000044 blue
			1 0.004 blue
			1 -0.004 blue
			28 0.0008928571428571429 blue
			1 0.008 blue
			1 0.008 blue
			1 0.007000000000000006 blue
			1 0.018000000000000002 blue
			1 -0.016999999999999998 blue
			1 0.015000000000000001 blue
			1 0.0050000000000000044 blue
			1 0.002 blue
			1 0.0009999999999999992 blue
			1 0.0020000000000000018 blue
			1 0.004 blue
			1 0.0009999999999999992 blue
			1 0.0010000000000000009 blue
			1 0.005999999999999998 blue
			1 0.0009999999999999992 blue
			1 0.008 blue
			1 0.009000000000000001 blue
			1 0.009000000000000001 blue
			1 0.007999999999999998 blue
			190 0.004131578947368421 blue
			1 0.0049999999999999975 blue
			1 0.006999999999999999 blue
			1 0.004999999999999999 blue
			1 0.0030000000000000027 blue
			1 0.013 blue
			1 0.009000000000000001 blue
			1 0.012999999999999998 blue
			1 0.004999999999999999 blue
			1 0.006999999999999992 blue
			1 0.0030000000000000027 blue
			1 0.0049999999999999906 blue
			1 0.0009999999999999992 blue
			31 0.00019354838709677424 blue
			1 0.011000000000000003 blue
			1 0.020000000000000004 blue
			1 0.012000000000000004 blue
			17 0.00017647058823529413 blue
			1 0.003999999999999998 blue
			1 0.001 blue
			1 0.0 blue
			1 0.002 blue
			1 0.001 blue
			1 0.004 blue
			1 0.0009999999999999992 blue
			1 0.001999999999999999 blue
			1 0.009000000000000001 blue
			1 0.002 blue
			1 0.0019999999999999983 blue
			1 0.003000000000000001 blue
			41 0.00012195121951219512 blue
			13 0.00023076923076923076 blue
			1 0.004 blue
			1 0.002 blue
			40 0.00015000000000000001 blue
			19 0.0002631578947368421 blue
			1 0.003999999999999999 blue
			1 0.001999999999999999 blue
			1 0.002 blue
			1 0.019 blue
			1 0.005999999999999998 blue
			1 0.022000000000000002 blue
			1 0.0010000000000000009 blue
			1 0.029 blue
			26 0.00015384615384615385 blue
			1 0.0009999999999999974 blue
			20 0.00015000000000000001 blue
			1 0.01 blue
			1 0.018000000000000002 blue
			39 0.0001282051282051282 blue
			1 0.004 blue
			1 0.0010000000000000009 blue
			1 0.002 blue
			1 0.0 blue
			1 0.004 blue
			1 0.002 blue
			1 0.007000000000000001 blue
			1 0.006999999999999999 blue
			1 0.0019999999999999983 blue
			1 0.003 blue
			19 0.00010526315789473685 blue
			1 0.01 blue
			1 0.003 blue
			1 0.004999999999999999 blue
			1 0.001 blue
			1 0.019 blue
			1 0.002 blue
			1 0.002 blue
			1 0.006 blue
			1 0.009999999999999998 blue
			1 0.002 blue
			1 0.001 blue
			1 0.003000000000000001 blue
			1 0.003 blue
			1 0.003000000000000001 blue
			1 0.005 blue
			1 -0.011 blue
			1 0.002 blue
			1 -0.008999999999999998 blue
			1 0.002 blue
			1 0.0010000000000000009 blue
			1 0.001 blue
			1 0.004 blue
			39 7.692307692307693e-05 blue
			1 0.004 blue
			1 -0.02 blue
			1 0.002 blue
			1 0.0010000000000000009 blue
			1 0.005999999999999998 blue
			1 0.002 blue
			1 0.004 blue
			1 0.001 blue
			1 0.002 blue
			16 0.0005 blue
			16 0.0003125 blue
			1 0.004 blue
			1 0.009000000000000001 blue
			11 0.00027272727272727274 blue
			1 0.001999999999999999 blue
			1 -0.007 blue
			1 0.0 blue
			47 4.2553191489361704e-05 blue
			1 0.006000000000000002 blue
			33 6.0606060606060605e-05 blue
			1 0.001 blue
			1 0.0010000000000000009 blue
			1 0.002 blue
			22 9.090909090909092e-05 blue
			1 0.002 blue
			1 0.015000000000000001 blue
			30 0.0001 blue
			1 0.0009999999999999992 blue
			1 0.002 blue
			1 0.006 blue
			1 0.002 blue
			1 -0.01 blue
			1 0.004999999999999999 blue
			1 0.002 blue
			1 0.002 blue
			1 0.001 blue
			1 -0.006 blue
			1 0.002 blue
			1 0.0 blue
			1 0.002999999999999999 blue
			38 0.0002631578947368421 blue
			1 0.03 blue
			22 9.090909090909092e-05 blue
			1 0.002 blue
			18 0.0 blue
			1 0.001 blue
			1 0.002 blue
			1 0.001 blue
			1 0.001 blue
			1 0.005000000000000001 blue
			1 0.004999999999999999 blue
			1 0.001 blue
			1 0.001 blue
			1 0.001 blue
			1 0.019 blue
			1 0.0010000000000000009 blue
			1 0.001 blue
			1 0.0010000000000000009 blue
			1 0.008 blue
			1 0.002 blue
			1 0.020000000000000004 blue
			1 0.0010000000000000009 blue
			1 0.001 blue
			1 0.004000000000000002 blue
			1 0.005000000000000001 blue
			1 0.0 blue
			1 0.002 blue
			1 0.012 blue
			1 0.002 blue
			1 0.027000000000000003 blue
			1 0.002 blue
			1 0.026 blue
			1 0.002 blue
			1 0.015 blue
			1 0.001 blue
			1 -0.001 blue
			1 -0.006000000000000002 blue
			1 0.003 blue
			1 0.002 blue
			13 0.0003076923076923077 blue
			9 0.00022222222222222223 blue
			7 0.00028571428571428574 blue
			18 5.555555555555556e-05 blue
			1 0.004 blue
			1 0.017 blue
			1 0.017 blue
			1 0.004 blue
			1 0.0009999999999999992 blue
			1 0.003999999999999999 blue
			1 0.002 blue
			1 0.002 blue
			1 0.0010000000000000009 blue
			1 0.008 blue
			16 0.0003125 blue
			1 0.002 blue
			33 0.0001515151515151515 blue
			1 0.019 blue
			1 0.002 blue
			1 0.006 blue
			1 0.018 blue
			1 0.019000000000000003 blue
			1 0.001 blue
			1 0.002999999999999999 blue
			1 0.024 blue
			1 0.001 blue
			1 0.019 blue
			26 0.0018076923076923077 blue
			33 0.0 blue
			1 0.024 blue
			1 0.004 blue
			1 0.0 blue
			1 0.002 blue
			1 0.001 blue
			1 0.001 blue
			1 0.001 blue
			1 0.003 blue
			1 0.002 blue
			1 0.001 blue
			1 0.001 blue
			1 0.002 blue
			1 0.002 blue
			1 0.002 blue
			1 0.0 blue
			1 0.001 blue
			1 0.001 blue
			1 0.001 blue
			1 0.003 blue
			1 0.001 blue
			1 -0.004 blue
			1 0.013 blue
			1 0.002 blue
			1 0.011 blue
			1 0.001 blue
			1 0.001 blue
			1 0.001 blue
			11 0.00027272727272727274 blue
			1 0.001 blue
			21 0.0002380952380952381 blue
			34 0.0 blue
			131 3.816793893129769e-05 blue
			116 8.620689655172414e-06 blue
			129 0.0 blue
			120 3.3333333333333335e-05 blue
			232 2.586206896551724e-05 blue
			70 7.142857142857145e-05 blue
			17 0.00011764705882352942 blue
			69 0.00011594202898550725 blue
			22 9.090909090909092e-05 blue
			452 8.849557522123894e-06 blue
			127 3.937007874015746e-05 blue
			21 4.761904761904762e-05 blue
			900 5.222222222222222e-05 blue
			133 4.511278195488726e-05 blue
			18 0.0002777777777777778 blue
			38 0.0 blue
			66 -6.0606060606060605e-05 blue
			33 9.090909090909098e-05 blue
			228 0.00011403508771929826 blue
			65 0.00018461538461538463 blue
			456 2.4122807017543866e-05 blue
			37 5.4054054054054006e-05 blue
			883 3.1710079275198195e-05 blue
			1 0.001 blue
			1 0.002 blue
			1 0.001 blue
			1 0.004 blue
			1 0.002 blue
			1 0.002 blue
			1 0.001 blue
			1 0.002 blue
			1 0.003 blue
			1 0.002 blue
			1 0.002 blue
			457 1.531728665207877e-05 blue
			453 8.83002207505518e-06 blue
			451 2.2172949002217298e-05 blue
			449 2.2271714922049e-05 blue
			462 2.597402597402597e-05 blue
			452 3.5398230088495574e-05 blue
			447 2.9082774049216996e-05 blue
			439 4.100227790432801e-05 blue
			458 8.733624454148464e-06 blue
			457 4.376367614879654e-06 blue
			442 9.049773755656116e-06 blue
			451 2.2172949002217285e-05 blue
			455 1.0989010989010984e-05 blue
			454 2.8634361233480185e-05 blue
			445 2.02247191011236e-05 blue
			457 2.1881838074398253e-05 blue
			434 1.6129032258064513e-05 blue
			451 1.773835920177382e-05 blue
			429 2.3310023310023313e-05 blue
			450 1.7777777777777763e-05 blue
			434 1.8433179723502303e-05 blue
			436 1.605504587155963e-05 blue
			430 2.0930232558139536e-05 blue
			451 2.2172949002217285e-05 blue
			429 4.662004662004666e-06 blue
			433 1.6166281755196303e-05 blue
			447 4.0268456375838916e-05 blue
			432 1.1574074074074068e-05 blue
			454 2.2026431718061662e-05 blue
			435 2.0689655172413797e-05 blue
			432 1.3888888888888901e-05 blue
			431 9.280742459396744e-06 blue
			431 1.6241299303944313e-05 blue
			454 1.9823788546255494e-05 blue
			453 1.545253863134659e-05 blue
			431 2.0881670533642695e-05 blue
			449 1.7817371937639215e-05 blue
			450 3.555555555555555e-05 blue
			433 1.8475750577367205e-05 blue
			437 2.059496567505721e-05 blue
			426 1.8779342723004694e-05 blue
			452 5.08849557522124e-05 blue
			430 2.0930232558139536e-05 blue
			446 1.5695067264574005e-05 blue
			442 2.0361990950226248e-05 blue
			454 1.7621145374449325e-05 blue
			741 2.2941970310391364e-05 blue
			774 2.3255813953488394e-05 blue
			802 2.493765586034915e-05 blue
			742 2.695417789757413e-05 blue
			747 2.141900937081662e-05 blue
			770 2.0779220779220798e-05 blue
			776 2.963917525773195e-05 blue
			784 2.551020408163264e-05 blue
			748 2.9411764705882344e-05 blue
			759 -2.635046113306985e-06 blue
			743 1.0767160161507412e-05 blue
			778 2.570694087403601e-05 blue
			789 2.5348542458808607e-05 blue
			738 3.252032520325204e-05 blue
			797 1.6311166875784204e-05 blue
			787 2.4142312579415487e-05 blue
			743 2.422611036339166e-05 blue
			744 1.8817204301075287e-05 blue
			755 1.5894039735099316e-05 blue
			749 2.6702269692923887e-05 blue
			787 2.9224904701397703e-05 blue
			800 1.5000000000000014e-05 blue
			799 2.127659574468087e-05 blue
			748 3.2085561497326196e-05 blue
			772 2.3316062176165822e-05 blue
			772 2.0725388601036287e-05 blue
			743 7.40242261103634e-05 blue
			792 2.0202020202020186e-05 blue
			786 1.9083969465648835e-05 blue
			738 2.7100271002710034e-05 blue
		};
		\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\begin{minipage}[t]{.40\linewidth}
		\begin{tikzpicture}[scale=0.6, transform shape]
		\begin{axis}[
		scatter/classes={blue={mark=x,draw=pbcyan},orange={mark=x,draw=gray},red={mark=x,draw=gray},green={mark=+,draw=pbgreen},purple={mark=x,draw=gray},olive={mark=x,draw=blue},peer={mark=x,draw=white}},
		ylabel=Overhead per transaction,
		xlabel=Transactions,
		xmode=log,
		ymode=log,
		grid=both,
		grid style={line width=.1pt, draw=gray!10},
		major grid style={line width=.2pt,draw=gray!50},
		minor tick num=5,
		xtick={1,10,100,1000,10000, 100000, 1000000, 10000000, 100000000},
		ytick={0,0.1,0.01,0.001,0.0001, 0.00001, 0.000001, 0.0000001, 0.00000001},
		]
		\addplot[scatter,only marks, scatter src=explicit symbolic]%
		table[meta=label] {
			x y label
			197 3.553299492385783e-05 green
			424660 6.499317100739414e-06 green
			4612 0.00593733738074588 green
			2 0.0085 green
			26448 0.015110632183908047 green
			3297 1.6378525932666058e-05 green
			1384 1.4450867052023124e-05 green
			59449 0.09190139447257314 green
			39424 1.065340909090909e-06 green
			3512 1.8792710706150346e-05 green
			1 0.016999999999999998 green
			125076 0.007659023313825193 green
			1764 0.00041666666666666664 green
			4292 0.006946178937558247 green
			1 0.017 green
			4898 0.0023527970600244995 green
			36 0.00030555555555555555 green
			13 0.0006923076923076924 green
			92 0.0002717391304347826 green
			62 0.0003548387096774192 green
			11 0.0008181818181818183 green
			36664 0.00022768928649356313 green
			24245 0.0013703856465250568 green
			62 0.0030161290322580645 green
			2 0.0085 green
			9300 1.6559139784946227e-05 green
			25604 2.7183252616778618e-05 green
			164 0.00023780487804878048 green
			31582 4.147932366537901e-06 green
			16 0.0008125000000000001 green
			1 0.016999999999999998 green
			1 0.018000000000000002 green
			117 0.00019658119658119659 green
			50769 0.006120014181882644 green
			24 0.0018333333333333333 green
			3 0.19733333333333333 green
			5 0.42400000000000004 green
			7968 0.010053840361445783 green
			12285 7.4074074074074075e-06 green
			6960 1.5804597701149419e-06 green
			658 0.03551975683890578 green
			79962 0.1330552137265201 green
			40 0.001 green
			36 0.00036111111111111115 green
			968 7.231404958677685e-06 green
			394 1.015228426395933e-05 green
			3 0.001666666666666666 green
			98 9.183673469387756e-05 green
			72 0.00011111111111111112 green
			180 1.666666666666668e-05 green
			92620 2.548045778449579e-06 green
			279293 4.3764075719763836e-05 green
			48305 1.0205982817513718e-05 green
			407 2.7027027027027027e-05 green
			15320 0.44628844647519583 green
			2752334 0.003914272395719415 green
			63626 0.00689295256656084 green
			39 -2.5641025641025663e-05 green
			35011 0.008423524035303191 green
			87340 0.019595065262193727 green
			1570700 0.006866687464187941 green
			3 0.19099999999999998 green
			10500 2.9523809523809525e-06 green
			2611 9.574875526618154e-06 green
			233180 2.1914400892014756e-06 green
			394 1.01522842639594e-05 green
			19 0.0012105263157894737 green
			118 0.015635593220338983 green
			1969 4.06297613001524e-06 green
			2801 8.211353088182791e-06 green
			88616 0.000620204026360928 green
			586368 2.1437049770792404e-06 green
			394 1.776649746192895e-05 green
			120 0.0007666666666666655 green
			8061 0.0004637141793822107 green
			86 3.488372093023251e-05 green
			224 8.92857142857142e-06 green
			2636 0.0023918816388467374 green
			2 -0.008500000000000002 green
			29431 1.6683089259624207e-05 green
			40 2.500000000000002e-05 green
			57411 0.0003379840100329205 green
			6125 0.0030907755102040817 green
			126 0.0006349206349206337 green
			6 0.15583333333333335 green
			5 0.0618 green
			1539 0.000861598440545809 green
			1556 0.009052699228791775 green
			11 9.090909090909092e-05 green
			2726 0.0974402054292003 green
			4385 0.5556549600912201 green
			19134 0.0034938852304797745 green
			3 0.0013333333333333346 green
			3 0.007666666666666668 green
			423 5.91016548463357e-05 green
			203169 0.0006198337344772087 green
			36 2.7777777777777803e-05 blue
			8155 4.6597179644389985e-06 blue
			1062 3.7664783427495325e-06 blue
			1570700 3.467880562806392e-05 blue
			22761 9.621721365493582e-06 blue
			2754890 0.00012550192566672342 blue
			5 0.014799999999999997 blue
			2214 -1.2195121951219511e-05 blue
			81091 2.4219703789569727e-05 blue
			88649 1.4506649821204978e-05 blue
			53 9.433962264150952e-05 blue
			465 -2.3655913978494616e-05 blue
			968 9.297520661157025e-06 blue
			16 0.0001250000000000001 blue
			10306 7.859499320784009e-06 blue
			286280 6.004610870476457e-06 blue
			1384 9.393063583815027e-06 blue
			3 -0.0013333333333333346 blue
			203019 1.4939488422265894e-05 blue
			3 0.0006666666666666673 blue
			225 2.2222222222222227e-05 blue
			1 0.0049999999999999975 blue
			423 -1.182033096926715e-05 blue
			394 7.61421319796955e-06 blue
			424687 6.522450651891862e-07 blue
			36 0.0005 blue
			92 3.2608695652173903e-05 blue
			1570700 3.521805564398039e-05 blue
			360 8.333333333333322e-06 blue
			586368 2.2306810740013098e-06 blue
			3 0.00033333333333333365 blue
			39424 4.565746753246754e-07 blue
			1 -0.0010000000000000009 blue
			9300 1.5053763440860217e-05 blue
			1969 3.5551041137633347e-06 blue
			197 1.01522842639594e-05 blue
			125076 2.2202500879465286e-05 blue
			1354 1.5509601181683913e-05 blue
			1 0.002 blue
			7326 1.3650013650013661e-07 blue
			6614 8.92047172664035e-06 blue
			2317 2.028485110056107e-05 blue
			26676 0.00011366021892337682 blue
			6960 8.333333333333335e-06 blue
			2053 2.2893326838772527e-05 blue
			125076 2.216252518468771e-05 blue
			2801 6.0692609782220626e-06 blue
			9300 9.139784946236567e-06 blue
			586368 2.1539374590700724e-06 blue
			2754890 5.0814733074642e-05 blue
			9 -0.00033333333333333327 blue
			11 9.090909090909092e-05 blue
			50134 5.545139027406551e-06 blue
			424687 6.710824677939286e-07 blue
			10500 3.2380952380952385e-06 blue
			1 0.0020000000000000018 blue
			16497 1.7639570831060214e-05 blue
			16847 1.1812192081676263e-05 blue
			1384 5.780346820809254e-06 blue
			26676 0.00011519718098665467 blue
			86 1.1627906976744197e-05 blue
			40 0.00032500000000000004 blue
			2636 2.2003034901365705e-05 blue
			30049 2.595760258244867e-05 blue
			4 0.009250000000000001 blue
			53 0.00018867924528301905 blue
			14576 1.1525795828759604e-05 blue
			29431 1.6581155924025687e-05 blue
			6130 1.566068515497553e-05 blue
			394 1.269035532994925e-05 blue
			60632 9.219554030874788e-06 blue
			19 0.0003157894736842104 blue
			4560 4.824561403508773e-06 blue
			126 0.00022222222222222242 blue
			3 0.0006666666666666661 blue
			7 -0.0005714285714285715 blue
			5 0.013399999999999995 blue
			53632 1.2231503579952268e-05 blue
			220 4.5454545454545465e-05 blue
			4899 2.1637068789548883e-05 blue
			7 0.0014285714285714284 blue
			81091 -2.5563872686241477e-05 blue
			36672 1.3361692844677138e-05 blue
			88654 1.4223836487919324e-05 blue
			8155 1.2262415695892102e-06 blue
			57457 3.078824164157543e-05 blue
			2 0.0010000000000000009 blue
			4 0.037250000000000005 blue
			3 0.0013333333333333333 blue
			87912 5.5851305851305816e-06 blue
			376 2.6595744680851086e-06 blue
			16497 3.6976419955143323e-06 blue
			36 0.00016666666666666663 blue
			4 0.008 blue
			2214 1.4453477868112015e-05 blue
			407 3.194103194103194e-05 blue
			234 -7.692307692307691e-05 blue
			1 0.001 blue
			9206 7.820986313273952e-06 blue
			53071 1.1494036291006387e-05 blue
			166 1.8072289156626502e-05 blue
			394 1.269035532994925e-05 blue
			6130 1.598694942903752e-05 blue
			39424 6.594967532467532e-07 blue
			5 0.006999999999999999 blue
			10500 2.6666666666666664e-06 blue
			202 4.950495049504946e-06 blue
			36672 1.1780104712041883e-05 blue
			5622 -0.00010690145855567398 blue
			91 -6.593406593406592e-05 blue
			30049 2.702252986788246e-05 blue
			5 0.008400000000000001 blue
			2127 0.00017254348848142923 blue
			3 0.0013333333333333333 blue
			407 3.1941031941031943e-05 blue
			197 -1.01522842639594e-05 blue
			166 2.4096385542168674e-05 blue
			6614 1.133958270335641e-05 blue
			2471 7.770133549170375e-05 blue
			2636 2.12443095599393e-05 blue
			25605 8.244483499316543e-05 blue
			31582 4.8761953011208926e-06 blue
			1764 0.0004058956916099773 blue
			9 0.0013333333333333333 blue
			394 5.0761421319797e-06 blue
			4684 7.258753202391119e-06 blue
			423 7.09219858156029e-06 blue
			394 2.53807106598985e-06 blue
			1969 5.078720162519049e-06 blue
			40 0.00012500000000000003 blue
			50134 5.764551003311127e-06 blue
			4 0.017750000000000002 blue
			2 0.002 blue
			19134 5.278561722588062e-06 blue
			57430 7.644088455511055e-06 blue
			560 7.142857142857143e-06 blue
			19134 1.6201526079230674e-06 blue
			3297 1.3952077646345167e-05 blue
			234 -1.2820512820512816e-05 blue
			945 3.915343915343916e-05 blue
			36 -0.00016666666666666663 blue
			3 0.0006666666666666673 blue
			1764 0.0004109977324263038 blue
			3 0.0006666666666666673 blue
			91 1.0989010989010999e-05 blue
			1 0.001 blue
			6 0.009833333333333331 blue
			2611 7.276905400229796e-06 blue
			87544 1.691720734716257e-05 blue
			1354 1.5509601181683913e-05 blue
			202 4.950495049504946e-06 blue
			2471 7.770133549170375e-05 blue
			3513 1.2809564474807856e-05 blue
			3297 1.3952077646345167e-05 blue
			968 1.136363636363636e-05 blue
			3542 4.7995482778091454e-05 blue
			945 2.9629629629629627e-05 blue
			1 0.001 blue
			394 1.01522842639594e-05 blue
			5622 -0.0008356456776947668 blue
			57430 7.452550931568866e-06 blue
			10542 2.048947068867388e-05 blue
			7336 5.452562704471101e-07 blue
			61 6.557377049180323e-05 blue
			57457 3.056198548479733e-05 blue
			92 6.521739130434785e-05 blue
			72 4.166666666666666e-05 blue
			22761 6.941698519397231e-06 blue
			98048 6.670202349869452e-06 blue
			60632 6.877556405858289e-06 blue
			464 -4.3103448275862105e-06 blue
			4684 5.764304013663534e-06 blue
			61 3.278688524590167e-05 blue
			29431 1.641126703136149e-05 blue
			233180 2.225748348915002e-06 blue
			2127 0.0001081335213916314 blue
			560 3.5714285714285714e-06 blue
			3513 1.4232849416453175e-05 blue
			6 0.009833333333333331 blue
			4898 1.7762351980400162e-05 blue
			1 0.002 blue
			31582 2.0264707744917976e-06 blue
			19090 7.752750130958618e-06 blue
			4 0.0032499999999999994 blue
			72 2.7777777777777803e-05 blue
			16 0.00031250000000000006 blue
			20 0.00014999999999999996 blue
			360 8.888888888888889e-05 blue
			3542 4.263128176171649e-05 blue
			203015 1.6171218875452557e-05 blue
			87 2.298850574712638e-05 blue
			25604 1.948914232151225e-05 blue
		};
		\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\caption{
		Overhead per \textbf{COMPLEX} transaction on \pb (left) and \miplib (right) on instances with more than 1 seconds in \veripb.
		Each $\times$ marks an instance.
		The $y$-axis gives the time for presolving and
		the $x$-axis gives the time for verifying. Green $+$ mark optimization instances and blue $\times$ mark decision instances.
	}\label{fig:figure2}
\end{figure}


